Squirmers with arbitrary shape and slip: modeling, simulation, and optimization

We consider arbitrary-shaped microswimmers of spherical topology and propose a framework for expressing their slip velocity in terms of tangential basis functions defined on the boundary of the swimmer using the Helmholtz decomposition. Given a time-independent slip velocity profile, we show that the trajectory followed by the microswimmer is a circular helix. We derive analytical expressions for the translational and rotational velocities of a prolate spheroid swimmer in terms of its Helmholtz decomposition modes and explore the effect of aspect ratio on these rigid body velocities. Then, for a given arbitrary swimmer shape of spherical topology, we investigate which slip profile minimizes the total power loss. A partial minimization is performed in which the direction of net motion of the swimmer is prescribed, followed by a global optimization procedure in which the best net motion direction is determined. The optimization results suggest that the competition between linear and rotational optimal motion is linked to symmetries in the shape of the microswimmer.

==> files/macros_local.tex <==
\Newcommand{\bfups}{\boldsymbol{\upupsilon}}
\Newcommand{\uS}{u\Ssup}
\Newcommand{\uSp}{(u\Ssup)'}
\Newcommand{\bffR} {\bff\Rsup}
\Newcommand{\bffHR} {\bffH\Rsup}
\Newcommand{\bfuHR} {\bfuH\Rsup}
\Newcommand{\bfuD} {\bfups\Dsup}
\Newcommand{\bfuS} {\bfups\Ssup}
\Newcommand{\bfwS} {\bfw\Ssup}
\Newcommand{\bfvS} {\bfv\Ssup}
\Newcommand{\bfzS} {\bfz\Ssup}
\Newcommand{\bfuR} {\bfups\Rsup}
\Newcommand{\bfUR} {\bfU\Rsup}
\Newcommand{\bfCR} {\bfC\Rsub}
\Newcommand{\bfDR} {\bfD\Rsub}
\Newcommand{\bfwR} {\bfw\Rsup}
\newcommand{\bfupal}{\boldsymbol{\upalpha}}


==> files/macros_marc.tex <==
\newlength{\kaka}
\newlength{\LSpace}
\newcommand{\Space}[1]{\settowidth{\LSpace}{#1}\rule{\LSpace}{0ex}}
\providecommand{\ahref}[2]{}
\newcommand{\guil}[1]{\og\!#1\!\fg{}}
\newcommand{\slbf}[1]{\textbf{\textsl{#1}}}

%  Sauts de ligne (equations)

\newcommand{\nnum}{\notag \\}
\newcommand{\Suite}[1][0ex]{ \\[#1] & \mbox{}\hspace{15pt}}
\newcommand{\suite}[1][0ex]{\notag \\[#1] & \mbox{}\hspace{15pt}}
% \newcommand{\Suite}[1]{\notag \\[#1] & \mbox{}\hspace{15pt}}
\newcommand{\Nnum}[1]{\notag \\[#1]}
\newcommand{\saut}{ \right. \nnum & \left. \mbox{} }
\newcommand{\saute}{ \right. \\ & \left. \mbox{} }

%  Espacements

\newcommand{\tab}{\hspace*{2em}}
\newcommand{\hs}[1]{\hspace{#1cm}}
%\newcommand{\vs}[1]{\vspace{#1cm}}
% \newcommand{\rl}[2]{\rule{#1cm}{#2cm}}
%\newcommand{\R}{\\ \rule{0.cm}{0.8cm}}

%  Limites

\newcommand{\epszer}{\varepsilon \rightarrow 0}
\newcommand{\limeps}{\lim_{\epszer}}

%  Fonctions

\DeclareMathOperator*{\argmax}{arg\;max}
\DeclareMathOperator*{\argmin}{arg\;min}
%\DeclareMathOperator*{\limsup}{lim\;sup}
\newcommand{\erf}{\operatorname{erf}}
\newcommand{\Log}{\operatorname{Log}}
\renewcommand{\cosh}{\operatorname{ch}}
\renewcommand{\sinh}{\operatorname{sh}}

%  Operateurs differentiels, fonctions...

\newcommand{\Div}{\mbox{div}\,} 
\newcommand{\DivS} {\mbox{div}_{\! S}}
\newcommand{\Rot}{\mbox{\bf rot}\,} 
\newcommand{\RotS}{\mbox{{\bf rot}}_{S}} 
\newcommand{\bfna}{\boldsymbol{\nabla}}
\newcommand{\bfnas}{\boldsymbol{\nabla}\ssup}
\newcommand{\bfnah}{\hat{\bfna}}
\newcommand{\bfnab}{\bar{\bfna}}
\newcommand{\nS}{\bfna_{\!\! S}}
\newcommand{\grad}{\mbox{{\bf grad}}}
\newcommand{\cotg}{\operatorname{cotg}}

%  Connecteurs avec espaces réduits

\newcommand{\shappr}{\hspace*{-0.1em}\approx\hspace*{-0.1em}}
\newcommand{\shtimes}{\hspace*{-0.1em}\times\hspace*{-0.1em}}
\newcommand{\shotimes}{\hspace*{-0.1em}\otimes\hspace*{-0.1em}}
\newcommand{\shcup}{\hspace*{-0.1em}\cup\hspace*{-0.1em}}
\newcommand{\shcap}{\hspace*{-0.1em}\cap\hspace*{-0.1em}}
\newcommand{\shcirc}{\hspace*{-0.1em}\circ\hspace*{-0.1em}}
\newcommand{\shm}{\hspace*{-0.1em}-\hspace*{-0.1em}}
\newcommand{\shp}{\hspace*{-0.1em}+\hspace*{-0.1em}}
\newcommand{\sheq}{\hspace*{-0.1em}=\hspace*{-0.1em}}
\newcommand{\shdeq}{\hspace*{-0.1em}:=\hspace*{-0.1em}}
\newcommand{\shequiv}{\hspace*{-0.1em}\equiv\hspace*{-0.1em}}
\newcommand{\shneq}{\hspace*{-0.1em}\not=\hspace*{-0.1em}}
\newcommand{\shl}{\hspace*{-0.1em}<\hspace*{-0.1em}}
\newcommand{\shg}{\hspace*{-0.1em}>\hspace*{-0.1em}}
\newcommand{\shleq}{\hspace*{-0.1em}\leq\hspace*{-0.1em}}
\newcommand{\shgeq}{\hspace*{-0.1em}\geq\hspace*{-0.1em}}
\newcommand{\shll}{\hspace*{-0.1em}\ll\hspace*{-0.1em}}
\newcommand{\shgg}{\hspace*{-0.1em}\gg\hspace*{-0.1em}}
\newcommand{\shin}{\hspace*{-0.1em}\in\hspace*{-0.1em}}
\newcommand{\shni}{\hspace*{-0.1em}\ni\hspace*{-0.1em}}
\newcommand{\shnin}{\hspace*{-0.1em}\not\in\hspace*{-0.1em}}
\newcommand{\shsetm}{\hspace*{-0.1em}\setminus\hspace*{-0.1em}}
\newcommand{\shsubs}{\hspace*{-0.1em}\subset\hspace*{-0.1em}}
\newcommand{\shSubs}{\hspace*{-0.1em}\Subset\hspace*{-0.1em}}
\newcommand{\shsups}{\hspace*{-0.1em}\supset\hspace*{-0.1em}}
\newcommand{\shnsubs}{\hspace*{-0.1em}\not\subset\hspace*{-0.1em}}
\newcommand{\shsubseq}{\hspace*{-0.1em}\subseteq\hspace*{-0.1em}}
\newcommand{\shoplus}{\hspace*{-0.1em}\oplus\hspace*{-0.1em}}
\newcommand{\vecpr}{\hspace*{-0.1em}\wedge\hspace*{-0.1em}}

%  ----------
%  OPERATEURS
%  ----------

%  Derivees

\newcommand{\del}[1][]{\partial_{#1}}
\newcommand{\derp}[2]{\dfrac{\partial #1}{\partial #2}}
\newcommand{\derpp}[2]{\dfrac{\partial^{2} #1}{\partial #2^{2}}}
\newcommand{\derppp}[2]{\dfrac{\partial^{3} #1}{\partial #2^{3}}}
\newcommand{\derpppp}[2]{\dfrac{\partial^{4} #1}{\partial #2^{4}}}
\newcommand{\derpq}[3]{\dfrac{\partial^{2} #1}{\partial #2 \partial #3}}
\newcommand{\der}[2]{\dfrac{\text{d}#1}{\text{d}#2}}
\newcommand{\ders}[2]{\dfrac{\text{d}^{2}#1}{\text{d}#2^{2}}}
\newcommand{\derpT}[2]{\partial #1/\partial #2}
\newcommand{\derpqT}[3]{\partial^{2} #1/\partial #2\partial #3}

\newcommand{\tder}[2]{\text{d}#1/\text{d}#2}
%\renewcommand{\del}[1]{\partial_{#1}}
\newcommand{\ddel}[1]{\partial_{#1}^2}
\newcommand{\dddel}[1]{\partial_{#1}^3}

%  Derivees particulaires

\newcommand{\dd}[1]{\protect\settowidth{\kaka}{\mbox{$#1$}}\protect\makebox[\kaka]{$\buildrel{\scriptscriptstyle\star}\over{#1}$}}
%\newcommand{\dd}[1]{\raisebox{-.4ex}{\mbox{$\stackrel{*}{#1}$}}\!}
%\newcommand{\dd}[1]{\stackrel{\star}{#1}}
%\newcommand{\dd}[1]{\stackrel{\star}{#1}\!\!\rule{0em}{1ex}}
\newcommand{\dvv}[1]{\stackrel{\scriptscriptstyle\star\vee}{#1}\!\!\rule{0em}{1ex}}
\newcommand{\vd}[1]{\stackrel{\scriptscriptstyle\vee\star}{#1}\!\!\rule{0em}{1ex}}
\newcommand{\vv}[1]{\stackrel{\scriptscriptstyle\vee}{#1}\!\!\rule{0em}{1ex}}
\newcommand{\ddpG}{\dd{p}_{\G}}
\newcommand{\ddqG}{\dd{q}_{\G}}
\newcommand{\DD}[1]{\protect\settowidth{\kaka}{\mbox{$#1$}}\makebox[\kaka]{$\buildrel{\diamond}\over{#1}$}}

% Notations pour le calcul tensoriel

\newcommand{\tens}{\hspace*{-1pt}\otimes\hspace*{-1pt}}
%\newcommand{\tens}[2] {#1 \!\otimes\! #2}
\newcommand{\contr}[2] {#1 {\boldsymbol{\cdot}} #2}
\newcommand{\dcontr}[2] {#1 : #2}
\newcommand{\T}[1]{\underline{#1}}
\newcommand{\TT}[1]{\T{\T{#1}}}
\newcommand{\TTT}[1]{\T{\TT{#1}}}
\newcommand{\TTTT}[1]{\T{\TTT{#1}}}

%  Autres

\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\bil}[2]{{\cal B}(#1,#2)}
\newcommand{\bracket}[1]{\langle #1 \rangle}
\newcommand{\Cbil}[2]{{\cal B}^{2}(#1,#2;\bfth,\bfmu)}
\newcommand{\Dbil}[2]{{\cal B}^{1}(#1,#2;\bfth)}
\newcommand{\ddbil}[2]{\dd{\cal D}(#1,#2)}
\newcommand{\dvbil}[2]{\dv{\cal D}(#1,#2)}
\newcommand{\innp}[3]{\lbra #1 , #2 \rbra_{#3}}
\newcommand{\pinv}[1]{\tfrac{1}{#1}}
\newcommand{\inv}[1]{\dfrac{1}{#1}}
\newcommand{\invm}[1]{\frac{-1}{#1}}
\newcommand{\jump}[1]{[\![ {#1} ]\!]}
\newcommand{\Jump}[1]{\bigl[\!\!\bigl[ {#1} \bigr]\!\!\bigr]}
\newcommand{\JUMP}[1]{\Bigl[\!\!\Bigl[ {#1} \Bigr]\!\!\Bigr]}
\newcommand{\moy}[2][]{{\left\langle{#2}\right\rangle}_{#1}}
\newcommand{\Norm}[2][]{\| #2 \|_{#1}}
\newcommand{\norm}[1]{\| \boldsymbol{#1} \|}
\newcommand{\norms}[1]{\| #1 \|}
\newcommand{\scal}[2]{#1 . #2}
\newcommand{\scalb}[2]{\boldsymbol{\dsmth #1 . #2}}
\newcommand{\Tn}[1]{\bfT^{n}[\boldsymbol{#1}]}
\newcommand{\vecp}[2]{\boldsymbol{#1}\wedge\boldsymbol{#2}}
\newcommand{\lbra}{\big\langle\hspace*{0.1em}}
\newcommand{\rbra}{\hspace*{0.1em}\big\rangle}
\newcommand{\Lbra}{\Big\langle\hspace*{0.1em}}
\newcommand{\Rbra}{\hspace*{0.1em}\Big\rangle}
\newcommand{\lsqb}{\big[\hspace*{0.1em}}
\newcommand{\rsqb}{\hspace*{0.1em}\big]}
\newcommand{\lcb}{\big\{\hspace*{0.1em}}
\newcommand{\rcb}{\hspace*{0.1em}\big\}}
\newcommand{\Lcb}{\Big\{\hspace*{0.1em}}
\newcommand{\Rcb}{\hspace*{0.1em}\Big\}}
\newcommand{\Lsqb}{\Big[\hspace*{0.1em}}
\newcommand{\Rsqb}{\hspace*{0.1em}\Big]}
\newcommand{\lpar}{\big(\hspace*{0.1em}}
\newcommand{\rpar}{\hspace*{0.1em}\big)}
\newcommand{\llpar}{\big(\!\big(\hspace*{0.1em}}
\newcommand{\rrpar}{\hspace*{0.1em}\big)\!\big)}
\newcommand{\labs}{\big|\hspace*{0.1em}}
\newcommand{\rabs}{\hspace*{0.1em}\big|}
\newcommand{\Labs}{\Big|\hspace*{0.1em}}
\newcommand{\Rabs}{\hspace*{0.1em}\Big|}
\newcommand{\lnrm}{\big\|\hspace*{0.1em}}
\newcommand{\rnrm}{\hspace*{0.1em}\big\|}
\newcommand{\Lnrm}{\Big\|\hspace*{0.1em}}
\newcommand{\Rnrm}{\hspace*{0.1em}\Big\|}
\newcommand{\Lpar}{\Big(\,}
\newcommand{\Rpar}{\,\Big)}

%  ------
%  DIVERS
%  ------

%  Liste de noms

\newcommand{\itempers}[2]{\item[{\rm #1} {\sc #2}]\mbox{\,}}
\newcommand{\pers}[2]{{\rm #1} {\sc #2}}
\newcommand{\itemT}{\item[$\triangleright$]}

\newcommand{\Vskm}{\vspace*{-1ex}}
\newcommand{\Vskp}{\vspace*{1ex}}
\newcommand{\VskM}{\vspace*{-2ex}}
\newcommand{\VskP}{\vspace*{2ex}}

%  Annotated equal sign

\newcommand{\Eq}[1]{\stackrel{\text{#1}}{=}}


%
%  Biblio en plusieurs morceaux, avec numerotation sequentielle%
%
\newcounter{refcounter}
\usepackage{ifthen}
\newenvironment{multibiblio}{
\begin{thebibliography}{}
\addtocounter{enumi}{\therefcounter}
}{
\ifthenelse{\value{enumi} = \value{refcounter}}{}{\setcounter{refcounter}{\value{enumi}}}
\end{thebibliography}
}
%
%  Appel bibliographie par BibTeX
%
\newcommand{\Biblista}{/home/mbonnet/tex/bibtex/biblio}
%\newcommand{\Biblista}{/home/mbonnet/tex/bibtex/biblio,/home/mbonnet/tex/bibtex/bibliomb}
\newcommand{\biblista}{/home/mbonnet/tex/bibtex/bibliof,/home/mbonnet/tex/bibtex/bibliomb}
%\newcommand{\biblisto}{/home/mbonnet/tex/bibtex/bibliof,/home/mbonnet/tex/bibtex/or,/home/mbonnet/tex/bibtex/bui}
\newcommand{\biblistb}%
  {/home/mbonnet/tex/bibtex/articles,/home/mbonnet/tex/bibtex/book,/home/mbonnet/tex/bibtex/or,/home/mbonnet/tex/bibtex/mb/articles,/home/mbonnet/tex/bibtex/mb/articlesap,/home/mbonnet/tex/bibtex/mb/articlessub,/home/mbonnet/tex/bibtex/mb/articlesprep,/home/mbonnet/tex/bibtex/mb/livre}
\newcommand{\biblistc}%
  {/home/mbonnet/tex/bibtex/incoll,/home/mbonnet/tex/bibtex/inproc,/home/mbonnet/tex/bibtex/rapp}
\newcommand{\biblistd}%
%  {/home/mbonnet/tex/bibtex/misc,/home/mbonnet/tex/bibtex/theses,/home/mbonnet/tex/bibtex/bui,/home/mbonnet/tex/bibtex/fiabilite,/home/mbonnet/tex/bibtex/couplage,/home/mbonnet/tex/final/ip03/ip03}
  {/home/mbonnet/tex/bibtex/td,/home/mbonnet/tex/bibtex/misc,/home/mbonnet/tex/bibtex/theses,/home/mbonnet/tex/bibtex/bui,/home/mbonnet/tex/bibtex/fiabilite,/home/mbonnet/tex/bibtex/couplage,/home/mbonnet/tex/bibtex/gdrchamps,/home/mbonnet/tex/bibtex/massimiliano,/home/mbonnet/tex/Conferences/compdyn/biblioICEGE}

\newcommand{\biblist}{\biblista,\biblistb,\biblistc,\biblistd}
\newcommand{\Biblist}{\Biblista,\biblistb,\biblistc,\biblistd}
\newcommand{\makebibliography}[2][/home/mbonnet/tex/bibtex/]{%
\bibliographystyle{#1#2}%
\bibliography{\Biblist}%
}

\newcommand{\makebibliographyf}[1]{%
\bibliographystyle{/home/mbonnet/tex/bibtex/#1}%
\bibliography{\biblist}%
}

%\newcommand{\makebibliographylms}[1]{%
%\bibliographystyle{/home/mbonnet/tex/bibtex/#1}%
%\bibliography{/home/mbonnet/tex/bibtex/biblio,/home/mbonnet/tex/bibtex/lms9697}%
%}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:
\newcommand{\bfus} {\boldsymbol{u}^{\star}}
\newcommand{\bfCs} {\boldsymbol{C}^{\star}}
\newcommand{\bfrhR} {\Rmath{\hat{\bfrR}}{}}
\newcommand{\bfTC} {\bfT\Csup}
\newcommand{\bfuF} {\bfu\Fsup}
\newcommand{\bfum} {\bfu\obs}
\newcommand{\bfrZ} {\bfr^{0}}
\newcommand{\bfyZ} {\bfy^{0}}
\newcommand{\rZ} {r^{0}}
% \newcommand{\xZ} {x^{0}}
% \newcommand{\yZ} {y^{0}}

\newcommand{\bfTGR} {\bfTR\Gsup}
\newcommand{\bfTCR} {\bfTR\Csup}
\newcommand{\bfuFR} {\bfuR\Fsup}
\newcommand{\bfumR} {\bfuR\obs}

\newcommand{\bfrZR} {\bfrR^{0}}
\newcommand{\bfyZR} {\bfyR^{0}}

\newcommand{\bfuGR}{\bfuR^{c}}
\newcommand{\bftGR}{\bftR^{c}}
\newcommand{\bfuGB}{\bfuB^{c}}
\newcommand{\bftGB}{\bftB^{c}}
\newcommand{\bfTGB} {\bfTB\Gsup}
\newcommand{\bfTCB} {\bfTB\Csup}
\newcommand{\bfuFB} {\bfuB\Fsup}
\newcommand{\bfumB} {\bfuB\obs}

\newcommand{\bfrZB} {\bfrB^{0}}
\newcommand{\bfyZB} {\bfyB^{0}}

\newcommand{\bfun}{\mathbf{1}}
\newcommand{\bfze}{\mathbf{0}}

\newcommand{\bfqd}{\bfq^{\scriptscriptstyle D\hspace{-1pt}}}
\newcommand{\bfTd}{\bfT^{\scriptscriptstyle D\hspace{-1pt}}}
\newcommand{\bftd}{\bft^{\scriptscriptstyle D\hspace{-1pt}}}
\newcommand{\bfud}{\bfu^{\scriptscriptstyle D\hspace{-1pt}}}
\newcommand{\bfuhd}{\bfuh{}^{\scriptscriptstyle D\hspace{-1pt}}}
\newcommand{\bfuo} {\bfu\obs}
\newcommand{\bfvo} {\bfv\obs}

\newcommand{\tilchi}{\tilde{\chi}}
\newcommand{\tileps}{\tilde{\varepsilon}}
\newcommand{\tillbd}{\tilde{\lambda}}
\newcommand{\tilph}{\widetilde{\phi}}
\newcommand{\tilps}{\widetilde{\psi}}
\newcommand{\tilze}{\widetilde{\zeta}}
\newcommand{\tiltau}{\tilde{\tau}}
\newcommand{\tilxi}{\tilde{\xi}}
\newcommand{\tilvph}{\tilde{\varphi}}
\newcommand{\Tilvph}{\widetilde{\varphi}}

\newcommand{\CSh} {\hat{\CS}}

\newcommand{\bfubh} {\hat{\bfub}{}}

\newcommand{\hatu}{\hat{u}}
\newcommand{\hatQ}{\hat{Q}}
\newcommand{\hatp}{\hat{p}}
\newcommand{\hatq}{\hat{q}}
\newcommand{\hatr}{\hat{r}}
\newcommand{\hatS}{\hat{S}}
\newcommand{\hatt}{\hat{t}}
\newcommand{\ooh}{\hat{\oo}}
\newcommand{\hOO}{\hat{\OO}}
\newcommand{\Eh} {\hat{E}}
\newcommand{\ph} {\hat{p}}
\newcommand{\qh} {\hat{q}}
\newcommand{\uh} {\hat{u}}
\newcommand{\wh} {\hat{w}}
\newcommand{\Uh} {\hat{U}}

\newcommand{\bfrbh} {\hat{\bar{\boldsymbol{r}}}{}}

\newcommand{\OObar}{\bar{\Omega}{}}
\newcommand{\xb} {\bar{x}{}}

\newcommand{\bfpS} {\boldsymbol{p}^{\star}}

\newcommand{\UUt}{\widetilde{\Ubb}}
\newcommand{\UUh}{\hat{\Ubb}}

%\newcommand{\bfm}[1]{\mbox{\boldmath $#1$}}
% --------------------------
% SYMBOLES PRECEDES DE DELTA
%
%  1) delta (minuscule)
% --------------------------

\newcommand{\delA}{\delta A}
\newcommand{\delB}{\delta B}
\newcommand{\delC}{\delta C}
\newcommand{\DelA}{\Delta A}
\newcommand{\DelB}{\Delta B}
\newcommand{\DelC}{\Delta C}
\newcommand{\DelE}{\Delta E}
\newcommand{\dk}{\delta k}
\newcommand{\dm}{\delta m}
\newcommand{\dmb}{\delta\bfm}
\newcommand{\dpb}{\delta\bfp}
\newcommand{\dbfC}{\delta\bfC}
\newcommand{\dCS}{\delta\CS}
\newcommand{\DCS}{\Delta\CS}
\newcommand{\DCSt}{\widetilde{\DCS}}
%\newcommand{\du}{\delta u}
\newcommand{\dela}{\delta a}
\newcommand{\delu}{\delta u}
\newcommand{\deluh}{\delta \hat{u}}
\newcommand{\delv}{\delta v}
\newcommand{\dsig}{\delta\sigma}
%\newcommand{\dth}{\delta\theta}
\newcommand{\dbfT}{\delta\bfT}
\newcommand{\dbfU}{\delta\bfU}
\newcommand{\dbfd}{\delta\bfd}
\newcommand{\dub}{\delta\bfu}
\newcommand{\dwb}{\delta\bfw}
\newcommand{\dyb}{\delta\bfy}
\newcommand{\deps}{\delta\bfeps}
\newcommand{\dXb}{\delta\bfX}
\newcommand{\dq}{\delta q}
\newcommand{\dep}{\delta p}
\newcommand{\de}{\delta \eta}
\newcommand{\dJ}{\delta J}
\newcommand{\dL}{\delta \Lcal}
\newcommand{\dpsi}{\delta \psi}
\newcommand{\dbfxi}{\delta\bfxi}
\newcommand{\dbfu}{\delta\bfu}
\newcommand{\dbft}{\delta\bft}
\newcommand{\Drho}{\Delta\rho}
\newcommand{\doo}{\delta\omega}
\newcommand{\dw}{\delta w}
\newcommand{\delp}{\delta p}
\newcommand{\dM}{\delta M}
\newcommand{\dP}{\delta P}
\newcommand{\dQ}{\delta Q}
\newcommand{\dR}{\delta R}
\newcommand{\dpN}{\delta\varphi_{N}}
\newcommand{\dpT}{\delta\varphi_{T}}
%\newcommand{\dbfy}{\delta\bfy}
\newcommand{\depsp}{\delta\bfepsp}

% --------------------------
%  2) Delta (majuscule)
% --------------------------

\newcommand{\DC}[1] {\Delta C(\bfm{#1})}

\newcommand{\DCC}{\bfm \Delta C}
\newcommand{\Dbfe}{\Delta\bfe}
\newcommand{\DbfF}{\Delta\bfF}
\newcommand{\Dbff}{\Delta\bff}
\newcommand{\Dbfh}{\Delta\bfh}
\newcommand{\Dmb}{\Delta\bfm}
\newcommand{\Dbfp}{\Delta\bfp}
\newcommand{\Dbft}{\Delta\bft}
\newcommand{\Dbfu}{\Delta\bfu}
\newcommand{\Dbfy}{\Delta\bfy}
\newcommand{\DelS}{\Delta S}
\newcommand{\DX}{\Delta X}
\newcommand{\Dk}{\Delta k}
\newcommand{\Dr}{\Delta r}
\newcommand{\Du}{\Delta u}
\newcommand{\Dee}{\Delta\TT{e}}
\newcommand{\Dxi}{\Delta\bfxi}
\newcommand{\Deps}{\Delta\bfeps}
\newcommand{\Dsig}{\Delta\bfsig} 
\newcommand{\Dtilu}{\Delta\tilu}
\newcommand{\DU}{\Delta U}
\newcommand{\DK}{\Delta K}
\newcommand{\DM}{\Delta M}
\newcommand{\DbfK}{\Delta {\bf K}}
\newcommand{\DbfM}{\Delta {\bf M}}
\newcommand{\Dx}{\Delta x}
\newcommand{\Dt}{\Delta t}
\newcommand{\DT}{\Delta T}
\newcommand{\Depb}{\Delta\epb}
\newcommand{\Depsp}{\Delta\bfepsp}
\newcommand{\Dpb}{\Delta\bfp}
\newcommand{\Dub}{\Delta\bfu}
\newcommand{\Dp}{\Delta p}
\newcommand{\bfdp}{\bfd\psup}

\newcommand{\bfepse}{\bfeps\esup}
\newcommand{\bfepsel}{\bfeps\el}
\newcommand{\bfepsp}{\bfeps^{\text{\tiny P}}}
\newcommand{\bfepsd}{\dot{\bfeps}}
\newcommand{\bfepspd}{\dot{\bfeps}{}\psup}
\newcommand{\bfepsvp}{\bfeps^{\text{\tiny VP}}}
\newcommand{\bfepsvpd}{\dot{\bfeps}^{\text{\tiny VP}}}
\newcommand{\bfald}{\dot{\bfal}}
\newcommand{\alphad}{\dot{\alpha}}
\newcommand{\alphadd}{\ddot{\alpha}}
\newcommand{\sigmad}{\dot{\sigma}}

\newcommand{\ddepb}{\dd{\ebar}{}\psup}

\newcommand{\elaseq}{^{\text{elas,eq}}}

\newcommand{\epbd}{\dot{\ebar}{}\psup}

\newcommand{\epb}{\ebar\psup}

\newcommand{\epsbp}{\bar{\bfeps}\psup}
\newcommand{\epse}{\eps\el}
\newcommand{\epspd}{\dot{\eps}\psup}
\newcommand{\epsp}{\eps\psup}
\newcommand{\epsd}{\dot{\eps}}

\newcommand{\evpbd}{\dot{\ebar}^{\text{\tiny VP}}}
\newcommand{\evpb}{\ebar^{\text{\tiny VP}}}

\newcommand{\hatn}{\hat{\bfn}}

\newcommand{\sigelaseq}{\sigma^{\text{elas,eq}}}

\newcommand{\sigeq}{\sigma^{\text{eq}}}

\newcommand{\sqdth}{\sqrt{2/3}}
\newcommand{\sqdt}{\sqrt{\mbox{$\frac{2}{3}$}}}
\newcommand{\sqtdh}{\sqrt{3/2}}
\newcommand{\sqtd}{\sqrt{\mbox{$\frac{3}{2}$}}}
\newcommand{\sqtt}{\sqrt{\mbox{$\frac{2}{3}$}}}


% --------------------
% DOMAINES, FRONTIERES
% --------------------

%  variations sur \Omega

\newcommand{\Oee}{\OO_{e}}
\newcommand{\OO}{\Omega}
\newcommand{\OOi}{\OO_{\infty}}
\newcommand{\OOo}{\overline{\OO}}
\newcommand{\OOb}{\bar{\OO}}
\newcommand{\OOB}{\OO_{B}}
\newcommand{\OOib}{\OOb_{\infty}}
\newcommand{\OOm}{\Omega^{-}}
\newcommand{\OOG}{\Omega_{\G}}
\newcommand{\OOp}{\OO_{\text{\tiny P}}}
\newcommand{\OOe}{\OO_{\varepsilon}}
%\newcommand{\OOc}{\OO^{c}}
\newcommand{\OOh}{\OO_{h}}
\newcommand{\OOt}{\Omega\true}
\newcommand{\OOz}{\Omega_0}
\newcommand{\tilOOp}{\tilde{\OO}^{\text{\tiny P}}}
\newcommand{\Sige}{\Sigma_{\varepsilon}}

%  variations sur \Gamma

\newcommand{\G}{\Gamma}
\newcommand{\Ga}{\G_{a}}
\newcommand{\Gb}{\bar{\G}}
\newcommand{\Gc}{\G_{c}}
\newcommand{\Ge}{\G(e)}
\newcommand{\Gt}{\G\!\Tsub}
\newcommand{\Gte}{\Gt^{e}}
\newcommand{\Gxi}{\G_{\xi}}
\newcommand{\Gi}{\G_{i}}
% \newcommand{\Gm}{\G_{\text{m}}}
\newcommand{\Gm}{\G_{m}}
\newcommand{\Gss}{\scriptscriptstyle\Gamma}
\newcommand{\Gd}{\G_{d}}
\newcommand{\Gu}{\G_{u}}
\newcommand{\Gp}{\G_{p}}
\newcommand{\Gq}{\G_{q}}
\newcommand{\Gpm}{\G^{-}_{p}}
\newcommand{\Gpp}{\G^{+}_{p}}
% \newcommand{\Gs}{\G_{\text{s}}}
\newcommand{\Gs}{\G_{s}}
\newcommand{\Gtr}{\G\true}
\newcommand{\Gst}{\G^{\star}}
\newcommand{\GD}{\Gamma_{\text{D}}}
\newcommand{\GN}{\Gamma_{\text{N}}}

%  variations sur S

\newcommand{\SCeff}{S\Csub^{\text{eff}}}
\newcommand{\SC}{S\Csub}
\newcommand{\SD}{S_{\text{D}}}
\newcommand{\SN}{S_{\text{N}}}
% \providecommand{\Sp}{}
% \renewcommand{\Sp}{S_{p}}
\Newcommand{\Sp}{S_{p}}
\newcommand{\So}{S\obs}
\newcommand{\SoN}{\SN\Obs}
\newcommand{\SoD}{\SD\Obs}
\newcommand{\Sq}{S_q}
\newcommand{\Ss}{S_{\text{sym}}}
\newcommand{\St}{S\Tsub}
\newcommand{\Stt}{\tilS_{T}}
\newcommand{\Stu}{\tilS_{u}}
\newcommand{\Su}{S_u}
\newcommand{\Sxi}{S_{\xi}}
\newcommand{\Sm}{S_{\text{obs}}}

%  divers avec \epsilon

\newcommand{\Be}{B_{\varepsilon}}
\newcommand{\Bex}{\Be(\bfx)}
\newcommand{\ce}{e_{\varepsilon}}
\newcommand{\Ce}{C_{\varepsilon}}
\newcommand{\De}{D_{\varepsilon}}
\newcommand{\deee}{\partial\eee}
\newcommand{\Dex}{\De(\bfx)}
\newcommand{\dGe}{\partial\G_{\varepsilon}}
\newcommand{\dOe}{\dO-\eee}
\newcommand{\dOes}{(\dOe)+s_{\varepsilon}}
\newcommand{\dse}{\partial\se}
\newcommand{\dve}{\partial\ve}
\newcommand{\eee}{e_{\varepsilon}}
\newcommand{\Gee}{\G_{\varepsilon}}
\newcommand{\Ges}{\Gee + \se}
\newcommand{\Gme}{\G - e_{\varepsilon}}
\newcommand{\Oe}{\OO_{\varepsilon}}
\newcommand{\Oex}{\Oe(\bfx)}
\newcommand{\Sc}{S_{c}}
\newcommand{\See}{S-e_{\varepsilon}}
\newcommand{\se}{s_{\varepsilon}}
\newcommand{\Se}{S_{\varepsilon}}
\newcommand{\Sex}{\Se(\bfx)}
\newcommand{\ve}{v_{\varepsilon}}
\newcommand{\Ve}{V_{\varepsilon}}
\newcommand{\vexi}{\ve(\bfxi)}
\newcommand{\vex}{\ve(\bfx)}

%  divers

\newcommand{\Cp}{C_{p}}
\newcommand{\Cu}{C_{u}}
\newcommand{\Rm}{R_{m}}
\newcommand{\Rs}{R_{s}}
\newcommand{\Vt}{\V_{T}}
\newcommand{\Vu}{\V_{u}}

%  Frontieres

\newcommand{\dB}{\partial B}
\newcommand{\dC}{\partial C}
\newcommand{\dD}{\partial D}
\newcommand{\ddSe}{\partial \Se}
\newcommand{\ddS}{\partial S}
\newcommand{\ddV}{\partial V}
\newcommand{\dE}{\partial E}
\newcommand{\dG}{\partial\G}
\newcommand{\dO}{\partial\OO}
\newcommand{\doO}{\partial_{0}\OO}
\newcommand{\dOp}{\partial\OOp}
\newcommand{\dTO}{\partial_{\T{T}}\OO}

%  ----------------------
%  ELEMENTS DIFFERENTIELS
%  ----------------------

\newcommand{\da}{\,\text{d}a}
\newcommand{\dal}{\,\text{d}\alpha}
\newcommand{\dax}{\,\text{d}a_{x}}
\newcommand{\dbfa}{\,\text{d}\bfa}
\newcommand{\dbfm}{\,\text{d}\bfm}
\newcommand{\dbfs}{\,\text{d}\bfs}
\newcommand{\dbfsh}{\,\text{d}\bfsh}
\newcommand{\dbfx}{\,\text{d}\bfx}
\newcommand{\dbfy}{\,\text{d}\bfy}
\newcommand{\dbfyb}{\,\text{d}\bfyb}
\newcommand{\dbfyT}{\,\text{d}\bfyT}
\newcommand{\dbfz}{\,\text{d}\bfz}
\newcommand{\dbfeta}{\,\text{d}\bfeta}
\newcommand{\dbxi}{\,\text{d}\bfxi}
\newcommand{\dbfzet}{\,\text{d}\bfzet}
\newcommand{\db}{\,\text{d}b}
\newcommand{\dc}{\,\text{d}c}
\newcommand{\dCy}{\,\text{d}C_{y}}
\newcommand{\dDy}{\,\text{d}D_{y}}
\newcommand{\ddR}{\,\text{d}R}
\newcommand{\deta}{\,\text{d}\eta}
\newcommand{\dGG}{\;\text{d}\G}
\newcommand{\dGx}{\dGG_{\! x}}
\newcommand{\dGxib}{\;\text{d}\bar{\G}_{\xib}}
\newcommand{\dGxi}{\;\text{d}\G_{\xi}}
\newcommand{\dla}{\,\text{d}\lambda}
\newcommand{\dMM}{\;\text{d}M}
\newcommand{\dOb}{\partial\Obar}
\newcommand{\dOO}{\;\text{d}\OO}
\newcommand{\dom}{\;\text{d}\oo}
\newcommand{\dOx}{\dOO_{x}}
\newcommand{\dOxi}{\dOO_{\xi}}
%\Newcommand{\dp}{\,\text{d}p}
\newcommand{\dph}{\;\text{d}\phi}
\newcommand{\dvph}{\;\text{d}\varphi}
\newcommand{\dvrho}{\;\text{d}\varrho}
\newcommand{\drb}{\;\text{d}\rbar}
\newcommand{\dr}{\,\text{d}r}
\newcommand{\drho}{\;\text{d}\rho}
\newcommand{\ds}{\,\text{d}s}
\newcommand{\dS}{\,\text{d}S}
\newcommand{\dSb}{\,\text{d}\overline{S}}
\newcommand{\dsfS}{\,\text{d}\sfS}
\newcommand{\dsfV}{\,\text{d}\sfV}
\newcommand{\dST}{\,\text{d}\widetilde{S}}
\newcommand{\dSxib}{\,\text{d}S_{\xib}}
\newcommand{\dSxih}{\,\text{d}S_{\xih}}
\newcommand{\dSxi}{\,\text{d}S_{\xi}}
\newcommand{\dsxt}{\ds_{\tilx}}
\newcommand{\dsx}{\,\text{d}s_{x}}
\newcommand{\dSx}{\,\text{d}S_{x}}
% \newcommand{\dSxh}{\,\text{d}S_{\hatx}}
\newcommand{\dSxt}{\,\text{d}S_{\tilx}}
\newcommand{\dsy}{\,\text{d}s_{y}}
\newcommand{\dSy}{\,\text{d}S_{y}}
\newcommand{\dSyb}{\,\text{d}S_{\ybar}}
\newcommand{\dSz}{\,\text{d}S_{z}}
\newcommand{\dtau}{\,\text{d}\tau}
\newcommand{\dthv}{\;\text{d}\vartheta}
\newcommand{\dth}{\;\text{d}\theta}
\newcommand{\dTh}{\;\text{d}\Theta}
\newcommand{\dthxi}{\;\text{d}\vartheta_{\xib}}
\newcommand{\dT}{\,\text{d}T}
\newcommand{\dt}{\,\text{d}t}
\newcommand{\du}{\,\text{d}u}
\newcommand{\dv}{\,\text{d}v}
\newcommand{\dV}{\;\text{d}V}
\newcommand{\JdV}{\;J\text{d}V}
\newcommand{\dVb}{\;\text{d}\overline{V}}
\newcommand{\dVT}{\;\text{d}\widetilde{V}}
\newcommand{\dVxib}{\;\text{d}\bar{V}_{\xib}}
\newcommand{\dVxb}{\;\text{d}\bar{V}_{\xb}}
\newcommand{\dVxi}{\;\text{d}V_{\xi}}
\newcommand{\dVx}{\,\text{d}V_{x}}
\newcommand{\dVxt}{\,\text{d}V_{\tilx}}
\newcommand{\dVy}{\,\text{d}V_{y}}
\newcommand{\dVyb}{\;\text{d}\bar{V}_{\ybar}}
\newcommand{\dVz}{\,\text{d}V_{z}}
%\newcommand{\dw}{\,\text{d}w}
\newcommand{\dxb}{\,\text{d}\bfx}
\newcommand{\dxi}{\,\text{d}\xi}
\newcommand{\dxib}{\,\text{d}\xib}
\newcommand{\dx}{\,\text{d}x}
\newcommand{\dy}{\,\text{d}y}
\newcommand{\dz}{\,\text{d}z}
%\renewcommand{\dv}{\,\text{d}v}
%  ----------
%  INTEGRALES
%  ----------

%  Integrales avec \Omega

\newcommand{\idOb}{\int_{\partial\Obar}}
\newcommand{\idO}{\int_{\dO}}
\newcommand{\idOp} {\int_{\dOp}}
\newcommand{\idOt} {\int_{\dO(t)}}
\newcommand{\idOo} {\int_{\partial_{0}\OO}}
\newcommand{\idTO}{\int_{\partial_T\OO}}
\newcommand{\idzO}{\int_{\partial_0\OO}}
\newcommand{\iOb}{\int_{\Obar}}
\newcommand{\iOc}{\int_{\OOc}}
\newcommand{\iOh}{\int_{\OO_{h}}}
\newcommand{\iOl}{\int_{\OO(\ell)}}
\newcommand{\iOldl}{\int_{\OO(\ell + \text{d}\ell)}}
\newcommand{\io}[1][]{\int_{\oo_{#1}}}
\newcommand{\iO}{\int_{\OO}}
\newcommand{\iOm}{\int_{\OOm}}
\newcommand{\iOp}{\int_{\OOp}}
\newcommand{\iOpt}{\int_{\tilde{\OOp}}}
\newcommand{\iOr}{\int_{\OOr}}
\newcommand{\iOt}{\int_{\OO(t)}}
\newcommand{\iOz}{\int_{\OO_0}}

%  Integrales avec \Gamma

\newcommand{\idG} {\int_{\partial\G}}
\newcommand{\iGa} {\int_{\G_{a}}}
\newcommand{\iGb} {\int_{\G_{b}}}
\newcommand{\iGbar} {\int_{\bar{\G}}}
\newcommand{\iGc}{\int_{\Gc}}
\newcommand{\iGd} {\int_{\G_{d}}}
\newcommand{\iGh} {\int_{\G_{h}}}
\newcommand{\iG} {\int_{\G}}
\newcommand{\iGk} {\int_{\G_{k}}}
\newcommand{\iGm} {\int_{\G_{m}}}
\newcommand{\iGN} {\int_{\GN}}
\newcommand{\iGD} {\int_{\GD}}
\newcommand{\iGp} {\int_{\G_{\! p}}}
\newcommand{\iGpm} {\int_{\G^{-}_{\! p}}}
\newcommand{\iGpp} {\int_{\G^{+}_{\! p}}}
\newcommand{\iGs} {\int_{\G_{s}}}
\newcommand{\iGst} {\int_{\G^{\star}}}
\newcommand{\iGte}{\int_{\Gte}}
\newcommand{\iGt}{\int_{\tilG}}
\newcommand{\iGu} {\int_{\G_{\! u}}}

%  Integrales avec S

\newcommand{\idS} {\int_{\ddS}}
\newcommand{\ig}{\int_{\gamma}}
\newcommand{\iSb}{\int_{S(b)}}
\newcommand{\iSc}{\int_{\Sc}}
\newcommand{\iScm}{\int_{\Sc^{-}}}
\newcommand{\iScp}{\int_{\Sc^{+}}}
\newcommand{\iSD}{\int_{\SD}}
\newcommand{\iSf}{\int_{S_F}}
\newcommand{\iS}{\int_{S}}
\newcommand{\iSh}{\int_{\widehat{S}}}
\newcommand{\iSm}{\int_{\Sm}}
\newcommand{\iSN}{\int_{\SN}}
\newcommand{\iSoD}{\int_{\SoD}}
\newcommand{\iSo}{\int_{\So}}
\newcommand{\iSoN}{\int_{\SoN}}
\newcommand{\iSp}{\int_{\Sp}}
\newcommand{\iSpm}{\int_{\Sp^{m}}}
\newcommand{\iSq}{\int_{\Sq}}
\newcommand{\iSs}{\int_{\Ss}}
\newcommand{\iStc}{\int_{\tilS_{c}}}
\newcommand{\iStcm}{\int_{\tilS_{c}^{-}}}
\newcommand{\iStcp}{\int_{\tilS_{c}^{+}}}
\newcommand{\iSt}{\int_{S_{T}}}
\newcommand{\iStq}{\int_{\tilS_{q}}}
\newcommand{\iStt}{\int_{\tilS_{T}}}
\newcommand{\iStu}{\int_{\tilS_{u}}}
\newcommand{\iSu}{\int_{\Su}}
\newcommand{\iSum}{\int_{\Su^{m}}}
\newcommand{\iSxi}{\int_{\Sxi}}
\newcommand{\itilS}{\int_{\tilde{S}}}

%  Integrales avec epsilon

\newcommand{\iCe} {\int_{\Ce}}
\newcommand{\ice} {\int_{\ce}}
\newcommand{\iDeps} {\int_{\Deps}}
\newcommand{\idOe}{\int_{\dOe}}
\newcommand{\idOes}{\int_{(\dOe)+\se}}
\newcommand{\idSe} {\int_{\ddS_{\varepsilon}}}
\newcommand{\iee} {\int_{\eee}}
\newcommand{\iGee} {\int_{\Gee}}
\newcommand{\iGes} {\int_{\Ges}}
\newcommand{\iOcOe}{\int_{\OOc-\OOe}}
\newcommand{\iodGe} {\oint_{\dGe}}
\newcommand{\iOee}{\int_{\Oee}}
\newcommand{\iOe}{\int_{\Oe}}
\newcommand{\iOpOe}{\int_{\OOp-\OOe}}
\newcommand{\ise} {\int_{\se}}
\newcommand{\iSe}{\int_{\Se}}
\newcommand{\iSex}{\int_{\Se(x)}}

%  Integrales, autres

\newcommand{\iB}{\int_{B}}
\newcommand{\iBex}{\int_{\Bex}}
\newcommand{\iBst} {\int_{B^{\star}}}
\newcommand{\iC}{\int_{C}}
\newcommand{\iDDe}{\int_{\Delta_{e}}}
\newcommand{\idD} {\int_{\partial D}}
\newcommand{\idE}{\int_{\dE}}
\newcommand{\iDe}{\int_{\Delta^{(e)}}}
\newcommand{\iDel}{\int_{\Delta}}
\newcommand{\iDex}{\int_{\Dex}}
\newcommand{\iD}{\int_{D}}
\newcommand{\iEEe}{\int_{E_{e}}}
\newcommand{\iEe}{\int_{E^{(e)}}}
\newcommand{\iE}{\int_{E}}
\newcommand{\iM} {\int_{M}}
\newcommand{\iR} {\int_{\RR}}
\newcommand{\iT}{\int_{0}^{T}}
\newcommand{\iV}{\int_{V}}
\newcommand{\iVcal}{\int_{\Vcal}}
\newcommand{\idV}{\int_{\partial V}}
\newcommand{\oidse} {\oint_{\dse}}
\newcommand{\oidS} {\oint_{\ddS}}

%  ------------------------------------------------
%  Cauchy Principal Value and Finite Part Integrals
%  ------------------------------------------------

%  preliminaires

 \newlength{\meno}
 \newlength{\integrale}
 \newlength{\trattino}
 \newlength{\integralegrande}
 \newlength{\uguale}
 \newlength{\ugualegrande}

 \settowidth{\meno}{\mbox{$-$}}
 \settowidth{\trattino}{\mbox{--}}
 \settowidth{\uguale}{\mbox{$=$}}
 \settowidth{\ugualegrande}{\mbox{$=$}}
 \settowidth{\integrale}{\mbox{$\int$}}
 \settowidth{\integralegrande}{\mbox{$\displaystyle\int$}}

 \addtolength{\trattino}{\integrale}
 \addtolength{\meno}{\integralegrande}
 \addtolength{\uguale}{\integrale}
 \addtolength{\ugualegrande}{\integralegrande}

%  definitions

\newcommand{\cpv}[1]{%
 \mbox{--}\mbox{\hspace*{-0.5\trattino}}\mbox{$\int_{#1}$}}
\newcommand{\cpvg}[1]{%
 \mbox{$-$}\mbox{\hspace{-0.5\meno}}\mbox{$\displaystyle\int_{#1}$}}
\newcommand{\fp}[1]{%
 \mbox{$=$}\mbox{\hspace*{-0.5\trattino}}\mbox{$\int_{#1}$}}
\newcommand{\fpg}[1]{%
 \mbox{$=$}\mbox{\hspace{-0.5\meno}}\mbox{$\displaystyle\int_{#1}$}}
\newcommand{\CPV}[2]{%
 \mbox{--}\mbox{\hspace{-0.5\trattino}}\mbox{$\int_{#1}^{#2}$}}
\newcommand{\CPVG}[2]{%
 \mbox{$-$}\mbox{\hspace{-0.5\meno}}\mbox{$\displaystyle\int_{#1}^{#2}$}}
\newcommand{\FP}[2]{%
 \mbox{$=$}\mbox{\hspace{-0.5\uguale}}\mbox{$\int_{#1}^{#2}$}}
\newcommand{\FPG}[2]{%
 \mbox{$=$}\mbox{\hspace{-0.5\ugualegrande}}\mbox{$\displaystyle\int_{#1}^{#2}$}}

%
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

\newcommand{\Gcalb}{\bar{\mathcal{G}}}
\newcommand{\Hcalb}{\bar{\mathcal{H}}}
\newcommand{\Lcalb}{\bar{\mathcal{L}}}
\newcommand{\Mcalb}{\bar{\mathcal{M}}}
\newcommand{\Wcalb}{\overline{\Wcal}}

\newcommand{\Lcalh}{\hat{\mathcal{L}}}
\newcommand{\Zcalh}{\hat{\mathcal{Z}}}
\newcommand{\Zcals}{\mathcal{Z}^{\star}}

\newcommand{\FcalT}{\widetilde{\mathcal{F}}}
%
\newcommand{\AS}{\text{\boldmath $\mathcal{A}$}}
\newcommand{\BS}{\ensuremath{\mbox{\boldmath $\mathcal{B}$}}}
\newcommand{\ASR}{\ensuremath{\mbox{\boldmath $\Rmath{\mathcal{A}}$}}}
\newcommand{\BSR}{\ensuremath{\mbox{\boldmath $\Rmath{\mathcal{B}}$}}}
\newcommand{\CS}{\text{\boldmath $\mathcal{C}$}}
\newcommand{\CSt}{\widetilde{\CS}}
\newcommand{\CSR}{\ensuremath{\mbox{\boldmath $\Rmath{\mathcal{C}}$}}}
\newcommand{\DS}{\mbox{\boldmath $\mathcal{D}$}}
\newcommand{\DSR}{\ensuremath{\mbox{\boldmath $\Rmath{\mathcal{D}}$}}}
\newcommand{\ES}{\ensuremath{\mbox{\boldmath $\mathcal{E}$}}}
\newcommand{\FS}{\ensuremath{\mbox{\boldmath $\mathcal{F}$}}}
\newcommand{\GS}{\mbox{\boldmath $\mathcal{G}$}}
\newcommand{\GSR}{\ensuremath{\mbox{\boldmath $\Rmath{\mathcal{G}}$}}}
\newcommand{\GSB}{\ensuremath{\mbox{\boldmath $\Bmath{\mathcal{G}}$}}}
\newcommand{\HS}{\mbox{\boldmath $\mathcal{H}$}}
\newcommand{\IS}{\mbox{\boldmath $\mathcal{I}$}}
\newcommand{\ISt}{\widetilde{\IS}}
\newcommand{\JS}{\mbox{\boldmath $\mathcal{J}$}}
\newcommand{\KS}{\mbox{\boldmath $\mathcal{K}$}}
\newcommand{\LS}{\mbox{\boldmath $\mathcal{L}$}}
\newcommand{\MS}{\mbox{\boldmath $\mathcal{M}$}}
\newcommand{\NS}{\mbox{\boldmath $\mathcal{N}$}}
\Newcommand{\PS}{\mbox{\boldmath $\mathcal{P}$}}
\newcommand{\QS}{\mbox{\boldmath $\mathcal{Q}$}}
\renewcommand{\SS}{\ensuremath{\mbox{\boldmath $\mathcal{S}$}}}
\newcommand{\RS}{\ensuremath{\mbox{\boldmath $\mathcal{R}$}}}
\newcommand{\TS}{\ensuremath{\mbox{\boldmath $\mathcal{T}$}}}
\newcommand{\US}{\ensuremath{\mbox{\boldmath $\mathcal{U}$}}}
\newcommand{\VS}{\text{\boldmath $\Vcal$}}
\newcommand{\WS}{\mbox{\boldmath $\Wcal$}}
\newcommand{\XS}{\mbox{\boldmath $\Xcal$}}
\newcommand{\XSt}{\widetilde{\XS}}
\newcommand{\YS}{\mbox{\boldmath $\Ycal$}}
\newcommand{\ZS}{\mbox{\boldmath $\Zcal$}}

\newcommand{\Cx}{\Ccal_{x}}
\newcommand{\Cxi}{\Ccal_{\xi}}
\newcommand{\Cxl}{\Ccal_{x}^{(\ell)}}
\newcommand{\Cxil}{\Ccal_{\xi}^{(\ell)}}
\newcommand{\Cxlb}{\Ccal_{x}^{(\lbar)}}
\newcommand{\Cxilb}{\Ccal_{\xi}^{(\lbar)}}
\newcommand{\Cxlp}{\Ccal_{x}^{(\ell+1)}}
\newcommand{\Cxilp}{\Ccal_{\xi}^{(\ell+1)}}
\newcommand{\Cxilm}{\Ccal_{\xi}^{(\ell-1)}}

\newcommand{\FcalN}{\Fcal\Nsub}
\newcommand{\VcalN}{\Vcal\Nsub}
\newcommand{\VcalD}{\Vcal\Dsub}
\newcommand{\VcalDz}{\Vcal\Dsub{}_{,0}}
\newcommand{\VcalNz}{\Vcal\Nsub{}_{,0}}
\newcommand{\Vcalz}{\Vcal_{0}}
\newcommand{\WcalN}{\Wcal\Nsub}
\newcommand{\WcalD}{\Wcal\Dsub}
\newcommand{\WcalDz}{\Wcal\Dsub{}_{,0}}
\newcommand{\WcalNz}{\Wcal\Nsub{}_{,0}}
\newcommand{\Wcalz}{\Wcal_{0}}

%  ------------------------
%  NOTATIONS ELEMENTS FINIS
%  ------------------------

\newcommand{\CA}{\mbox{CA}}
\newcommand{\dxit}{\,{\rm d}\bfxit}
\newcommand{\Er}{E_{r}}
\newcommand{\Jda}{J(\bfa) \,{\rm d}\bfa}
\newcommand{\Jdap}{J(\bfa') \,{\rm d}\bfa'}
\newcommand{\Jdeta}{\Jeta \deta}
\newcommand{\Jdxi}{\Jxi \dxi}
\newcommand{\Jdxit}{\Jxit \dxit}
\newcommand{\Jeta}{J(\bfeta)}
\newcommand{\Jxi}{J(\bfxi)}
\newcommand{\Jxit}{J(\bfxit)}
\newcommand{\Me}{M_{e}}    
\newcommand{\NBEM}{N_{\text{BEM}}}
\newcommand{\NB}{N\Bsub}
\Newcommand{\NC} {{\rm NC}}
\newcommand{\NEL} {{\rm NEL}}
\newcommand{\Ne}{\rmN_{e}}
\newcommand{\NE}{\rmN\Esub}
\Newcommand{\NF}{\rmN\Fsub}
\newcommand{\nF}{n\Fsub}
\renewcommand{\NG}{N_{G}}
\newcommand{\NI}{N\Isub}
\newcommand{\Nn}{N_{N}}
\Newcommand{\NN}{\rmN\Nsub}

%  ------------
%  DIVERS MATHS
%  ------------

%  Produits contractes

\newcommand{\tip}{\hspace*{1pt}\smash{\raisebox{-0.4ex}{\scalebox{1.4}{$\begin{gathered}\cdot\\[-3ex]\cdot\hspace*{-0.1pt}\cdot\end{gathered}$}}}\hspace*{2pt}}
\newcommand{\ip} {\!\Cdot\!}
\newcommand{\dip} {\! :\!}
\newcommand{\sip} {\! \cdot\!}
\newcommand{\pip} {\! :\hspace*{-3pt} \cdot\hspace*{-3pt} :\!}
\newcommand{\qip} {\!::\!}
%\newcommand{\tip}{\!:\hspace*{-0.555em}\raisebox{-0.06ex}{$\cdot$}\hspace*{0.1em}}
\newcommand{\dotp}{\raisebox{1pt}{\hspace*{1pt}\scalebox{0.45}{$\bullet$}}\hspace*{1pt}}
\newcommand{\Cdot}{\raisebox{1pt}{\hspace*{1pt}\scalebox{0.6}{$\bullet$}}\hspace*{1pt}}

%  Inverses

\newcommand{\pdemi} {\mbox{$\frac{1}{2}$}}
\newcommand{\tdemi} {\tfrac{1}{2}}
\newcommand{\ttiers} {\tfrac{1}{3}}
\newcommand{\tquart} {\tfrac{1}{4}}
\newcommand{\demi} {\inv{2}}
\newcommand{\tiers} {\inv{3}}
\newcommand{\quart} {\inv{4}}
\newcommand{\huitieme} {\inv{8}}

%  TD, asymptotique

\newcommand{\Acalr}{\mathcal{A}_{\incsize}}
\newcommand{\Ar}{A_{\incsize}}
\newcommand{\ar}{a_{\incsize}}
\newcommand{\ars}{a^{\star}_{\incsize}}
\newcommand{\ASr}{\AS_{\incsize}}
% \newcommand{\betaBB}{\beta_{B}}
\newcommand{\betaB}{\beta_{\Bcal}}
\newcommand{\betar}{\beta_{\incsize}}
\newcommand{\bfdelrb}{\overline{\bfdel}_{\incsize}}
\newcommand{\bfdelr}{\bfdel_{\incsize}}
\newcommand{\bffz}[1][]{\bff^{#1}_{\xZ}}
\newcommand{\bfgar}{\bfga_{\incsize}}
\newcommand{\bfgz}[1][]{\bfg^{#1}_{\xZ}}
\newcommand{\bfGz}[1][]{\bfG^{#1}_{\xZ}}
\newcommand{\bfgzh}[1][]{\bfgh^{#1}_{\xZ}}
\newcommand{\bfpr}{\bfp_{\incsize}}
\newcommand{\bfqr}{\bfq_{\incsize}}
\newcommand{\bfrr}{\bfr_{\incsize}}
\newcommand{\bfFr}{\bfF_{\incsize}}
\newcommand{\bfJr}{\bfJ_{\incsize}}
\newcommand{\bfKr}{\bfK_{\incsize}}
\newcommand{\bfLr}{\bfL_{\incsize}}
\newcommand{\bfPr}{\bfP_{\incsize}}
\newcommand{\bfPhr}{\bfPh_{\incsize}}
\newcommand{\bfPsr}{\bfPs_{\incsize}}
\newcommand{\bfQr}{\bfQ_{\incsize}}
\newcommand{\bfRr}{\bfR_{\incsize}}
\newcommand{\bftr}{\bft_{\incsize}}
\newcommand{\bfwr}{\bfw_{\incsize}}
\newcommand{\bfyr}{\bfy_{\incsize}}
\newcommand{\bfzr}{\bfz_{\incsize}}
\newcommand{\bfUBc}{\bfU_{\Bcal}}
\newcommand{\bfuBc}{\bfu_{\Bcal}}
\newcommand{\bfur}{\bfu_{\incsize}}
\newcommand{\bfurDb}{\bfub{}_{\incsize}\Dsup}
\newcommand{\bfurD}{\bfu_{\incsize}\Dsup}
\newcommand{\bfurDN}{\bfu_{\incsize}\DNsupc}
\newcommand{\bfurNb}{\bfub{}_{\incsize}\Nsup}
\newcommand{\bfurN}{\bfu_{\incsize}\Nsup}
\newcommand{\bfurR}{\Rmath{\bfuR_{\incsize}}}
\newcommand{\bfurt}{\tilde{\bfu}_{\incsize}}
\newcommand{\bfutrdd}{\ddot{\tilde{\bfu}}^{\incsize}}
\newcommand{\bfutrd}{\dot{\tilde{\bfu}}^{\incsize}}
\newcommand{\bfutr}{\tilde{\bfu}^{\incsize}}
\newcommand{\bfvBc}{\bfv_{\Bcal}}
\newcommand{\bfvrb}{\overline{\bfv}_{\incsize}}
\newcommand{\bfvr}{\bfv_{\incsize}}
\newcommand{\bfVr}{\bfV_{\incsize}}
\newcommand{\bfvrDb}{\bfvb{}_{\incsize}\Dsup}
\newcommand{\bfvrD}{\bfv_{\incsize}\Dsup}
\newcommand{\bfvrDN}{\bfv_{\incsize}\DNsupc}
\newcommand{\bfvrNb}{\bfvb{}_{\incsize}\Nsup}
\newcommand{\bfvrN}{\bfv_{\incsize}\Nsup}
\newcommand{\bfvrt}{\tilde{\bfv}_{\incsize}}
\newcommand{\bfvrT}{\widetilde{\bfv}_{\incsize}}
\newcommand{\bfxir}{\bfxi/\incsize}
\newcommand{\bfxS} {\bfx\ssub}
\newcommand{\bfxZ} {\bfz}
\newcommand{\Br} {B_{\incsize}}
\newcommand{\Brb} {\overline{B}_{\incsize}}
\newcommand{\Brz} {B_{\incsize,\xZ}}
\newcommand{\brzz}{b_{\incsize,\xZ}}
\newcommand{\dBrz} {\partial\Brz}
\newcommand{\DDr} {D_{\incsize}}
\newcommand{\DDrz} {D_{\incsize,\bfxZ}}
\newcommand{\dOOrz}{\dO_{\incsize,\bfxZ}}
\newcommand{\delr}{\delta_{\incsize}}
\newcommand{\delrb}{\bar{\delta}_{\incsize}}
\newcommand{\DSr}{\DS_{\incsize}}
\newcommand{\er}{e_{\incsize}}
\newcommand{\erz} {e_{\incsize,\xZ}}
% \newcommand{\etaBB}{\eta_{B}}
\newcommand{\etaB}{\eta_{\Bcal}}
\newcommand{\etaz}{\eta_{\xZ}}
\newcommand{\etar}{\eta_{\incsize}}
\newcommand{\Fr} {F_{\incsize}}
\newcommand{\Fcalr} {\Fcal_{\incsize}}
\newcommand{\gamr}{\gamma^{\incsize}}
\newcommand{\GcalB}{\overline{\Gcal}{}}
\newcommand{\GcalBr}{\overline{\Gcal}_{\incsize}}
\newcommand{\GcalBCr}{\overline{\Gcal}{}_{\incsize}\csup}
% \newcommand{\GcalB}{\mathcal{G}_{\Bcal}}
% \newcommand{\GcalBCr}{\mathcal{G}_{\Bcal,\incsize}\csup}
\newcommand{\Gcalr}{\mathcal{G}_{\incsize}}
\newcommand{\gka} {\gamma k\incsize}
\newcommand{\gkr} {\gamma kr}
\newcommand{\Gr} {\G_{\!\incsize}}
\newcommand{\HcalB}{\overline{\Hcal}{}}
\newcommand{\HcalBr}{\overline{\Hcal}_{\incsize}}
\newcommand{\HcalBCr}{\overline{\Hcal}{}_{\incsize}\csup}
% \newcommand{\HcalB}{\mathcal{H}_{\Bcal}}
% \newcommand{\HcalBCr}{\mathcal{H}_{\Bcal,\incsize}\csup}
\newcommand{\Hcalr}{\mathcal{H}_{\incsize}}
\newcommand{\iBcal}{\int_{\Bcal}}
\newcommand{\iBcalp}{\int_{\Bcal'}}
\newcommand{\iBr} {\int_{\Br}}
\newcommand{\iBrp} {\int_{\Br'}}
\newcommand{\iBrm} {\int_{\Br^{(m)}}}
\newcommand{\iBrz} {\int_{\Brz}}
\newcommand{\ibrz}{\int_{\brzz}}
\newcommand{\idOcal}{\int_{\partial\Ocal}}
\newcommand{\idBcal}{\int_{\partial\Bcal}}
\newcommand{\idBrz}{\int_{\partial\Brz}}
\newcommand{\idvrz}{\int_{\partial\vrz}}
\newcommand{\iDcal}{\int_{\Dcal}}
\newcommand{\iGr} {\int_{\Gr}}
\newcommand{\incsize}{\eps}
\newcommand{\inczer}{\incsize\to0}
\newcommand{\iOcal}{\int_{\Ocal}}
\newcommand{\iOrz}{\int_{\OOrz}}
\newcommand{\iScal}{\int_{\Scal}}
\newcommand{\iSscal}{\int_{\Scal^{\star}}}
\newcommand{\isfS}{\int_{\sfS}}
\newcommand{\isfSr}{\int_{\incsize\sfS}}
\newcommand{\iSrz}{\int_{\Srz}}
\newcommand{\isrz}{\int_{\srz}}
\newcommand{\iUrz}{\int_{\Urz}}
%\newcommand{\iVcal}{\int_{\Vcal}}
\newcommand{\ivrz}{\int_{\vrz}}
\newcommand{\DJr}{\Delta J_{\incsize}}
\newcommand{\DKr}{\Delta K_{\incsize}}
\newcommand{\DLr}{\Delta L_{\incsize}}
\newcommand{\Jr}{J_{\incsize}}
\newcommand{\ka} {k\incsize}
\newcommand{\kappar}{\kappa_{\incsize}}
\newcommand{\Kcalr}{\Kcal_{\incsize}}
\newcommand{\kr}{k_{\incsize}}
\newcommand{\Kr}{K_{\incsize}}
\newcommand{\LcalB}{\mathcal{L}_{\Bcal}}
\newcommand{\LcalBr}{\overline{\Lcal}{}_{\incsize}}
\newcommand{\LcalBC}[1][]{\overline{\Lcal}{}\csup_{#1}}
\newcommand{\LcalBCr}{\LcalBr\csup}
\newcommand{\Lcalr}{\mathcal{L}_{\incsize}}
\newcommand{\Lr}{L_{\incsize}}
\newcommand{\LSB}{\LS_{\Bcal}}
\newcommand{\LSr}{\LS_{\incsize}}
\newcommand{\McalB}{\overline{\Mcal}{}}
% \newcommand{\McalB}{\mathcal{M}_{\Bcal}}
\newcommand{\Mcalr}{\Mcal_{\incsize}}
\newcommand{\NcalB}{\overline{\Ncal}{}}
% \newcommand{\NcalB}{\mathcal{N}_{\Bcal}}
\newcommand{\OOr}{\Omega_{\incsize}}
\newcommand{\OOrz}{\Omega_{\incsize,\bfxZ}}
\newcommand{\peps}{p^{\incsize}}
\newcommand{\pB} {p_{B}}
\newcommand{\phir}{\phi_{\incsize}}
\newcommand{\pr}{p^{\incsize}}
\newcommand{\PViGb} {\dashint_{\Gb}}
\newcommand{\PViGr} {\dashint_{\Gr(\xZ)}}
\newcommand{\qB} {q_{B}}
\newcommand{\qeps}{q^{\incsize}}
\newcommand{\qr}{q^{\incsize}}
\newcommand{\sfvrz}{\sfv_{\incsize,\xZ}}
\newcommand{\Sr} {S_{\incsize}}
\newcommand{\Sscal} {\Scal^{\star}}
\newcommand{\Srz} {S_{\incsize,\bfxZ}}
\newcommand{\srz} {s_{\incsize,\xZ}}
\newcommand{\srzT} {\tils_{\incsize,\xZ}}
\newcommand{\tilvrz}{\tilv_{\incsize,\xZ}}
%\newcommand{\uBB} {u_{B}}
\newcommand{\uBB} {u^{B}}
\newcommand{\uB} {u_{\Bcal}}
\newcommand{\UB}[1][]{U^{#1}_{\Bcal}}
\newcommand{\UBH}[1][]{\widehat{U}^{#1}_{\Bcal}}
\newcommand{\UcalB}{\mathcal{U}_{\Bcal}}
\newcommand{\ueps}{u^{\incsize}}
\newcommand{\Ueps}{U^{\incsize}}
\newcommand{\uzz}{u_{\xZ}}
\newcommand{\uzh}{\uh_{\xZ}}
\newcommand{\UIrm}{U^{\incsize-}\Isub}
\newcommand{\UIrp}{U^{\incsize+}\Isub}
\newcommand{\UIr}{U^{\incsize}\Isub}
\newcommand{\Um}{U_{0}}
\newcommand{\UOrm}{U^{\incsize-}\Osub}
\newcommand{\UOrp}{U^{\incsize+}\Osub}
\newcommand{\UOr}{U^{\incsize}\Osub}
\newcommand{\Up}{U_{2}}
\newcommand{\urb}{\ubar{}^{\incsize}}
\newcommand{\urDb}{\ubar{}_{\incsize}\Dsup}
\newcommand{\urdd}{\ddot{u}^{\incsize}}
\newcommand{\urd}{\dot{u}^{\incsize}}
\newcommand{\urDN}{u_{\incsize}\DNsupc}
\newcommand{\urD}{u_{\incsize}\Dsup}
\newcommand{\urNb}{\ubar{}_{\incsize}\Nsup}
\newcommand{\urN}{u_{\incsize}\Nsup}
\newcommand{\ur}{u_{\incsize}}
\newcommand{\Ur}{U^{\incsize}}
%\newcommand{\Ur}{U_{\incsize}}
\newcommand{\Urz}{U_{\incsize,\bfxZ}}
\newcommand{\utrdd}{\ddot{\tilde{u}}^{\incsize}}
\newcommand{\utrd}{\dot{\tilde{u}}^{\incsize}}
\newcommand{\utr}{\tilde{u}^{\incsize}}
\newcommand{\urt}{\tilde{u}_{\incsize}}
\newcommand{\vBB} {v_{B}}
\newcommand{\vB} {v_{\Bcal}}
\newcommand{\veps}{v^{\incsize}}
%\newcommand{\vrb}{\vbar{}^{\incsize}}
\newcommand{\vrDb}{\vbar{}_{\incsize}\Dsup}
\newcommand{\vrd}{\dot{v}^{\incsize}}
\newcommand{\vrD}{v^{\incsize}\Dsub}
\newcommand{\Vrm}{V^{\incsize}_{0}}
\newcommand{\vrNb}{\vbar{}_{\incsize}\Nsup}
\newcommand{\vrN}{v^{\incsize}\Nsub}
\newcommand{\Vrp}{V^{\incsize}_{2}}
\newcommand{\vrb}{\overline{v}{}_{\incsize}}
\newcommand{\vrr}{\mathring{v}{}_{\incsize}}
\newcommand{\vrh}{\hat{v}{}_{\incsize}}
\newcommand{\vrT}{\widetilde{v}{}_{\incsize}}
\newcommand{\vrt}{\tilde{v}{}^{\incsize}}
\newcommand{\vr}{v_{\incsize}}
\newcommand{\Vr}{V^{\incsize}_{1}}
\newcommand{\Vrz}{V_{\incsize,\xZ}}
\newcommand{\vrz}{v_{\incsize,\xZ}}
\newcommand{\vrzz}{v_{\incsize_0,\xZ}}
\newcommand{\vrzT}{\tilv_{\incsize,\xZ}}
\newcommand{\wrd}{\dot{w}^{\incsize}}
\newcommand{\wrDN}{w_{\incsize}\DNsupc}
\newcommand{\wrD}{w_{\incsize}\Dsup}
\newcommand{\Wrm}{W^{\incsize}_{0}}
\newcommand{\wrN}{w_{\incsize}\Nsup}
\newcommand{\Wrp}{W^{\incsize}_{2}}
\newcommand{\Wr}{W^{\incsize}_{1}}
\newcommand{\XB}[1][]{X^{#1}_{\Bcal}}
\newcommand{\xZ} {z}
\newcommand{\YB}[1][]{Y^{#1}_{\Bcal}}
\newcommand{\YBh}[1][]{\widehat{Y}{}^{#1}_{\!\!\Bcal}}
\newcommand{\ZB}[1][]{Z^{#1}_{\Bcal}}
\newcommand{\Zcalr}{\Zcal_{\incsize}}
\renewcommand{\wr}{w^{\incsize}}

\newcommand{\cs}{c^{\star}}
\newcommand{\rhos}{\rho^{\star}}
\newcommand{\mus}{\mu^{\star}}
\newcommand{\nus}{\nu^{\star}}
\newcommand{\bfmur}{\bfmu_{\incsize}}
\newcommand{\mur}{\mu_{\incsize}}
\newcommand{\epsra}[1][a]{\varepsilon_{\text{r}#1}}
\newcommand{\mura}[1][a]{\mu_{\text{r}#1}}
\newcommand{\bfrhvr}{\bfrhv_{\incsize}}
\newcommand{\ccr}{c_{\incsize}}
\newcommand{\rhor}{\rho_{\incsize}}
\newcommand{\rhvr}{\varrho_{\incsize}}
\newcommand{\CSr}{\CS_{\incsize}}
\newcommand{\CSB}{\CS_{\Bcal}}
\newcommand{\CSBt}{\widetilde{\CS}{}_{\Bcal}}
\newcommand{\Ccalr}{\Ccal_{\incsize}}
\newcommand{\CSs} {\CS^{\star}}
\newcommand{\CSst} {\widetilde{\CS}{}^{\star}}
\newcommand{\OOs} {\OO^{\star}}
\newcommand{\mmr}{m_{\incsize}}
\newcommand{\nnr}{n_{\incsize}}
\newcommand{\kappas}{\kappa^{\star}}

\newcommand{\WNz}{W_{0}\Nsup}
% \newcommand{\WDz}{W_{0}\Dsup}
\newcommand{\WN}{W\Nsup}
\newcommand{\WD}{W\Dsup}
\newcommand{\Fo}{F_{\text{o}}}
\newcommand{\Fno}{F_{\text{no}}}
\newcommand{\Go}{S_{\text{o}}}
\newcommand{\Gno}{S_{\text{no}}}

%  Divers

\newcommand{\dummy}{\mbox{\,\raisebox{0.1ex}{\scalebox{0.4}{\textbullet}}\,}}
\newcommand{\defeq}{\stackrel{\text{def}}{=}}
%\newcommand{\sig}{\sigma}
\newcommand{\eps}{\varepsilon}
\newcommand{\NU} {{\rm NU}}
\newcommand{\oo}{\omega}
\newcommand{\pD}{p\Dsup}
\newcommand{\phiDp}{\phiD{}_{,p}}
\newcommand{\phiDpp}{\phiD{}_{,pp}}
\newcommand{\phiD}{\varphi\Dsub}
\newcommand{\phiNu}{\phiN{}_{,u}}
\newcommand{\phiNuu}{\phiN{}_{,uu}}
\newcommand{\phiN}{\varphi\Nsub}
\newcommand{\pst}{p^{\star}}
\newcommand{\qD}{q\Dsup}
\newcommand{\td}{t^{\scriptscriptstyle D\hspace{-1pt}}}
\newcommand{\thm}{\theta_{\nu}}
\newcommand{\thn}{\theta_{n}}
\newcommand{\ths}{\theta_{s}}
\newcommand{\tn}{t_{n}}
\newcommand{\tnh}{\hatt_{n}}
\newcommand{\udd}{\dot{u}{}^{\scriptscriptstyle D\hspace{-1pt}}}
\newcommand{\ud}{u^{\scriptscriptstyle D\hspace{-1pt}}}
\newcommand{\uF}{u\Fsup}
\newcommand{\uG}{u_{\G}}
\newcommand{\uhd}{\dot{\uh}}
\newcommand{\ust}{u^{\star}}
% \newcommand{\xib} {\bar{\xi}}
\newcommand{\GkR} {G_{k,}{}\Rsub}

%  Composantes de contraintes et déformations

\newcommand{\xir}{u_{r}}
% \newcommand{\xit}{u_{\theta}}

\newcommand{\sigrr}{\sigma_{rr}}
\newcommand{\sigrt}{\sigma_{r\theta}}
\newcommand{\sigrz}{\sigma_{rz}}
\newcommand{\sigtz}{\sigma_{\theta z}}
\newcommand{\sigtt}{\sigma_{\theta\theta}}
\newcommand{\sigpp}{\sigma_{\varphi\varphi}}
\newcommand{\sigxx}{\sigma_{xx}}
\newcommand{\sigyy}{\sigma_{yy}}
\newcommand{\sigzz}{\sigma_{zz}}
\newcommand{\sigxy}{\sigma_{xy}}
\newcommand{\sigxz}{\sigma_{xz}}
\newcommand{\sigyz}{\sigma_{yz}}

\newcommand{\epsrr}{\varepsilon_{rr}}
\newcommand{\epsrt}{\varepsilon_{r\theta}}
\newcommand{\epsrz}{\varepsilon_{rz}}
\newcommand{\epstz}{\varepsilon_{\theta z}}
\newcommand{\epstt}{\varepsilon_{\theta\theta}}
\newcommand{\epspp}{\varepsilon_{\varphi\varphi}}
\newcommand{\epsxx}{\varepsilon_{xx}}
\newcommand{\epsyy}{\varepsilon_{yy}}
\newcommand{\epszz}{\varepsilon_{zz}}
\newcommand{\epsxy}{\varepsilon_{xy}}
\newcommand{\epsxz}{\varepsilon_{xz}}
\newcommand{\epsyz}{\varepsilon_{yz}}

%  Environnements

%\newenvironment{cmatrix}{\left\{\begin{matrix}}{\end{matrix}\right\}}
%  -----------------------------------
%  Textual subscripts and superscripts
%  -----------------------------------

\newcommand{\csup}{^{\text{\scriptsize c}}}
\newcommand{\Csup}{^{\text{\tiny C}}}
\newcommand{\Dsup}{^{\text{\tiny D}}}
\newcommand{\dsup}{^{\text{\scriptsize d}}}
\newcommand{\esup}{^{\text{\scriptsize e}}}
\newcommand{\Esup}{^{\text{\tiny E}}}
\newcommand{\Fsup}{^{\text{\tiny F}}}
\newcommand{\Gsup}{^{\text{\tiny G}}}
\newcommand{\Hsup}{^{\text{\tiny H}}}
\newcommand{\isup}{^{\text{\tiny i}}}
\newcommand{\Isup}{^{\text{\tiny I}}}
\newcommand{\Jsup}{^{\text{\tiny J}}}
\newcommand{\Lsup}{^{\text{\tiny L}}}
\newcommand{\msup}{^{\text{\scriptsize m}}}
\newcommand{\Nsup}{^{\text{\tiny N}}}
\newcommand{\Osup}{^{\text{\tiny O}}}
\newcommand{\psup}{^{\text{\scriptsize p}}}
\newcommand{\Psup}{^{\text{\tiny P}}}
\newcommand{\Rsup}{^{\text{\tiny R}}}
\newcommand{\Ssup}{^{\text{\tiny S}}}
\newcommand{\ssup}{^{\text{s}}}
\newcommand{\Tsup}{^{\text{\tiny T}}}
\newcommand{\Vsup}{^{\text{\tiny V}}}
\newcommand{\Zsup}{^{\text{\tiny Z}}}
\newcommand{\starT}{^{\star\text{\tiny T}}}

\newcommand{\Asub}{_{\text{\tiny A}}}
\newcommand{\Bsubp}{_{\text{\tiny B'}}}
\newcommand{\Bsub}{_{\text{\tiny B}}}
\newcommand{\bsub}{_{\text{\scriptsize b}}}
\newcommand{\Csubp}{_{\text{\tiny C'}}}
\newcommand{\csub}{_{\text{\scriptsize c}}}
\newcommand{\Csub}{_{\text{\tiny C}}}
\newcommand{\dsub}{_{\text{d}}}
\newcommand{\Dsub}{_{\text{\tiny D}}}
\newcommand{\esub}{_{\text{\scriptsize e}}}
\newcommand{\Esub}{_{\text{\tiny E}}}
\newcommand{\Fsub}{_{\text{\tiny F}}}
\newcommand{\fsub}{_{\text{\tiny f}}}
\newcommand{\hsub}{_{\text{\scriptsize h}}}
\newcommand{\Hsub}{_{\text{\tiny H}}}
\newcommand{\Isub}{_{\text{\tiny I}}}
\newcommand{\isub}{_{\text{\scriptsize i}}}
\newcommand{\Jsub}{_{\text{\tiny J}}}
\newcommand{\Ksub}{_{\text{\tiny K}}}
%\newcommand{\Lsub}{_{\text{\tiny L}}}
\newcommand{\Lsub}{_{\text{\scriptsize L}}}
\newcommand{\Msub}{_{\text{\tiny M}}}
\newcommand{\Nsub}{_{\text{\tiny N}}}
\newcommand{\osub}{_{\text{o}}}
\newcommand{\Osub}{_{\text{\tiny O}}}
\newcommand{\Psub}{_{\text{\tiny P}}}
\newcommand{\psub}{_{\text{\tiny p}}}
\newcommand{\Qsub}{_{\text{\tiny Q}}}
\newcommand{\rsub}{_{\text{\tiny r}}}
\newcommand{\Rsub}{_{\text{\tiny R}}}
\newcommand{\Ssub}{_{\text{\tiny S}}}
\newcommand{\ssub}{_{\text{s}}}
\newcommand{\tsub}{_{\text{t}}}
\newcommand{\Tsub}{_{\text{\tiny T}}}
%\newcommand{\Usub}{_{\text{\tiny U}}}
\newcommand{\Usub}{_{\text{\scriptsize U}}}
\newcommand{\Vsub}{_{\text{\tiny V}}}
\newcommand{\Wsub}{_{\text{\tiny W}}}
\newcommand{\vsub}{_{\text{\scriptsize v}}}
\newcommand{\Ysub}{_{\text{\tiny Y}}}

\newcommand{\msub}{_{\text{\scriptsize m}}}
\newcommand{\osup}{^{\text{o}}}
\newcommand{\tsup}{^{\text{t}}}

\newcommand{\DDsup}{^{\text{\tiny DD}}}
\newcommand{\DIsup}{^{\text{\tiny DI}}}

\newcommand{\DDsub}{_{\text{\tiny DD}}}
\newcommand{\DNsub}{_{\text{\tiny DN}}}
\newcommand{\DNsubc}{_{\text{\tiny D,N}}}
\newcommand{\DNsupc}{^{\text{\tiny D,N}}}

\newcommand{\ECsub}{_{\text{\tiny EC}}}
\newcommand{\ELsub}{_{\text{\tiny PL}}}

\newcommand{\FFsub}{_{\text{\tiny FF}}}
\newcommand{\FLsub}{_{\text{\tiny FL}}}
\newcommand{\FLsup}{^{\text{\tiny FL}}}
\newcommand{\FMsub}{_{\text{\tiny FM}}}

\newcommand{\IIsub}{_{\text{\tiny II}}}
\newcommand{\IJsub}{_{\text{\tiny IJ}}}
\newcommand{\IKsub}{_{\text{\tiny IK}}}
\newcommand{\ILsub}{_{\text{\tiny IL}}}

\newcommand{\JIsub}{_{\text{\tiny JI}}}
\newcommand{\JJsub}{_{\text{\tiny JJ}}}
\newcommand{\JKsub}{_{\text{\tiny JK}}}
\newcommand{\JLsub}{_{\text{\tiny JL}}}
\newcommand{\JMsub}{_{\text{\tiny JM}}}
\newcommand{\JTsub}{_{\text{\tiny JT}}}

\newcommand{\KKsub}{_{\text{\tiny KK}}}

\newcommand{\LJsub}{_{\text{\tiny LJ}}}
\newcommand{\LFsub}{_{\text{\tiny LF}}}
\newcommand{\LLsub}{_{\text{\tiny LL}}}
\newcommand{\LMsub}{_{\text{\tiny LM}}}
\newcommand{\LTsub}{_{\text{\tiny LT}}}
\newcommand{\LSsub}{_{\text{\tiny LS}}}

\newcommand{\MFsub}{_{\text{\tiny MF}}}
\newcommand{\MLsub}{_{\text{\tiny ML}}}
\newcommand{\MMsub}{_{\text{\tiny MM}}}

\newcommand{\NNsub}{_{\text{\tiny NN}}}

\newcommand{\PLsub}{_{\text{\tiny PL}}}

\newcommand{\RIsub}{_{\text{\tiny RI}}}
\newcommand{\RRsub}{_{\text{\tiny RR}}}
\newcommand{\RSsub}{_{\text{\tiny RS}}}

\newcommand{\SRsub}{_{\text{\tiny SR}}}
\newcommand{\SSsub}{_{\text{\tiny SS}}}

\newcommand{\TTsub}{_{\text{\tiny TT}}}
\newcommand{\TLsub}{_{\text{\tiny TL}}}

\newcommand{\VPsup}{^{\text{\tiny VP}}}

\newcommand{\DNsup}{^{\text{\tiny D,N}}}
\newcommand{\IDsup}{^{\text{\tiny ID}}}
\newcommand{\IIsup}{^{\text{\tiny II}}}
\newcommand{\EPsup}{^{\text{\tiny EP}}}

\newcommand{\IIIsub}{_{\text{\tiny III}}}
\newcommand{\CQMsub}{_{\text{\tiny CQM}}}
\newcommand{\HFAsub}{\ensuremath{_{\text{HFA}}}}

\newcommand{\Approx}{^{\text{approx}}}
\newcommand{\adm}{_{\text{adm}}}
\newcommand{\all}{_{\text{all}}}
\newcommand{\calc}{_{\text{calc}}}
\newcommand{\Calc}{^{\text{calc}}}
\newcommand{\CG}{_{\text{CG}}}
\newcommand{\CM}{_{\text{CM}}}
\newcommand{\comp}{_{\text{comp}}}
\newcommand{\cond}{\text{cond}}
\newcommand{\CPU}{\text{CPU}}
\newcommand{\ddl}{\textsc{ddl}\xspace}
\newcommand{\ddls}{\textsc{ddl}s\xspace}
\newcommand{\dev}{_{\text{dev}}}
\newcommand{\Det}{\text{det}}
\newcommand{\Diag}{\text{diag}}
\newcommand{\Dim}{\text{dim}}
\newcommand{\dof}{\ensuremath{\text{\texttt{dof}}}\xspace}
\newcommand{\eff}{_{\text{eff}}}
\newcommand{\elas}{^{\text{elas}}}
\newcommand{\el}{^{\text{\scriptsize el}}}
\newcommand{\ECE}{_{\text{\tiny ECE}}}
\newcommand{\ECR}{_{\text{\tiny ECR}}}
\newcommand{\EP}{^{\text{\scriptsize ep}}}
\newcommand{\ER}{\text{ER}}
\newcommand{\eq}{_{\text{\scriptsize eq}}}
\newcommand{\Est}{^{\text{est}}}
\newcommand{\est}{_{\text{est}}}
\newcommand{\even}{^{\text{even}}}
\newcommand{\Exact}{^{\text{ex}}}
\newcommand{\exact}{_{\text{ex}}}
\newcommand{\expsup}{^{\text{\scriptsize exp}}}
\newcommand{\ext}{_{\text{ext}}}
\newcommand{\Ext}{^{\text{ext}}}
\newcommand{\glob}{_{\text{glob}}}
\newcommand{\hard}{_{\text{hard}}}
\newcommand{\Int}{_{\text{int}}}
\newcommand{\Irr}{_{\text{irr}}}
\newcommand{\Inc}{^{\text{inc}}}
\newcommand{\inc}{_{\text{inc}}}
\newcommand{\iter}{_{\text{iter}}}
\newcommand{\loc}{_{\text{loc}}}
\newcommand{\LSM}{_{\text{\tiny LSM}}}
\newcommand{\sMax}{_{\text{max}}}
\newcommand{\MAP}{_{\text{MAP}}}
\newcommand{\Max}{^{\text{max}}}
\newcommand{\meas}{_{\text{meas}}}
\newcommand{\sMin}{_{\text{min}}}
\newcommand{\Min}{^{\text{min}}}
\newcommand{\Noise}{^{\text{noise}}}
\newcommand{\obs}{_{\text{obs}}}
\newcommand{\near}{_{\text{near}}}
\newcommand{\Obs}{^{\text{obs}}}
\newcommand{\Out}{^{\text{out}}}
\newcommand{\out}{_{\text{out}}}
\newcommand{\odd}{^{\text{odd}}}
\newcommand{\Opt}{^{\text{opt}}}
\newcommand{\opt}{_{\text{opt}}}
\newcommand{\plas}{^{\text{plas}}}
\newcommand{\Pot}{_{\text{pot}}}
\newcommand{\prior}{_{\text{prior}}}
\newcommand{\Rad}{\ensuremath{^{\text{rad}}}}
\newcommand{\Rel}{^{\text{rel}}}
\newcommand{\Relmax}{^{\text{rel,max}}}
\newcommand{\Reft}{^{\text{Ref}}}
\Newcommand{\Ref}{^{\text{ref}}}
\newcommand{\Reg}{^{\text{reg}}}
\newcommand{\Res}{^{\text{res}}}
\newcommand{\Rev}{^{\text{rev}}}
\Newcommand{\skew}{_{\text{skew}}}
\newcommand{\soft}{_{\text{soft}}}
\newcommand{\Span}{\text{span}}
\newcommand{\sph}{_{\text{sph}}}
\newcommand{\Sym}{^{\text{sym}}}
\newcommand{\sym}{_{\text{sym}}}
\Newcommand{\Tr}{\text{Tr}}
\newcommand{\Th}{^{\text{Th}}}
\newcommand{\therm}{_{\text{th}}}
\newcommand{\true}{_{\text{true}}}
\newcommand{\True}{^{\text{true}}}
\newcommand{\Vect}{\text{Vect}}

%  --------------------------
%  Dirichlet / Neumann
%  --------------------------

\newcommand{\uD} {u\Dsup}
\newcommand{\uN} {u\Nsup}
\newcommand{\VD} {V\Dsup}
\newcommand{\wD} {w\Dsup}
\newcommand{\wN} {w\Nsup}
\newcommand{\uDN} {u\DNsupc}
\newcommand{\wDN} {w\DNsupc}
\newcommand{\uDb} {\ubar{}\Dsup}
\newcommand{\uNb} {\ubar{}\Nsup}
\newcommand{\wDb} {\wbar{}\Dsup}
\newcommand{\wNb} {\wbar{}\Nsup}
\newcommand{\bfuDb} {\bfub{}\Dsup}
\newcommand{\bfuNb} {\bfub{}\Nsup}
\newcommand{\bfuD} {\bfu\Dsup}
\newcommand{\bfuN} {\bfu\Nsup}
\newcommand{\bfuS} {\bfu\Ssup}
\newcommand{\bfwD} {\bfw\Dsup}
\newcommand{\bfwN} {\bfw\Nsup}
\newcommand{\bfwDb} {\bfwb\Dsup}
\newcommand{\bfwNb} {\bfwb\Nsup}
\newcommand{\bfuhD} {\bfuh\Dsub}
\newcommand{\bfuhN} {\bfuh\Nsub}
\newcommand{\bfusD} {\bfu\Dsub^{\star}}
\newcommand{\bfusN} {\bfu\Nsub^{\star}}
\newcommand{\bfusDb} {\bfub{}\Dsub^{\star}}
\newcommand{\bfusNb} {\bfub{}\Nsub^{\star}}
\newcommand{\uhD} {\uh\Dsub}
\newcommand{\uhN} {\uh\Nsub}
\newcommand{\UhD} {\Uh\Dsub}
\newcommand{\UhN} {\Uh\Nsub}
\newcommand{\bfuDN} {\bfu\DNsupc}
\newcommand{\bfwDN} {\bfw\DNsupc}

%  --------------------------
%  Fracture-mechanics indexes
%  --------------------------

\newcommand{\Ic}{_{\text{\scriptsize Ic}}}

\newcommand{\KIc}{K\Ic}
\newcommand{\KI}{K\Isub}
\newcommand{\KII}{K\IIsub}
\newcommand{\KIII}{K\IIIsub}
\newcommand{\KIIIu}{\KIII^{u}}
\newcommand{\KIIIs}{\KIII^{\sigma}}

%  ------------------------------------------
%  Misc. math constructs using Roman typeface
%  ------------------------------------------

\renewcommand{\Re}{\text{Re}}
\renewcommand{\Im}{\text{Im}}

%  ---------------------------------------------
%  Misc. textual constructs using Roman typeface
%  ---------------------------------------------

\newcommand{\avec}{\hs{1.}\mbox{ avec }\hs{0.5}}

\newcommand{\oeuvre}{\oe uvre\xspace}
\newcommand{\noeud}{n\oe ud\xspace}
\newcommand{\noeuds}{n\oe uds\xspace}
\newcommand{\sign}{\text{sign}}
\newcommand{\supp}{\text{supp}}
\newcommand{\dist}{\text{dist}}
\newcommand{\Matlab}{\textsc{Matlab}}

%  Cosinus, sinus...

\newcommand{\ca}{\cos{\alpha}}
\newcommand{\cca}{\cos^{2}{\alpha}}
\newcommand{\cceL}{\cos^{2}{(\eta L)}}
\newcommand{\ccgL}{\cos^{2}{(\gL)}}
\newcommand{\ccgx}{\cos^{2}{(\gamma x)}}
\newcommand{\ccheL}{\cosh^{2}{(\eta L)}}
\newcommand{\cchgL}{\cosh^{2}{(\gamma L)}}
\newcommand{\cchgx}{\cosh^{2}{(\gamma x)}}
\newcommand{\ccost}{\cos^{2}{\theta}}
\newcommand{\ceL}{\cos\!{(\eta L)}}
\newcommand{\cgbL}{\cos\!{(\gbL)}}
\newcommand{\cgL}{\cos\!{(\gL)}}
\newcommand{\cgx}{\cos\!{(\gamma x)}}
\newcommand{\cgxi}{\cos\!{(\gamma x_{m})}}
\newcommand{\cgy}{\cos\!{(\gamma x)}}
\newcommand{\cheL}{\cosh\!{(\eta L)}}
\newcommand{\chgbL}{\cosh\!{(\gbL)}}
\newcommand{\chgL}{\cosh\!{(\gamma L)}}
\newcommand{\chgx}{\cosh\!{(\gamma x)}}
\newcommand{\chgxi}{\cosh\!{(\gamma x_{m})}}
\newcommand{\chgy}{\cosh\!{(\gamma y)}}
\newcommand{\coscp}{\cos^{2}\varphi}
\newcommand{\cosp}{\cos\varphi}
\newcommand{\cost}[1]{\cos #1 \theta }
\newcommand{\csa}{\ca\sa}
\newcommand{\cseL}{\ceL\seL}
\newcommand{\csgL}{\cgL\sgL}
\newcommand{\csgx}{\cgx\sgx}
\newcommand{\csheL}{\chgL\shgL}
\newcommand{\cshgL}{\chgL\shgL}
\newcommand{\cshgx}{\chgx\shgx}
\newcommand{\gbL}{\gamma\beta L}
\newcommand{\gL}{\gamma L}
\newcommand{\sa}{\sin{\alpha}}
\newcommand{\seL}{\sin\!{(\eta L)}}
\newcommand{\sgbL}{\sin\!{(\gbL)}}
\newcommand{\sgL}{\sin\!{(\gL)}}
\newcommand{\sgxi}{\sin\!{(\gamma x_{m})}}
\newcommand{\sgx}{\sin\!{(\gamma x)}}
\newcommand{\sgy}{\sin\!{(\gamma x)}}
\newcommand{\sheL}{\sinh\!{(\eta L)}}
\newcommand{\shgbL}{\sinh\!{(\gbL)}}
\newcommand{\shgL}{\sinh\!{(\gamma L)}}
\newcommand{\shgxi}{\sinh\!{(\gamma x_{m})}}
\newcommand{\shgx}{\sinh\!{(\gamma x)}}
\newcommand{\shgy}{\sinh\!{(\gamma y)}}
\newcommand{\sinp}{\sin\varphi}
\newcommand{\sinsp}{\sin^{2}\varphi}
\newcommand{\sint}[1]{\sin #1 \theta }
\newcommand{\ssa}{\sin^{2}{\alpha}}
\newcommand{\sseL}{\sin^{2}{(\eta L)}}
\newcommand{\ssgL}{\sin^{2}{(\gL)}}
\newcommand{\ssgx}{\sin^{2}{(\gamma x)}}
\newcommand{\ssheL}{\sinh^{2}{(\eta L)}}
\newcommand{\sshgL}{\sinh^{2}{(\gamma L)}}
\newcommand{\sshgx}{\sinh^{2}{(\gamma x)}}
\newcommand{\ssint}{\sin^{2}{\theta}}
%  --------------
%  mathrm letters
%  --------------

\newcommand{\rma} {\mathrm{a}}
\newcommand{\rmb} {\mathrm{b}}
\newcommand{\rmc} {\mathrm{c}}
\newcommand{\rmd} {\mathrm{d}}
\newcommand{\rme} {\mathrm{e}}
\newcommand{\rmf} {\mathrm{f}}
\newcommand{\rmg} {\mathrm{g}}
\newcommand{\rmh} {\mathrm{h}}
\newcommand{\rmj} {\mathrm{j}}
\newcommand{\rmi} {\mathrm{i}}
\newcommand{\rmk} {\mathrm{k}}
\newcommand{\rml} {\mathrm{l}}
\newcommand{\rmm} {\mathrm{m}}
\newcommand{\rmn} {\mathrm{n}}
\newcommand{\rmo} {\mathrm{o}}
\newcommand{\rmp} {\mathrm{p}}
\newcommand{\rmq} {\mathrm{q}}
\newcommand{\rmr} {\mathrm{r}}
\newcommand{\rms} {\mathrm{s}}
\newcommand{\rmt} {\mathrm{t}}
\newcommand{\rmu} {\mathrm{u}}
\newcommand{\rmv} {\mathrm{v}}
\newcommand{\rmw} {\mathrm{w}}
\newcommand{\rmx} {\mathrm{x}}
\newcommand{\rmy} {\mathrm{y}}
\newcommand{\rmz} {\mathrm{z}}
\newcommand{\rmA} {\mathrm{A}}
\newcommand{\rmB} {\mathrm{B}}
\newcommand{\rmC} {\mathrm{C}}
\newcommand{\rmD} {\mathrm{D}}
\newcommand{\rmE} {\mathrm{E}}
\newcommand{\rmF} {\mathrm{F}}
\newcommand{\rmG} {\mathrm{G}}
\newcommand{\rmH} {\mathrm{H}}
\newcommand{\rmI} {\mathrm{I}}
\newcommand{\rmJ} {\mathrm{J}}
\newcommand{\rmK} {\mathrm{K}}
\newcommand{\rmL} {\mathrm{L}}
\newcommand{\rmM} {\mathrm{M}}
\newcommand{\rmN} {\mathrm{N}}
\newcommand{\rmO} {\mathrm{O}}
\newcommand{\rmP} {\mathrm{P}}
\newcommand{\rmQ} {\mathrm{Q}}
\newcommand{\rmR} {\mathrm{R}}
\newcommand{\rmS} {\mathrm{S}}
\newcommand{\rmT} {\mathrm{T}}
\newcommand{\rmU} {\mathrm{U}}
\newcommand{\rmV} {\mathrm{V}}
\newcommand{\rmW} {\mathrm{W}}
\newcommand{\rmX} {\mathrm{X}}
\newcommand{\rmY} {\mathrm{Y}}
\newcommand{\rmZ} {\mathrm{Z}}
%  --------------
%  mathrm tilde letters
%  --------------

\newcommand{\rmaB} {\bar{\rma}}
\newcommand{\rmbB} {\bar{\rmb}}
\newcommand{\rmcB} {\bar{\rmc}}
\newcommand{\rmdB} {\bar{\rmd}}
\newcommand{\rmeB} {\bar{\rme}}
\newcommand{\rmfB} {\bar{\rmf}}
\newcommand{\rmgB} {\bar{\rmg}}
\newcommand{\rmhB} {\bar{\rmh}}
\newcommand{\rmjB} {\bar{\rmj}}
\newcommand{\rmkB} {\bar{\rmk}}
\newcommand{\rmlB} {\bar{\rml}}
\newcommand{\rmmB} {\bar{\rmm}}
\newcommand{\rmnB} {\bar{\rmn}}
\newcommand{\rmoB} {\bar{\rmo}}
\newcommand{\rmpB} {\bar{\rmp}}
\newcommand{\rmqB} {\bar{\rmq}}
\newcommand{\rmrB} {\bar{\rmr}}
\newcommand{\rmsB} {\bar{\rms}}
\newcommand{\rmtB} {\bar{\rmt}}
\newcommand{\rmuB} {\bar{\rmu}}
\newcommand{\rmvB} {\bar{\rmv}}
\newcommand{\rmwB} {\bar{\rmw}}
\newcommand{\rmxB} {\bar{\rmx}}
\newcommand{\rmyB} {\bar{\rmy}}
\newcommand{\rmzB} {\bar{\rmz}}
\newcommand{\rmAB} {\overline{\rmA}}
\newcommand{\rmBB} {\overline{\rmB}}
\newcommand{\rmCB} {\overline{\rmC}}
\newcommand{\rmDB} {\overline{\rmD}}
\newcommand{\rmEB} {\overline{\rmE}}
\newcommand{\rmFB} {\overline{\rmF}}
\newcommand{\rmGB} {\overline{\rmG}}
\newcommand{\rmHB} {\overline{\rmH}}
\newcommand{\rmIB} {\overline{\rmI}}
\newcommand{\rmJB} {\overline{\rmJ}}
\newcommand{\rmKB} {\overline{\rmK}}
\newcommand{\rmLB} {\overline{\rmL}}
\newcommand{\rmMB} {\overline{\rmM}}
\newcommand{\rmNB} {\overline{\rmN}}
\newcommand{\rmOB} {\overline{\rmO}}
\newcommand{\rmPB} {\overline{\rmP}}
\newcommand{\rmQB} {\overline{\rmQ}}
\newcommand{\rmRB} {\overline{\rmR}}
\newcommand{\rmSB} {\overline{\rmS}}
\newcommand{\rmTB} {\overline{\rmT}}
\newcommand{\rmUB} {\overline{\rmU}}
\newcommand{\rmVB} {\overline{\rmV}}
\newcommand{\rmWB} {\overline{\rmW}}
\newcommand{\rmXB} {\overline{\rmX}}
\newcommand{\rmYB} {\overline{\rmY}}
\newcommand{\rmZB} {\overline{\rmZ}}
%  --------------
%  mathrm tilde letters
%  --------------

\newcommand{\rmaT} {\tilde{\rma}}
\newcommand{\rmbT} {\tilde{\rmb}}
\newcommand{\rmcT} {\tilde{\rmc}}
\newcommand{\rmdT} {\tilde{\rmd}}
\newcommand{\rmeT} {\tilde{\rme}}
\newcommand{\rmfT} {\tilde{\rmf}}
\newcommand{\rmgT} {\tilde{\rmg}}
\newcommand{\rmhT} {\tilde{\rmh}}
\newcommand{\rmjT} {\tilde{\rmj}}
\newcommand{\rmkT} {\tilde{\rmk}}
\newcommand{\rmlT} {\tilde{\rml}}
\newcommand{\rmmT} {\tilde{\rmm}}
\newcommand{\rmnT} {\tilde{\rmn}}
\newcommand{\rmoT} {\tilde{\rmo}}
\newcommand{\rmpT} {\tilde{\rmp}}
\newcommand{\rmqT} {\tilde{\rmq}}
\newcommand{\rmrT} {\tilde{\rmr}}
\newcommand{\rmsT} {\tilde{\rms}}
\newcommand{\rmtT} {\tilde{\rmt}}
\newcommand{\rmuT} {\tilde{\rmu}}
\newcommand{\rmvT} {\tilde{\rmv}}
\newcommand{\rmwT} {\tilde{\rmw}}
\newcommand{\rmxT} {\tilde{\rmx}}
\newcommand{\rmyT} {\tilde{\rmy}}
\newcommand{\rmzT} {\tilde{\rmz}}
\newcommand{\rmAT} {\widetilde{\rmA}}
\newcommand{\rmBT} {\widetilde{\rmB}}
\newcommand{\rmCT} {\widetilde{\rmC}}
\newcommand{\rmDT} {\widetilde{\rmD}}
\newcommand{\rmET} {\widetilde{\rmE}}
\newcommand{\rmFT} {\widetilde{\rmF}}
\newcommand{\rmGT} {\widetilde{\rmG}}
\newcommand{\rmHT} {\widetilde{\rmH}}
\newcommand{\rmIT} {\widetilde{\rmI}}
\newcommand{\rmJT} {\widetilde{\rmJ}}
\newcommand{\rmKT} {\widetilde{\rmK}}
\newcommand{\rmLT} {\widetilde{\rmL}}
\newcommand{\rmMT} {\widetilde{\rmM}}
\newcommand{\rmNT} {\widetilde{\rmN}}
\newcommand{\rmOT} {\widetilde{\rmO}}
\newcommand{\rmPT} {\widetilde{\rmP}}
\newcommand{\rmQT} {\widetilde{\rmQ}}
\newcommand{\rmRT} {\widetilde{\rmR}}
\newcommand{\rmST} {\widetilde{\rmS}}
\newcommand{\rmTT} {\widetilde{\rmT}}
\newcommand{\rmUT} {\widetilde{\rmU}}
\newcommand{\rmVT} {\widetilde{\rmV}}
\newcommand{\rmWT} {\widetilde{\rmW}}
\newcommand{\rmXT} {\widetilde{\rmX}}
\newcommand{\rmYT} {\widetilde{\rmY}}
\newcommand{\rmZT} {\widetilde{\rmZ}}
%  ----------------------
%  Sansserif Roman letters
%  ----------------------

\newcommand{\sfA} {\mathsf{A}}
\newcommand{\sfB} {\mathsf{B}}
\newcommand{\sfC} {\mathsf{C}}
\newcommand{\sfD} {\mathsf{D}}
\newcommand{\sfE} {\mathsf{E}}
\newcommand{\sfF} {\mathsf{F}}
\newcommand{\sfG} {\mathsf{G}}
\newcommand{\sfH} {\mathsf{H}}
\newcommand{\sfI} {\mathsf{I}}
\newcommand{\sfJ} {\mathsf{J}}
\newcommand{\sfK} {\mathsf{K}}
\newcommand{\sfL} {\mathsf{L}}
\newcommand{\sfM} {\mathsf{M}}
\newcommand{\sfN} {\mathsf{N}}
\newcommand{\sfO} {\mathsf{O}}
\newcommand{\sfP} {\mathsf{P}}
\newcommand{\sfQ} {\mathsf{Q}}
\newcommand{\sfR} {\mathsf{R}}
\newcommand{\sfS} {\mathsf{S}}
\newcommand{\sfT} {\mathsf{T}}
\newcommand{\sfU} {\mathsf{U}}
\newcommand{\sfV} {\mathsf{V}}
\newcommand{\sfW} {\mathsf{W}}
\newcommand{\sfX} {\mathsf{X}}
\newcommand{\sfY} {\mathsf{Y}}
\newcommand{\sfZ} {\mathsf{Z}}

\newcommand{\sfa} {\mathsf{a}}
\newcommand{\sfb} {\mathsf{b}}
\newcommand{\sfc} {\mathsf{c}}
\newcommand{\sfd} {\mathsf{d}}
\newcommand{\sfe} {\mathsf{e}}
\newcommand{\sff} {\mathsf{f}}
\newcommand{\sfg} {\mathsf{g}}
\newcommand{\sfh} {\mathsf{h}}
\newcommand{\sfi} {\mathsf{i}}
\newcommand{\sfj} {\mathsf{j}}
\newcommand{\sfk} {\mathsf{k}}
\newcommand{\sfl} {\mathsf{l}}
\newcommand{\sfm} {\mathsf{m}}
\newcommand{\sfn} {\mathsf{n}}
\newcommand{\sfo} {\mathsf{o}}
\newcommand{\sfp} {\mathsf{p}}
\newcommand{\sfq} {\mathsf{q}}
\newcommand{\sfr} {\mathsf{r}}
\newcommand{\sfs} {\mathsf{s}}
\newcommand{\sft} {\mathsf{t}}
\newcommand{\sfu} {\mathsf{u}}
\newcommand{\sfv} {\mathsf{v}}
\newcommand{\sfw} {\mathsf{w}}
\newcommand{\sfx} {\mathsf{x}}
\newcommand{\sfy} {\mathsf{y}}
\newcommand{\sfz} {\mathsf{z}}
%  --------------
%  mathsf hat letters
%  --------------

\newcommand{\sfah} {\hat{\sfa}}
\newcommand{\sfbh} {\hat{\sfb}}
\newcommand{\sfch} {\hat{\sfc}}
\newcommand{\sfdh} {\hat{\sfd}}
\newcommand{\sfeh} {\hat{\sfe}}
\newcommand{\sffh} {\hat{\sff}}
\newcommand{\sfgh} {\hat{\sfg}}
\newcommand{\sfhh} {\hat{\sfh}}
\newcommand{\sfjh} {\hat{\sfj}}
\newcommand{\sfkh} {\hat{\sfk}}
\newcommand{\sflh} {\hat{\sfl}}
\newcommand{\sfmh} {\hat{\sfm}}
\newcommand{\sfnh} {\hat{\sfn}}
\newcommand{\sfoh} {\hat{\sfo}}
\newcommand{\sfph} {\hat{\sfp}}
\newcommand{\sfqh} {\hat{\sfq}}
\newcommand{\sfrh} {\hat{\sfr}}
\newcommand{\sfsh} {\hat{\sfs}}
\newcommand{\sfth} {\hat{\sft}}
\newcommand{\sfuh} {\hat{\sfu}}
\newcommand{\sfvh} {\hat{\sfv}}
\newcommand{\sfwh} {\hat{\sfw}}
\newcommand{\sfxh} {\hat{\sfx}}
\newcommand{\sfyh} {\hat{\sfy}}
\newcommand{\sfzh} {\hat{\sfz}}
\newcommand{\sfAH} {\widehat{\sfA}}
\newcommand{\sfBH} {\widehat{\sfB}}
\newcommand{\sfCH} {\widehat{\sfC}}
\newcommand{\sfDH} {\widehat{\sfD}}
\newcommand{\sfEH} {\widehat{\sfE}}
\newcommand{\sfFH} {\widehat{\sfF}}
\newcommand{\sfGH} {\widehat{\sfG}}
\newcommand{\sfHH} {\widehat{\sfH}}
\newcommand{\sfIH} {\widehat{\sfI}}
\newcommand{\sfJH} {\widehat{\sfJ}}
\newcommand{\sfKH} {\widehat{\sfK}}
\newcommand{\sfLH} {\widehat{\sfL}}
\newcommand{\sfMH} {\widehat{\sfM}}
\newcommand{\sfNH} {\widehat{\sfN}}
\newcommand{\sfOH} {\widehat{\sfO}}
\newcommand{\sfPH} {\widehat{\sfP}}
\newcommand{\sfQH} {\widehat{\sfQ}}
\newcommand{\sfRH} {\widehat{\sfR}}
\newcommand{\sfSH} {\widehat{\sfS}}
\newcommand{\sfTH} {\widehat{\sfT}}
\newcommand{\sfUH} {\widehat{\sfU}}
\newcommand{\sfVH} {\widehat{\sfV}}
\newcommand{\sfWH} {\widehat{\sfW}}
\newcommand{\sfXH} {\widehat{\sfX}}
\newcommand{\sfYH} {\widehat{\sfY}}
\newcommand{\sfZH} {\widehat{\sfZ}}
%  --------------
%  mathrm bar letters
%  --------------

\newcommand{\sfab} {\bar{\sfa}}
\newcommand{\sfbb} {\bar{\sfb}}
\newcommand{\sfcb} {\bar{\sfc}}
\newcommand{\sfdb} {\bar{\sfd}}
\newcommand{\sfeb} {\bar{\sfe}}
\newcommand{\sffb} {\bar{\sff}}
\newcommand{\sfgb} {\bar{\sfg}}
\newcommand{\sfhb} {\bar{\sfh}}
\newcommand{\sfjb} {\bar{\sfj}}
\newcommand{\sfkb} {\bar{\sfk}}
\newcommand{\sflb} {\bar{\sfl}}
\newcommand{\sfmb} {\bar{\sfm}}
\newcommand{\sfnb} {\bar{\sfn}}
\newcommand{\sfob} {\bar{\sfo}}
\newcommand{\sfpb} {\bar{\sfp}}
\newcommand{\sfqb} {\bar{\sfq}}
\newcommand{\sfrb} {\bar{\sfr}}
\newcommand{\sfsb} {\bar{\sfs}}
\newcommand{\sftb} {\bar{\sft}}
\newcommand{\sfub} {\bar{\sfu}}
\newcommand{\sfvb} {\bar{\sfv}}
\newcommand{\sfwb} {\bar{\sfw}}
\newcommand{\sfxb} {\bar{\sfx}}
\newcommand{\sfyb} {\bar{\sfy}}
\newcommand{\sfzb} {\bar{\sfz}}

\newcommand{\sfaB} {\overline{\sfa}}
\newcommand{\sfbB} {\overline{\sfb}}
\newcommand{\sfcB} {\overline{\sfc}}
\newcommand{\sfdB} {\overline{\sfd}}
\newcommand{\sfeB} {\overline{\sfe}}
\newcommand{\sffB} {\overline{\sff}}
\newcommand{\sfgB} {\overline{\sfg}}
\newcommand{\sfhB} {\overline{\sfh}}
\newcommand{\sfjB} {\overline{\sfj}}
\newcommand{\sfkB} {\overline{\sfk}}
\newcommand{\sflB} {\overline{\sfl}}
\newcommand{\sfmB} {\overline{\sfm}}
\newcommand{\sfnB} {\overline{\sfn}}
\newcommand{\sfoB} {\overline{\sfo}}
\newcommand{\sfpB} {\overline{\sfp}}
\newcommand{\sfqB} {\overline{\sfq}}
\newcommand{\sfrB} {\overline{\sfr}}
\newcommand{\sfsB} {\overline{\sfs}}
\newcommand{\sftB} {\overline{\sft}}
\newcommand{\sfuB} {\overline{\sfu}}
\newcommand{\sfvB} {\overline{\sfv}}
\newcommand{\sfwB} {\overline{\sfw}}
\newcommand{\sfxB} {\overline{\sfx}}
\newcommand{\sfyB} {\overline{\sfy}}
\newcommand{\sfzB} {\overline{\sfz}}

\newcommand{\sfAb} {\bar{\sfA}}
\newcommand{\sfBb} {\bar{\sfB}}
\newcommand{\sfCb} {\bar{\sfC}}
\newcommand{\sfDb} {\bar{\sfD}}
\newcommand{\sfEb} {\bar{\sfE}}
\newcommand{\sfFb} {\bar{\sfF}}
\newcommand{\sfGb} {\bar{\sfG}}
\newcommand{\sfHb} {\bar{\sfH}}
\newcommand{\sfIb} {\bar{\sfI}}
\newcommand{\sfJb} {\bar{\sfJ}}
\newcommand{\sfKb} {\bar{\sfK}}
\newcommand{\sfLb} {\bar{\sfL}}
\newcommand{\sfMb} {\bar{\sfM}}
\newcommand{\sfNb} {\bar{\sfN}}
\newcommand{\sfOb} {\bar{\sfO}}
\newcommand{\sfPb} {\bar{\sfP}}
\newcommand{\sfQb} {\bar{\sfQ}}
\newcommand{\sfRb} {\bar{\sfR}}
\newcommand{\sfSb} {\bar{\sfS}}
\newcommand{\sfTb} {\bar{\sfT}}
\newcommand{\sfUb} {\bar{\sfU}}
\newcommand{\sfVb} {\bar{\sfV}}
\newcommand{\sfWb} {\bar{\sfW}}
\newcommand{\sfXb} {\bar{\sfX}}
\newcommand{\sfYb} {\bar{\sfY}}
\newcommand{\sfZb} {\bar{\sfZ}}

\newcommand{\sfAB} {\overline{\sfA}}
\newcommand{\sfBB} {\overline{\sfB}}
\newcommand{\sfCB} {\overline{\sfC}}
\newcommand{\sfDB} {\overline{\sfD}}
\newcommand{\sfEB} {\overline{\sfE}}
\newcommand{\sfFB} {\overline{\sfF}}
\newcommand{\sfGB} {\overline{\sfG}}
\newcommand{\sfHB} {\overline{\sfH}}
\newcommand{\sfIB} {\overline{\sfI}}
\newcommand{\sfJB} {\overline{\sfJ}}
\newcommand{\sfKB} {\overline{\sfK}}
\newcommand{\sfLB} {\overline{\sfL}}
\newcommand{\sfMB} {\overline{\sfM}}
\newcommand{\sfNB} {\overline{\sfN}}
\newcommand{\sfOB} {\overline{\sfO}}
\newcommand{\sfPB} {\overline{\sfP}}
\newcommand{\sfQB} {\overline{\sfQ}}
\newcommand{\sfRB} {\overline{\sfR}}
\newcommand{\sfSB} {\overline{\sfS}}
\newcommand{\sfTB} {\overline{\sfT}}
\newcommand{\sfUB} {\overline{\sfU}}
\newcommand{\sfVB} {\overline{\sfV}}
\newcommand{\sfWB} {\overline{\sfW}}
\newcommand{\sfXB} {\overline{\sfX}}
\newcommand{\sfYB} {\overline{\sfY}}
\newcommand{\sfZB} {\overline{\sfZ}}
%  --------------
%  mathrm tilde letters
%  --------------

\newcommand{\sfaT} {\tilde{\sfa}}
\newcommand{\sfbT} {\tilde{\sfb}}
\newcommand{\sfcT} {\tilde{\sfc}}
\newcommand{\sfdT} {\tilde{\sfd}}
\newcommand{\sfeT} {\tilde{\sfe}}
\newcommand{\sffT} {\tilde{\sff}}
\newcommand{\sfgT} {\tilde{\sfg}}
\newcommand{\sfhT} {\tilde{\sfh}}
\newcommand{\sfjT} {\tilde{\sfj}}
\newcommand{\sfkT} {\tilde{\sfk}}
\newcommand{\sflT} {\tilde{\sfl}}
\newcommand{\sfmT} {\tilde{\sfm}}
\newcommand{\sfnT} {\tilde{\sfn}}
\newcommand{\sfoT} {\tilde{\sfo}}
\newcommand{\sfpT} {\tilde{\sfp}}
\newcommand{\sfqT} {\tilde{\sfq}}
\newcommand{\sfrT} {\tilde{\sfr}}
\newcommand{\sfsT} {\tilde{\sfs}}
\newcommand{\sftT} {\tilde{\sft}}
\newcommand{\sfuT} {\tilde{\sfu}}
\newcommand{\sfvT} {\tilde{\sfv}}
\newcommand{\sfwT} {\tilde{\sfw}}
\newcommand{\sfxT} {\tilde{\sfx}}
\newcommand{\sfyT} {\tilde{\sfy}}
\newcommand{\sfzT} {\tilde{\sfz}}
\newcommand{\sfAT} {\widetilde{\sfA}}
\newcommand{\sfBT} {\widetilde{\sfB}}
\newcommand{\sfCT} {\widetilde{\sfC}}
\newcommand{\sfDT} {\widetilde{\sfD}}
\newcommand{\sfET} {\widetilde{\sfE}}
\newcommand{\sfFT} {\widetilde{\sfF}}
\newcommand{\sfGT} {\widetilde{\sfG}}
\newcommand{\sfHT} {\widetilde{\sfH}}
\newcommand{\sfIT} {\widetilde{\sfI}}
\newcommand{\sfJT} {\widetilde{\sfJ}}
\newcommand{\sfKT} {\widetilde{\sfK}}
\newcommand{\sfLT} {\widetilde{\sfL}}
\newcommand{\sfMT} {\widetilde{\sfM}}
\newcommand{\sfNT} {\widetilde{\sfN}}
\newcommand{\sfOT} {\widetilde{\sfO}}
\newcommand{\sfPT} {\widetilde{\sfP}}
\newcommand{\sfQT} {\widetilde{\sfQ}}
\newcommand{\sfRT} {\widetilde{\sfR}}
\newcommand{\sfST} {\widetilde{\sfS}}
\newcommand{\sfTT} {\widetilde{\sfT}}
\newcommand{\sfUT} {\widetilde{\sfU}}
\newcommand{\sfVT} {\widetilde{\sfV}}
\newcommand{\sfWT} {\widetilde{\sfW}}
\newcommand{\sfXT} {\widetilde{\sfX}}
\newcommand{\sfYT} {\widetilde{\sfY}}
\newcommand{\sfZT} {\widetilde{\sfZ}}
%  ------------------------
%  Tilded letters, boldmath
%  ------------------------

\newcommand{\bfat} {\tilde{\boldsymbol{a}}{}}
\newcommand{\bfbt} {\tilde{\boldsymbol{b}}{}}
\newcommand{\bfct} {\tilde{\boldsymbol{c}}{}}
\newcommand{\bfdt} {\tilde{\boldsymbol{d}}{}}
\newcommand{\bfet} {\tilde{\boldsymbol{e}}{}}
\newcommand{\bfft} {\tilde{\boldsymbol{f}}{}}
\newcommand{\bfgt} {\tilde{\boldsymbol{g}}{}}
\newcommand{\bfht} {\tilde{\boldsymbol{h}}{}}
\newcommand{\bfjt} {\tilde{\boldsymbol{j}}{}}
\newcommand{\bfkt} {\tilde{\boldsymbol{k}}{}}
\newcommand{\bflt} {\tilde{\boldsymbol{\ell}}{}}
\newcommand{\bfmt} {\tilde{\boldsymbol{m}}{}}
\newcommand{\bfnt} {\tilde{\boldsymbol{n}}{}}
\newcommand{\bfot} {\tilde{\boldsymbol{o}}{}}
\newcommand{\bfpt} {\tilde{\boldsymbol{p}}{}}
\newcommand{\bfqt} {\tilde{\boldsymbol{q}}{}}
\newcommand{\bfrt} {\tilde{\boldsymbol{r}}{}}
\newcommand{\bfst} {\tilde{\boldsymbol{s}}{}}
\newcommand{\bftt} {\tilde{\boldsymbol{t}}{}}
\newcommand{\bfut} {\tilde{\boldsymbol{u}}{}}
\newcommand{\bfvt} {\tilde{\boldsymbol{v}}{}}
\newcommand{\bfwt} {\tilde{\boldsymbol{w}}{}}
\newcommand{\bfxt} {\tilde{\boldsymbol{x}}{}}
\newcommand{\bfyt} {\tilde{\boldsymbol{y}}{}}
\newcommand{\bfzt} {\tilde{\boldsymbol{z}}{}}
\newcommand{\bfAt} {\tilde{\boldsymbol{A}}{}}
\newcommand{\bfBt} {\tilde{\boldsymbol{B}}{}}
\newcommand{\bfCt} {\tilde{\boldsymbol{C}}{}}
\newcommand{\bfDt} {\tilde{\boldsymbol{D}}{}}
\newcommand{\bfEt} {\tilde{\boldsymbol{E}}{}}
\newcommand{\bfFt} {\tilde{\boldsymbol{F}}{}}
\newcommand{\bfGt} {\tilde{\boldsymbol{G}}{}}
\newcommand{\bfHt} {\tilde{\boldsymbol{H}}{}}
\newcommand{\bfIt} {\tilde{\boldsymbol{I}}{}}
\newcommand{\bfJt} {\tilde{\boldsymbol{J}}{}}
\newcommand{\bfKt} {\tilde{\boldsymbol{K}}{}}
\newcommand{\bfLt} {\tilde{\boldsymbol{L}}{}}
\newcommand{\bfMt} {\tilde{\boldsymbol{M}}{}}
\newcommand{\bfNt} {\tilde{\boldsymbol{N}}{}}
\newcommand{\bfOt} {\tilde{\boldsymbol{O}}{}}
\newcommand{\bfPt} {\tilde{\boldsymbol{P}}{}}
\newcommand{\bfQt} {\tilde{\boldsymbol{Q}}{}}
\newcommand{\bfRt} {\tilde{\boldsymbol{R}}{}}
\newcommand{\bfSt} {\tilde{\boldsymbol{S}}{}}
\newcommand{\bfTt} {\tilde{\boldsymbol{T}}{}}
\newcommand{\bfUt} {\tilde{\boldsymbol{U}}{}}
\newcommand{\bfVt} {\tilde{\boldsymbol{V}}{}}
\newcommand{\bfWt} {\tilde{\boldsymbol{W}}{}}
\newcommand{\bfXt} {\tilde{\boldsymbol{X}}{}}
\newcommand{\bfYt} {\tilde{\boldsymbol{Y}}{}}
\newcommand{\bfZt} {\tilde{\boldsymbol{Z}}{}}

\newcommand{\bfaT} {\widetilde{\boldsymbol{a}}{}}
\newcommand{\bfbT} {\widetilde{\boldsymbol{b}}{}}
\newcommand{\bfcT} {\widetilde{\boldsymbol{c}}{}}
\newcommand{\bfdT} {\widetilde{\boldsymbol{d}}{}}
\newcommand{\bfeT} {\widetilde{\boldsymbol{e}}{}}
\newcommand{\bffT} {\widetilde{\boldsymbol{f}}{}}
\newcommand{\bfgT} {\widetilde{\boldsymbol{g}}{}}
\newcommand{\bfhT} {\widetilde{\boldsymbol{h}}{}}
\newcommand{\bfjT} {\widetilde{\boldsymbol{j}}{}}
\newcommand{\bfkT} {\widetilde{\boldsymbol{k}}{}}
\newcommand{\bflT} {\widetilde{\boldsymbol{\ell}}{}}
\newcommand{\bfmT} {\widetilde{\boldsymbol{m}}{}}
\newcommand{\bfnT} {\widetilde{\boldsymbol{n}}{}}
\newcommand{\bfoT} {\widetilde{\boldsymbol{o}}{}}
\newcommand{\bfpT} {\widetilde{\boldsymbol{p}}{}}
\newcommand{\bfqT} {\widetilde{\boldsymbol{q}}{}}
\newcommand{\bfrT} {\widetilde{\boldsymbol{r}}{}}
\newcommand{\bfsT} {\widetilde{\boldsymbol{s}}{}}
\newcommand{\bftT} {\widetilde{\boldsymbol{t}}{}}
\newcommand{\bfuT} {\widetilde{\boldsymbol{u}}{}}
\newcommand{\bfvT} {\widetilde{\boldsymbol{v}}{}}
\newcommand{\bfwT} {\widetilde{\boldsymbol{w}}{}}
\newcommand{\bfxT} {\widetilde{\boldsymbol{x}}{}}
\newcommand{\bfyT} {\widetilde{\boldsymbol{y}}{}}
\newcommand{\bfzT} {\widetilde{\boldsymbol{z}}{}}
\newcommand{\bfAT} {\widetilde{\boldsymbol{A}}{}}
\newcommand{\bfBT} {\widetilde{\boldsymbol{B}}{}}
\newcommand{\bfCT} {\widetilde{\boldsymbol{C}}{}}
\newcommand{\bfDT} {\widetilde{\boldsymbol{D}}{}}
\newcommand{\bfET} {\widetilde{\boldsymbol{E}}{}}
\newcommand{\bfFT} {\widetilde{\boldsymbol{F}}{}}
\newcommand{\bfGT} {\widetilde{\boldsymbol{G}}{}}
\newcommand{\bfHT} {\widetilde{\boldsymbol{H}}{}}
\newcommand{\bfIT} {\widetilde{\boldsymbol{I}}{}}
\newcommand{\bfJT} {\widetilde{\boldsymbol{J}}{}}
\newcommand{\bfKT} {\widetilde{\boldsymbol{K}}{}}
\newcommand{\bfLT} {\widetilde{\boldsymbol{L}}{}}
\newcommand{\bfMT} {\widetilde{\boldsymbol{M}}{}}
\newcommand{\bfNT} {\widetilde{\boldsymbol{N}}{}}
\newcommand{\bfOT} {\widetilde{\boldsymbol{O}}{}}
\newcommand{\bfPT} {\widetilde{\boldsymbol{P}}{}}
\newcommand{\bfQT} {\widetilde{\boldsymbol{Q}}{}}
\newcommand{\bfRT} {\widetilde{\boldsymbol{R}}{}}
\newcommand{\bfST} {\widetilde{\boldsymbol{S}}{}}
\newcommand{\bfTT} {\widetilde{\boldsymbol{T}}{}}
\newcommand{\bfUT} {\widetilde{\boldsymbol{U}}{}}
\newcommand{\bfVT} {\widetilde{\boldsymbol{V}}{}}
\newcommand{\bfWT} {\widetilde{\boldsymbol{W}}{}}
\newcommand{\bfXT} {\widetilde{\boldsymbol{X}}{}}
\newcommand{\bfYT} {\widetilde{\boldsymbol{Y}}{}}
\newcommand{\bfZT} {\widetilde{\boldsymbol{Z}}{}}
%  ---------------------
%  Hat letters, boldmath
%  ---------------------

\newcommand{\bfah} {\hat{\boldsymbol{a}}{}}
\newcommand{\bfbh} {\hat{\boldsymbol{b}}{}}
\newcommand{\bfch} {\hat{\boldsymbol{c}}{}}
\newcommand{\bfdh} {\hat{\boldsymbol{d}}{}}
\newcommand{\bfeh} {\hat{\boldsymbol{e}}{}}
\newcommand{\bffh} {\hat{\boldsymbol{f}}{}}
\newcommand{\bfgh} {\hat{\boldsymbol{g}}{}}
\newcommand{\bfhh} {\hat{\boldsymbol{h}}{}}
\newcommand{\bfih} {\hat{\boldsymbol{\imath}}{}}
\newcommand{\bfjh} {\hat{\boldsymbol{\jmath}}{}}
\newcommand{\bfkh} {\hat{\boldsymbol{k}}{}}
\newcommand{\bflh} {\hat{\boldsymbol{\ell}}{}}
\newcommand{\bfmh} {\hat{\boldsymbol{m}}{}}
\newcommand{\bfnh} {\hat{\boldsymbol{n}}{}}
\newcommand{\bfoh} {\hat{\boldsymbol{o}}{}}
% \newcommand{\bfph} {\hat{\boldsymbol{p}}{}}
\newcommand{\bfqh} {\hat{\boldsymbol{q}}{}}
\newcommand{\bfrh} {\hat{\boldsymbol{r}}{}}
\newcommand{\bfsh} {\hat{\boldsymbol{s}}{}}
% \newcommand{\bfth} {\hat{\boldsymbol{t}}{}}
\newcommand{\bfuh} {\hat{\boldsymbol{u}}{}}
\newcommand{\bfvh} {\hat{\boldsymbol{v}}{}}
\newcommand{\bfwh} {\hat{\boldsymbol{w}}{}}
\newcommand{\bfxh} {\hat{\boldsymbol{x}}{}}
\newcommand{\bfyh} {\hat{\boldsymbol{y}}{}}
\newcommand{\bfzh} {\hat{\boldsymbol{z}}{}}

\newcommand{\bfAh} {\hat{\boldsymbol{A}}{}}
\newcommand{\bfBh} {\hat{\boldsymbol{B}}{}}
\newcommand{\bfCh} {\hat{\boldsymbol{C}}{}}
\newcommand{\bfDh} {\hat{\boldsymbol{D}}{}}
\newcommand{\bfEh} {\hat{\boldsymbol{E}}{}}
\newcommand{\bfFh} {\hat{\boldsymbol{F}}{}}
\newcommand{\bfGh} {\hat{\boldsymbol{G}}{}}
\newcommand{\bfHh} {\hat{\boldsymbol{H}}{}}
\newcommand{\bfIh} {\hat{\boldsymbol{I}}{}}
\newcommand{\bfJh} {\hat{\boldsymbol{J}}{}}
\newcommand{\bfKh} {\hat{\boldsymbol{K}}{}}
\newcommand{\bfLh} {\hat{\boldsymbol{L}}{}}
\newcommand{\bfMh} {\hat{\boldsymbol{M}}{}}
\newcommand{\bfNh} {\hat{\boldsymbol{N}}{}}
\newcommand{\bfOh} {\hat{\boldsymbol{O}}{}}
% \newcommand{\bfPh} {\hat{\boldsymbol{P}}{}}
\newcommand{\bfQh} {\hat{\boldsymbol{Q}}{}}
\newcommand{\bfRh} {\hat{\boldsymbol{R}}{}}
\newcommand{\bfSh} {\hat{\boldsymbol{S}}{}}
% \newcommand{\bfTh} {\hat{\boldsymbol{T}}{}}
\newcommand{\bfUh} {\hat{\boldsymbol{U}}{}}
\newcommand{\bfVh} {\hat{\boldsymbol{V}}{}}
\newcommand{\bfWh} {\hat{\boldsymbol{W}}{}}
\newcommand{\bfXh} {\hat{\boldsymbol{X}}{}}
\newcommand{\bfYh} {\hat{\boldsymbol{Y}}{}}
\newcommand{\bfZh} {\hat{\boldsymbol{Z}}{}}

\newcommand{\bfaH} {\widehat{\boldsymbol{a}}{}}
\newcommand{\bfbH} {\widehat{\boldsymbol{b}}{}}
\newcommand{\bfcH} {\widehat{\boldsymbol{c}}{}}
\newcommand{\bfdH} {\widehat{\boldsymbol{d}}{}}
\newcommand{\bfeH} {\widehat{\boldsymbol{e}}{}}
\newcommand{\bffH} {\widehat{\boldsymbol{f}}{}}
\newcommand{\bfgH} {\widehat{\boldsymbol{g}}{}}
\newcommand{\bfhH} {\widehat{\boldsymbol{h}}{}}
\newcommand{\bfiH} {\widehat{\boldsymbol{\imath}}{}}
\newcommand{\bfjH} {\widehat{\boldsymbol{\jmath}}{}}
\newcommand{\bfkH} {\widehat{\boldsymbol{k}}{}}
\newcommand{\bflH} {\widehat{\boldsymbol{\ell}}{}}
\newcommand{\bfmH} {\widehat{\boldsymbol{m}}{}}
\newcommand{\bfnH} {\widehat{\boldsymbol{n}}{}}
\newcommand{\bfoH} {\widehat{\boldsymbol{o}}{}}
\newcommand{\bfpH} {\widehat{\boldsymbol{p}}{}}
\newcommand{\bfqH} {\widehat{\boldsymbol{q}}{}}
\newcommand{\bfrH} {\widehat{\boldsymbol{r}}{}}
\newcommand{\bfsH} {\widehat{\boldsymbol{s}}{}}
\newcommand{\bftH} {\widehat{\boldsymbol{t}}{}}
\newcommand{\bfuH} {\widehat{\boldsymbol{u}}{}}
\newcommand{\bfvH} {\widehat{\boldsymbol{v}}{}}
\newcommand{\bfwH} {\widehat{\boldsymbol{w}}{}}
\newcommand{\bfxH} {\widehat{\boldsymbol{x}}{}}
\newcommand{\bfyH} {\widehat{\boldsymbol{y}}{}}
\newcommand{\bfzH} {\widehat{\boldsymbol{z}}{}}

\newcommand{\bfAH} {\widehat{\boldsymbol{A}}{}}
\newcommand{\bfBH} {\widehat{\boldsymbol{B}}{}}
\newcommand{\bfCH} {\widehat{\boldsymbol{C}}{}}
\newcommand{\bfDH} {\widehat{\boldsymbol{D}}{}}
\newcommand{\bfEH} {\widehat{\boldsymbol{E}}{}}
\newcommand{\bfFH} {\widehat{\boldsymbol{F}}{}}
\newcommand{\bfGH} {\widehat{\boldsymbol{G}}{}}
\newcommand{\bfHH} {\widehat{\boldsymbol{H}}{}}
\newcommand{\bfIH} {\widehat{\boldsymbol{I}}{}}
\newcommand{\bfJH} {\widehat{\boldsymbol{J}}{}}
\newcommand{\bfKH} {\widehat{\boldsymbol{K}}{}}
\newcommand{\bfLH} {\widehat{\boldsymbol{L}}{}}
\newcommand{\bfMH} {\widehat{\boldsymbol{M}}{}}
\newcommand{\bfNH} {\widehat{\boldsymbol{N}}{}}
\newcommand{\bfOH} {\widehat{\boldsymbol{O}}{}}
\newcommand{\bfPH} {\widehat{\boldsymbol{P}}{}}
\newcommand{\bfQH} {\widehat{\boldsymbol{Q}}{}}
\newcommand{\bfRH} {\widehat{\boldsymbol{R}}{}}
\newcommand{\bfSH} {\widehat{\boldsymbol{S}}{}}
\newcommand{\bfTH} {\widehat{\boldsymbol{T}}{}}
\newcommand{\bfUH} {\widehat{\boldsymbol{U}}{}}
\newcommand{\bfVH} {\widehat{\boldsymbol{V}}{}}
\newcommand{\bfWH} {\widehat{\boldsymbol{W}}{}}
\newcommand{\bfXH} {\widehat{\boldsymbol{X}}{}}
\newcommand{\bfYH} {\widehat{\boldsymbol{Y}}{}}
\newcommand{\bfZH} {\widehat{\boldsymbol{Z}}{}}
%  -----------------------
%  Roman letters, boldface
%  -----------------------

\newcommand{\bra} {\mathbf{a}}
\newcommand{\brb} {\mathbf{b}}
\newcommand{\brc} {\mathbf{c}}
\newcommand{\brd} {\mathbf{d}}
\newcommand{\bre} {\mathbf{e}}
\newcommand{\brf} {\mathbf{f}}
\newcommand{\brg} {\mathbf{g}}
\newcommand{\brh} {\mathbf{h}}
\newcommand{\bri} {\mathbf{i}}
\newcommand{\brj} {\mathbf{j}}
\newcommand{\brk} {\mathbf{k}}
\newcommand{\brl} {\mathbf{l}}
\newcommand{\brm} {\mathbf{m}}
\newcommand{\brn} {\mathbf{n}}
\newcommand{\bro} {\mathbf{o}}
\newcommand{\brp} {\mathbf{p}}
\newcommand{\brq} {\mathbf{q}}
\newcommand{\brr} {\mathbf{r}}
\newcommand{\brs} {\mathbf{s}}
\newcommand{\brt} {\mathbf{t}}
\newcommand{\bru} {\mathbf{u}}
\newcommand{\brv} {\mathbf{v}}
\newcommand{\brw} {\mathbf{w}}
\newcommand{\brx} {\mathbf{x}}
\newcommand{\bry} {\mathbf{y}}
\newcommand{\brz} {\mathbf{z}}

\newcommand{\brA} {\mathbf{A}}
\newcommand{\brB} {\mathbf{B}}
\newcommand{\brC} {\mathbf{C}}
\newcommand{\brD} {\mathbf{D}}
\newcommand{\brE} {\mathbf{E}}
\newcommand{\brF} {\mathbf{F}}
\newcommand{\brG} {\mathbf{G}}
\newcommand{\brH} {\mathbf{H}}
\newcommand{\brI} {\mathbf{I}}
\newcommand{\brJ} {\mathbf{J}}
\newcommand{\brK} {\mathbf{K}}
\newcommand{\brL} {\mathbf{L}}
\newcommand{\brM} {\mathbf{M}}
\newcommand{\brN} {\mathbf{N}}
\newcommand{\brO} {\mathbf{O}}
\newcommand{\brP} {\mathbf{P}}
\newcommand{\brQ} {\mathbf{Q}}
\newcommand{\brR} {\mathbf{R}}
\newcommand{\brS} {\mathbf{S}}
\newcommand{\brT} {\mathbf{T}}
\newcommand{\brU} {\mathbf{U}}
\newcommand{\brV} {\mathbf{V}}
\newcommand{\brW} {\mathbf{W}}
\newcommand{\brX} {\mathbf{X}}
\newcommand{\brY} {\mathbf{Y}}
\newcommand{\brZ} {\mathbf{Z}}
%  ----------------------
%  Sansserif boldface Roman letters
%  ----------------------

\newcommand{\bsfA} {\boldsymbol{\mathsf{A}}}
\newcommand{\bsfB} {\boldsymbol{\mathsf{B}}}
\newcommand{\bsfC} {\boldsymbol{\mathsf{C}}}
\newcommand{\bsfD} {\boldsymbol{\mathsf{D}}}
\newcommand{\bsfE} {\boldsymbol{\mathsf{E}}}
\newcommand{\bsfF} {\boldsymbol{\mathsf{F}}}
\newcommand{\bsfG} {\boldsymbol{\mathsf{G}}}
\newcommand{\bsfH} {\boldsymbol{\mathsf{H}}}
\newcommand{\bsfI} {\boldsymbol{\mathsf{I}}}
\newcommand{\bsfJ} {\boldsymbol{\mathsf{J}}}
\newcommand{\bsfK} {\boldsymbol{\mathsf{K}}}
\newcommand{\bsfL} {\boldsymbol{\mathsf{L}}}
\newcommand{\bsfM} {\boldsymbol{\mathsf{M}}}
\newcommand{\bsfN} {\boldsymbol{\mathsf{N}}}
\newcommand{\bsfO} {\boldsymbol{\mathsf{O}}}
\newcommand{\bsfP} {\boldsymbol{\mathsf{P}}}
\newcommand{\bsfQ} {\boldsymbol{\mathsf{Q}}}
\newcommand{\bsfR} {\boldsymbol{\mathsf{R}}}
\newcommand{\bsfS} {\boldsymbol{\mathsf{S}}}
\newcommand{\bsfT} {\boldsymbol{\mathsf{T}}}
\newcommand{\bsfU} {\boldsymbol{\mathsf{U}}}
\newcommand{\bsfV} {\boldsymbol{\mathsf{V}}}
\newcommand{\bsfW} {\boldsymbol{\mathsf{W}}}
\newcommand{\bsfX} {\boldsymbol{\mathsf{X}}}
\newcommand{\bsfY} {\boldsymbol{\mathsf{Y}}}
\newcommand{\bsfZ} {\boldsymbol{\mathsf{Z}}}

\newcommand{\bsfa} {\boldsymbol{\mathsf{a}}}
\newcommand{\bsfb} {\boldsymbol{\mathsf{b}}}
\newcommand{\bsfc} {\boldsymbol{\mathsf{c}}}
\newcommand{\bsfd} {\boldsymbol{\mathsf{d}}}
\newcommand{\bsfe} {\boldsymbol{\mathsf{e}}}
\newcommand{\bsff} {\boldsymbol{\mathsf{f}}}
\newcommand{\bsfg} {\boldsymbol{\mathsf{g}}}
\newcommand{\bsfh} {\boldsymbol{\mathsf{h}}}
\newcommand{\bsfi} {\boldsymbol{\mathsf{i}}}
\newcommand{\bsfj} {\boldsymbol{\mathsf{j}}}
\newcommand{\bsfk} {\boldsymbol{\mathsf{k}}}
\newcommand{\bsfl} {\boldsymbol{\mathsf{l}}}
\newcommand{\bsfm} {\boldsymbol{\mathsf{m}}}
\newcommand{\bsfn} {\boldsymbol{\mathsf{n}}}
\newcommand{\bsfo} {\boldsymbol{\mathsf{o}}}
\newcommand{\bsfp} {\boldsymbol{\mathsf{p}}}
\newcommand{\bsfq} {\boldsymbol{\mathsf{q}}}
\newcommand{\bsfr} {\boldsymbol{\mathsf{r}}}
\newcommand{\bsfs} {\boldsymbol{\mathsf{s}}}
\newcommand{\bsft} {\boldsymbol{\mathsf{t}}}
\newcommand{\bsfu} {\boldsymbol{\mathsf{u}}}
\newcommand{\bsfv} {\boldsymbol{\mathsf{v}}}
\newcommand{\bsfw} {\boldsymbol{\mathsf{w}}}
\newcommand{\bsfx} {\boldsymbol{\mathsf{x}}}
\newcommand{\bsfy} {\boldsymbol{\mathsf{y}}}
\newcommand{\bsfz} {\boldsymbol{\mathsf{z}}}
%  ---------------------
%  Colored letters (red)
%  ---------------------

\newcommand{\bfaR} {\RBmath{a}}
\newcommand{\bfbR} {\RBmath{b}}
\newcommand{\bfcR} {\RBmath{c}}
\newcommand{\bfdR} {\RBmath{d}}
\newcommand{\bfeR} {\RBmath{e}}
\newcommand{\bffR} {\RBmath{f}}
\newcommand{\bfgR} {\RBmath{g}}
\newcommand{\bfhR} {\RBmath{h}}
\newcommand{\bfjR} {\RBmath{j}}
\newcommand{\bfkR} {\RBmath{k}}
\newcommand{\bflR} {\RBmath{\ell}}
\newcommand{\bfmR} {\RBmath{m}}
\newcommand{\bfnR} {\RBmath{n}}
\newcommand{\bfoR} {\RBmath{o}}
\newcommand{\bfpR} {\RBmath{p}}
\newcommand{\bfqR} {\RBmath{q}}
\newcommand{\bfrR} {\RBmath{r}}
\newcommand{\bfsR} {\RBmath{s}}
\newcommand{\bftR} {\RBmath{t}}
\newcommand{\bfuR} {\RBmath{u}}
\newcommand{\bfvR} {\RBmath{v}}
\newcommand{\bfwR} {\RBmath{w}}
\newcommand{\bfxR} {\RBmath{x}}
\newcommand{\bfyR} {\RBmath{y}}
\newcommand{\bfzR} {\RBmath{z}}
\newcommand{\bfAR} {\RBmath{A}}
\newcommand{\bfBR} {\RBmath{B}}
\newcommand{\bfCR} {\RBmath{C}}
\newcommand{\bfDR} {\RBmath{D}}
\newcommand{\bfER} {\RBmath{E}}
\newcommand{\bfFR} {\RBmath{F}}
\newcommand{\bfGR} {\RBmath{G}}
\newcommand{\bfHR} {\RBmath{H}}
\newcommand{\bfIR} {\RBmath{I}}
\newcommand{\bfJR} {\RBmath{J}}
\newcommand{\bfKR} {\RBmath{K}}
\newcommand{\bfLR} {\RBmath{L}}
\newcommand{\bfMR} {\RBmath{M}}
\newcommand{\bfNR} {\RBmath{N}}
\newcommand{\bfOR} {\RBmath{O}}
\newcommand{\bfPR} {\RBmath{P}}
\newcommand{\bfQR} {\RBmath{Q}}
\newcommand{\bfRR} {\RBmath{R}}
\newcommand{\bfSR} {\RBmath{S}}
\newcommand{\bfTR} {\RBmath{T}}
\newcommand{\bfUR} {\RBmath{U}}
\newcommand{\bfVR} {\RBmath{V}}
\newcommand{\bfWR} {\RBmath{W}}
\newcommand{\bfXR} {\RBmath{X}}
\newcommand{\bfYR} {\RBmath{Y}}
\newcommand{\bfZR} {\RBmath{Z}}
%  -----------------------
%  Colored letters (green)
%  -----------------------

\newcommand{\bfaG} {\GBmath{a}}
\newcommand{\bfbG} {\GBmath{b}}
\newcommand{\bfcG} {\GBmath{c}}
\newcommand{\bfdG} {\GBmath{d}}
\newcommand{\bfeG} {\GBmath{e}}
\newcommand{\bffG} {\GBmath{f}}
\newcommand{\bfgG} {\GBmath{g}}
\newcommand{\bfhG} {\GBmath{h}}
\newcommand{\bfjG} {\GBmath{j}}
\newcommand{\bfkG} {\GBmath{k}}
\newcommand{\bflG} {\GBmath{\ell}}
\newcommand{\bfmG} {\GBmath{m}}
\newcommand{\bfnG} {\GBmath{n}}
\newcommand{\bfoG} {\GBmath{o}}
\newcommand{\bfpG} {\GBmath{p}}
\newcommand{\bfqG} {\GBmath{q}}
\newcommand{\bfrG} {\GBmath{r}}
\newcommand{\bfsG} {\GBmath{s}}
\newcommand{\bftG} {\GBmath{t}}
\newcommand{\bfuG} {\GBmath{u}}
\newcommand{\bfvG} {\GBmath{v}}
\newcommand{\bfwG} {\GBmath{w}}
\newcommand{\bfxG} {\GBmath{x}}
\newcommand{\bfyG} {\GBmath{y}}
\newcommand{\bfzG} {\GBmath{z}}
\newcommand{\bfAG} {\GBmath{A}}
\newcommand{\bfBG} {\GBmath{B}}
\newcommand{\bfCG} {\GBmath{C}}
\newcommand{\bfDG} {\GBmath{D}}
\newcommand{\bfEG} {\GBmath{E}}
\newcommand{\bfFG} {\GBmath{F}}
\newcommand{\bfGG} {\GBmath{G}}
\newcommand{\bfHG} {\GBmath{H}}
\newcommand{\bfIG} {\GBmath{I}}
\newcommand{\bfJG} {\GBmath{J}}
\newcommand{\bfKG} {\GBmath{K}}
\newcommand{\bfLG} {\GBmath{L}}
\newcommand{\bfMG} {\GBmath{M}}
\newcommand{\bfNG} {\GBmath{N}}
\newcommand{\bfOG} {\GBmath{O}}
\newcommand{\bfPG} {\GBmath{P}}
\newcommand{\bfQG} {\GBmath{Q}}
\newcommand{\bfRG} {\GBmath{R}}
\newcommand{\bfSG} {\GBmath{S}}
\newcommand{\bfTG} {\GBmath{T}}
\newcommand{\bfUG} {\GBmath{U}}
\newcommand{\bfVG} {\GBmath{V}}
\newcommand{\bfWG} {\GBmath{W}}
\newcommand{\bfXG} {\GBmath{X}}
\newcommand{\bfYG} {\GBmath{Y}}
\newcommand{\bfZG} {\GBmath{Z}}
%  ----------------------
%  Colored letters (blue)
%  ----------------------

\newcommand{\bfaBB} {\BBmath{a}}
\newcommand{\bfbBB} {\BBmath{b}}
\newcommand{\bfcBB} {\BBmath{c}}
\newcommand{\bfdBB} {\BBmath{d}}
\newcommand{\bfeBB} {\BBmath{e}}
\newcommand{\bffBB} {\BBmath{f}}
\newcommand{\bfgBB} {\BBmath{g}}
\newcommand{\bfhBB} {\BBmath{h}}
\newcommand{\bfjBB} {\BBmath{j}}
\newcommand{\bfkBB} {\BBmath{k}}
\newcommand{\bflBB} {\BBmath{\ell}}
\newcommand{\bfmBB} {\BBmath{m}}
\newcommand{\bfnBB} {\BBmath{n}}
\newcommand{\bfoBB} {\BBmath{o}}
\newcommand{\bfpBB} {\BBmath{p}}
\newcommand{\bfqBB} {\BBmath{q}}
\newcommand{\bfrBB} {\BBmath{r}}
\newcommand{\bfsBB} {\BBmath{s}}
\newcommand{\bftBB} {\BBmath{t}}
\newcommand{\bfuBB} {\BBmath{u}}
\newcommand{\bfvBB} {\BBmath{v}}
\newcommand{\bfwBB} {\BBmath{w}}
\newcommand{\bfxBB} {\BBmath{x}}
\newcommand{\bfyBB} {\BBmath{y}}
\newcommand{\bfzBB} {\BBmath{z}}
\newcommand{\bfABB} {\BBmath{A}}
\newcommand{\bfBBB} {\BBmath{B}}
\newcommand{\bfCBB} {\BBmath{C}}
\newcommand{\bfDBB} {\BBmath{D}}
\newcommand{\bfEBB} {\BBmath{E}}
\newcommand{\bfFBB} {\BBmath{F}}
\newcommand{\bfGBB} {\BBmath{G}}
\newcommand{\bfHBB} {\BBmath{H}}
\newcommand{\bfIBB} {\BBmath{I}}
\newcommand{\bfJBB} {\BBmath{J}}
\newcommand{\bfKBB} {\BBmath{K}}
\newcommand{\bfLBB} {\BBmath{L}}
\newcommand{\bfMBB} {\BBmath{M}}
\newcommand{\bfNBB} {\BBmath{N}}
\newcommand{\bfOBB} {\BBmath{O}}
\newcommand{\bfPBB} {\BBmath{P}}
\newcommand{\bfQBB} {\BBmath{Q}}
\newcommand{\bfRBB} {\BBmath{R}}
\newcommand{\bfSBB} {\BBmath{S}}
\newcommand{\bfTBB} {\BBmath{T}}
\newcommand{\bfUBB} {\BBmath{U}}
\newcommand{\bfVBB} {\BBmath{V}}
\newcommand{\bfWBB} {\BBmath{W}}
\newcommand{\bfXBB} {\BBmath{X}}
\newcommand{\bfYBB} {\BBmath{Y}}
\newcommand{\bfZBB} {\BBmath{Z}}
%  -----------------------
%  Roman letters, boldmath
%  -----------------------

\newcommand{\bfa} {\boldsymbol{a}}
\newcommand{\bfb} {\boldsymbol{b}}
\newcommand{\bfc} {\boldsymbol{c}}
\newcommand{\bfd} {\boldsymbol{d}}
\newcommand{\bfe} {\boldsymbol{e}}
\newcommand{\bff} {\boldsymbol{f}}
\newcommand{\bfg} {\boldsymbol{g}}
\newcommand{\bfh} {\boldsymbol{h}}
\newcommand{\bfj} {\boldsymbol{j}}
\newcommand{\bfk} {\boldsymbol{k}}
\newcommand{\bfl} {\boldsymbol{\ell}}
\newcommand{\bfm} {\boldsymbol{m}}
\newcommand{\bfn} {\boldsymbol{n}}
\newcommand{\bfo} {\boldsymbol{o}}
\newcommand{\bfp} {\boldsymbol{p}}
\newcommand{\bfq} {\boldsymbol{q}}
\newcommand{\bfr} {\boldsymbol{r}}
\newcommand{\bfs} {\boldsymbol{s}}
\newcommand{\bft} {\boldsymbol{t}}
\newcommand{\bfu} {\boldsymbol{u}}
\newcommand{\bfv} {\boldsymbol{v}}
\newcommand{\bfw} {\boldsymbol{w}}
\newcommand{\bfx} {\boldsymbol{x}}
\newcommand{\bfy} {\boldsymbol{y}}
\newcommand{\bfz} {\boldsymbol{z}}
\newcommand{\bfA} {\boldsymbol{A}}
\newcommand{\bfB} {\boldsymbol{B}}
\newcommand{\bfC} {\boldsymbol{C}}
\newcommand{\bfD} {\boldsymbol{D}}
\newcommand{\bfE} {\boldsymbol{E}}
\newcommand{\bfF} {\boldsymbol{F}}
\newcommand{\bfG} {\boldsymbol{G}}
\newcommand{\bfH} {\boldsymbol{H}}
\newcommand{\bfI} {\boldsymbol{I}}
\newcommand{\bfJ} {\boldsymbol{J}}
\newcommand{\bfK} {\boldsymbol{K}}
\newcommand{\bfL} {\boldsymbol{L}}
\newcommand{\bfM} {\boldsymbol{M}}
\newcommand{\bfN} {\boldsymbol{N}}
\newcommand{\bfO} {\boldsymbol{O}}
\newcommand{\bfP} {\boldsymbol{P}}
\newcommand{\bfQ} {\boldsymbol{Q}}
\newcommand{\bfR} {\boldsymbol{R}}
\newcommand{\bfS} {\boldsymbol{S}}
\newcommand{\bfT} {\boldsymbol{T}}
\newcommand{\bfU} {\boldsymbol{U}}
\newcommand{\bfV} {\boldsymbol{V}}
\newcommand{\bfW} {\boldsymbol{W}}
\newcommand{\bfX} {\boldsymbol{X}}
\newcommand{\bfY} {\boldsymbol{Y}}
\newcommand{\bfZ} {\boldsymbol{Z}}
%  --------------
%  Tilded letters
%  --------------

\newcommand{\TilA}{\widetilde{A}}
\newcommand{\TilB}{\widetilde{B}}
\newcommand{\TilC}{\widetilde{C}}
\newcommand{\TilD}{\widetilde{D}}
\newcommand{\TilE}{\widetilde{E}}
\newcommand{\TilF}{\widetilde{F}}
\newcommand{\TilG}{\widetilde{G}}
\newcommand{\TilH}{\widetilde{H}}
\newcommand{\TilI}{\widetilde{I}}
\newcommand{\TilJ}{\widetilde{J}}
\newcommand{\TilK}{\widetilde{K}}
\newcommand{\TilL}{\widetilde{L}}
\newcommand{\TilM}{\widetilde{M}}
\newcommand{\TilN}{\widetilde{N}}
\newcommand{\TilO}{\widetilde{O}}
\newcommand{\TilP}{\widetilde{P}}
\newcommand{\TilQ}{\widetilde{Q}}
\newcommand{\TilR}{\widetilde{R}}
\newcommand{\TilS}{\widetilde{S}}
\newcommand{\TilT}{\widetilde{T}}
\newcommand{\TilU}{\widetilde{U}}
\newcommand{\TilV}{\widetilde{V}}
\newcommand{\TilW}{\widetilde{W}}
\newcommand{\TilX}{\widetilde{X}}
\newcommand{\TilY}{\widetilde{Y}}
\newcommand{\TilZ}{\widetilde{Z}}

\newcommand{\Tila}{\widetilde{a}}
\newcommand{\Tilb}{\widetilde{b}}
\newcommand{\Tilc}{\widetilde{c}}
\newcommand{\Tild}{\widetilde{d}}
\newcommand{\Tile}{\widetilde{e}}
\newcommand{\Tilf}{\widetilde{f}}
\newcommand{\Tilg}{\widetilde{g}}
\newcommand{\Tilh}{\widetilde{h}}
\newcommand{\Tili}{\widetilde{i}}
\newcommand{\Tilj}{\widetilde{j}}
\newcommand{\Tilk}{\widetilde{k}}
\newcommand{\Till}{\widetilde{l}}
\newcommand{\Tilm}{\widetilde{m}}
\newcommand{\Tiln}{\widetilde{n}}
\newcommand{\Tilo}{\widetilde{o}}
\newcommand{\Tilp}{\widetilde{p}}
\newcommand{\Tilq}{\widetilde{q}}
\newcommand{\Tilr}{\widetilde{r}}
\newcommand{\Tils}{\widetilde{s}}
\newcommand{\Tilt}{\widetilde{t}}
\newcommand{\Tilu}{\widetilde{u}}
\newcommand{\Tilv}{\widetilde{v}}
\newcommand{\Tilw}{\widetilde{w}}
\newcommand{\Tilx}{\widetilde{x}}
\newcommand{\Tily}{\widetilde{y}}
\newcommand{\Tilz}{\widetilde{z}}

\newcommand{\tilA}{\tilde{A}}
\newcommand{\tilB}{\tilde{B}}
\newcommand{\tilC}{\tilde{C}}
\newcommand{\tilD}{\tilde{D}}
\newcommand{\tilE}{\tilde{E}}
\newcommand{\tilF}{\tilde{F}}
\newcommand{\tilG}{\tilde{G}}
\newcommand{\tilH}{\tilde{H}}
\newcommand{\tilI}{\tilde{I}}
\newcommand{\tilJ}{\tilde{J}}
\newcommand{\tilK}{\tilde{K}}
\newcommand{\tilL}{\tilde{L}}
\newcommand{\tilM}{\tilde{M}}
\newcommand{\tilN}{\tilde{N}}
\newcommand{\tilO}{\tilde{O}}
\newcommand{\tilP}{\tilde{P}}
\newcommand{\tilQ}{\tilde{Q}}
\newcommand{\tilR}{\tilde{R}}
\newcommand{\tilS}{\tilde{S}}
\newcommand{\tilT}{\tilde{T}}
\newcommand{\tilU}{\tilde{U}}
\newcommand{\tilV}{\tilde{V}}
\newcommand{\tilW}{\tilde{W}}
\newcommand{\tilX}{\tilde{X}}
\newcommand{\tilY}{\tilde{Y}}
\newcommand{\tilZ}{\tilde{Z}}

\newcommand{\tila}{\tilde{a}}
\newcommand{\tilb}{\tilde{b}}
\newcommand{\tilc}{\tilde{c}}
\providecommand{\tild}{\tilde{d}}
\newcommand{\tile}{\tilde{e}}
\newcommand{\tilf}{\tilde{f}}
\newcommand{\tilg}{\tilde{g}}
\newcommand{\tilh}{\tilde{h}}
\newcommand{\tili}{\tilde{i}}
\newcommand{\tilj}{\tilde{j}}
\newcommand{\tilk}{\tilde{k}}
\newcommand{\till}{\tilde{l}}
\newcommand{\tilm}{\tilde{m}}
\newcommand{\tiln}{\tilde{n}}
\newcommand{\tilo}{\tilde{o}}
\newcommand{\tilp}{\tilde{p}}
\newcommand{\tilq}{\tilde{q}}
\newcommand{\tilr}{\tilde{r}}
\newcommand{\tils}{\tilde{s}}
\newcommand{\tilt}{\tilde{t}}
\newcommand{\tilu}{\tilde{u}}
\newcommand{\tilv}{\tilde{v}}
\newcommand{\tilw}{\tilde{w}}
\newcommand{\tilx}{\tilde{x}}
\newcommand{\tily}{\tilde{y}}
\newcommand{\tilz}{\tilde{z}}
%  ---------------------
%  Hat letters, boldface
%  ---------------------

\newcommand{\brah} {\hat{\mathbf{a}}{}}
\newcommand{\brbh} {\hat{\mathbf{b}}{}}
\newcommand{\brch} {\hat{\mathbf{c}}{}}
\newcommand{\brdh} {\hat{\mathbf{d}}{}}
\newcommand{\breh} {\hat{\mathbf{e}}{}}
\newcommand{\brfh} {\hat{\mathbf{f}}{}}
\newcommand{\brgh} {\hat{\mathbf{g}}{}}
\newcommand{\brhh} {\hat{\mathbf{h}}{}}
\newcommand{\brih} {\hat{\mathbf{\imath}}{}}
\newcommand{\brjh} {\hat{\mathbf{\jmath}}{}}
\newcommand{\brkh} {\hat{\mathbf{k}}{}}
\newcommand{\brlh} {\hat{\mathbf{\ell}}{}}
\newcommand{\brmh} {\hat{\mathbf{m}}{}}
\newcommand{\brnh} {\hat{\mathbf{n}}{}}
\newcommand{\broh} {\hat{\mathbf{o}}{}}
\newcommand{\brph} {\hat{\mathbf{p}}{}}
\newcommand{\brqh} {\hat{\mathbf{q}}{}}
\newcommand{\brrh} {\hat{\mathbf{r}}{}}
\newcommand{\brsh} {\hat{\mathbf{s}}{}}
\newcommand{\brth} {\hat{\mathbf{t}}{}}
\newcommand{\bruh} {\hat{\mathbf{u}}{}}
\newcommand{\brvh} {\hat{\mathbf{v}}{}}
\newcommand{\brwh} {\hat{\mathbf{w}}{}}
\newcommand{\brxh} {\hat{\mathbf{x}}{}}
\newcommand{\bryh} {\hat{\mathbf{y}}{}}
\newcommand{\brzh} {\hat{\mathbf{z}}{}}

\newcommand{\brAh} {\hat{\mathbf{A}}{}}
\newcommand{\brBh} {\hat{\mathbf{B}}{}}
\newcommand{\brCh} {\hat{\mathbf{C}}{}}
\newcommand{\brDh} {\hat{\mathbf{D}}{}}
\newcommand{\brEh} {\hat{\mathbf{E}}{}}
\newcommand{\brFh} {\hat{\mathbf{F}}{}}
\newcommand{\brGh} {\hat{\mathbf{G}}{}}
\newcommand{\brHh} {\hat{\mathbf{H}}{}}
\newcommand{\brIh} {\hat{\mathbf{I}}{}}
\newcommand{\brJh} {\hat{\mathbf{J}}{}}
\newcommand{\brKh} {\hat{\mathbf{K}}{}}
\newcommand{\brLh} {\hat{\mathbf{L}}{}}
\newcommand{\brMh} {\hat{\mathbf{M}}{}}
\newcommand{\brNh} {\hat{\mathbf{N}}{}}
\newcommand{\brOh} {\hat{\mathbf{O}}{}}
\newcommand{\brPh} {\hat{\mathbf{P}}{}}
\newcommand{\brQh} {\hat{\mathbf{Q}}{}}
\newcommand{\brRh} {\hat{\mathbf{R}}{}}
\newcommand{\brSh} {\hat{\mathbf{S}}{}}
\newcommand{\brTh} {\hat{\mathbf{T}}{}}
\newcommand{\brUh} {\hat{\mathbf{U}}{}}
\newcommand{\brVh} {\hat{\mathbf{V}}{}}
\newcommand{\brWh} {\hat{\mathbf{W}}{}}
\newcommand{\brXh} {\hat{\mathbf{X}}{}}
\newcommand{\brYh} {\hat{\mathbf{Y}}{}}
\newcommand{\brZh} {\hat{\mathbf{Z}}{}}

\newcommand{\braH} {\widehat{\mathbf{a}}{}}
\newcommand{\brbH} {\widehat{\mathbf{b}}{}}
\newcommand{\brcH} {\widehat{\mathbf{c}}{}}
\newcommand{\brdH} {\widehat{\mathbf{d}}{}}
\newcommand{\breH} {\widehat{\mathbf{e}}{}}
\newcommand{\brfH} {\widehat{\mathbf{f}}{}}
\newcommand{\brgH} {\widehat{\mathbf{g}}{}}
\newcommand{\brhH} {\widehat{\mathbf{h}}{}}
\newcommand{\briH} {\widehat{\mathbf{\imath}}{}}
\newcommand{\brjH} {\widehat{\mathbf{\jmath}}{}}
\newcommand{\brkH} {\widehat{\mathbf{k}}{}}
\newcommand{\brlH} {\widehat{\mathbf{\ell}}{}}
\newcommand{\brmH} {\widehat{\mathbf{m}}{}}
\newcommand{\brnH} {\widehat{\mathbf{n}}{}}
\newcommand{\broH} {\widehat{\mathbf{o}}{}}
\newcommand{\brpH} {\widehat{\mathbf{p}}{}}
\newcommand{\brqH} {\widehat{\mathbf{q}}{}}
\newcommand{\brrH} {\widehat{\mathbf{r}}{}}
\newcommand{\brsH} {\widehat{\mathbf{s}}{}}
\newcommand{\brtH} {\widehat{\mathbf{t}}{}}
\newcommand{\bruH} {\widehat{\mathbf{u}}{}}
\newcommand{\brvH} {\widehat{\mathbf{v}}{}}
\newcommand{\brwH} {\widehat{\mathbf{w}}{}}
\newcommand{\brxH} {\widehat{\mathbf{x}}{}}
\newcommand{\bryH} {\widehat{\mathbf{y}}{}}
\newcommand{\brzH} {\widehat{\mathbf{z}}{}}

\newcommand{\brAH} {\widehat{\mathbf{A}}{}}
\newcommand{\brBH} {\widehat{\mathbf{B}}{}}
\newcommand{\brCH} {\widehat{\mathbf{C}}{}}
\newcommand{\brDH} {\widehat{\mathbf{D}}{}}
\newcommand{\brEH} {\widehat{\mathbf{E}}{}}
\newcommand{\brFH} {\widehat{\mathbf{F}}{}}
\newcommand{\brGH} {\widehat{\mathbf{G}}{}}
\newcommand{\brHH} {\widehat{\mathbf{H}}{}}
\newcommand{\brIH} {\widehat{\mathbf{I}}{}}
\newcommand{\brJH} {\widehat{\mathbf{J}}{}}
\newcommand{\brKH} {\widehat{\mathbf{K}}{}}
\newcommand{\brLH} {\widehat{\mathbf{L}}{}}
\newcommand{\brMH} {\widehat{\mathbf{M}}{}}
\newcommand{\brNH} {\widehat{\mathbf{N}}{}}
\newcommand{\brOH} {\widehat{\mathbf{O}}{}}
\newcommand{\brPH} {\widehat{\mathbf{P}}{}}
\newcommand{\brQH} {\widehat{\mathbf{Q}}{}}
\newcommand{\brRH} {\widehat{\mathbf{R}}{}}
\newcommand{\brSH} {\widehat{\mathbf{S}}{}}
\newcommand{\brTH} {\widehat{\mathbf{T}}{}}
\newcommand{\brUH} {\widehat{\mathbf{U}}{}}
\newcommand{\brVH} {\widehat{\mathbf{V}}{}}
\newcommand{\brWH} {\widehat{\mathbf{W}}{}}
\newcommand{\brXH} {\widehat{\mathbf{X}}{}}
\newcommand{\brYH} {\widehat{\mathbf{Y}}{}}
\newcommand{\brZH} {\widehat{\mathbf{Z}}{}}
%  ---------------------
%  Hat letters, boldface
%  ---------------------

\newcommand{\brat} {\tilde{\mathbf{a}}{}}
\newcommand{\brbt} {\tilde{\mathbf{b}}{}}
\newcommand{\brct} {\tilde{\mathbf{c}}{}}
\newcommand{\brdt} {\tilde{\mathbf{d}}{}}
\newcommand{\bret} {\tilde{\mathbf{e}}{}}
\newcommand{\brft} {\tilde{\mathbf{f}}{}}
\newcommand{\brgt} {\tilde{\mathbf{g}}{}}
\newcommand{\brht} {\tilde{\mathbf{h}}{}}
\newcommand{\brit} {\tilde{\mathbf{\imath}}{}}
\newcommand{\brjt} {\tilde{\mathbf{\jmath}}{}}
\newcommand{\brkt} {\tilde{\mathbf{k}}{}}
\newcommand{\brlt} {\tilde{\mathbf{\ell}}{}}
\newcommand{\brmt} {\tilde{\mathbf{m}}{}}
\newcommand{\brnt} {\tilde{\mathbf{n}}{}}
\newcommand{\brot} {\tilde{\mathbf{o}}{}}
\newcommand{\brpt} {\tilde{\mathbf{p}}{}}
\newcommand{\brqt} {\tilde{\mathbf{q}}{}}
\newcommand{\brrt} {\tilde{\mathbf{r}}{}}
\newcommand{\brst} {\tilde{\mathbf{s}}{}}
\newcommand{\brtt} {\tilde{\mathbf{t}}{}}
\newcommand{\brut} {\tilde{\mathbf{u}}{}}
\newcommand{\brvt} {\tilde{\mathbf{v}}{}}
\newcommand{\brwt} {\tilde{\mathbf{w}}{}}
\newcommand{\brxt} {\tilde{\mathbf{x}}{}}
\newcommand{\bryt} {\tilde{\mathbf{y}}{}}
\newcommand{\brzt} {\tilde{\mathbf{z}}{}}

\newcommand{\brAt} {\tilde{\mathbf{A}}{}}
\newcommand{\brBt} {\tilde{\mathbf{B}}{}}
\newcommand{\brCt} {\tilde{\mathbf{C}}{}}
\newcommand{\brDt} {\tilde{\mathbf{D}}{}}
\newcommand{\brEt} {\tilde{\mathbf{E}}{}}
\newcommand{\brFt} {\tilde{\mathbf{F}}{}}
\newcommand{\brGt} {\tilde{\mathbf{G}}{}}
\newcommand{\brHt} {\tilde{\mathbf{H}}{}}
\newcommand{\brIt} {\tilde{\mathbf{I}}{}}
\newcommand{\brJt} {\tilde{\mathbf{J}}{}}
\newcommand{\brKt} {\tilde{\mathbf{K}}{}}
\newcommand{\brLt} {\tilde{\mathbf{L}}{}}
\newcommand{\brMt} {\tilde{\mathbf{M}}{}}
\newcommand{\brNt} {\tilde{\mathbf{N}}{}}
\newcommand{\brOt} {\tilde{\mathbf{O}}{}}
\newcommand{\brPt} {\tilde{\mathbf{P}}{}}
\newcommand{\brQt} {\tilde{\mathbf{Q}}{}}
\newcommand{\brRt} {\tilde{\mathbf{R}}{}}
\newcommand{\brSt} {\tilde{\mathbf{S}}{}}
\newcommand{\brTt} {\tilde{\mathbf{T}}{}}
\newcommand{\brUt} {\tilde{\mathbf{U}}{}}
\newcommand{\brVt} {\tilde{\mathbf{V}}{}}
\newcommand{\brWt} {\tilde{\mathbf{W}}{}}
\newcommand{\brXt} {\tilde{\mathbf{X}}{}}
\newcommand{\brYt} {\tilde{\mathbf{Y}}{}}
\newcommand{\brZt} {\tilde{\mathbf{Z}}{}}

\newcommand{\braT} {\widetilde{\mathbf{a}}{}}
\newcommand{\brbT} {\widetilde{\mathbf{b}}{}}
\newcommand{\brcT} {\widetilde{\mathbf{c}}{}}
\newcommand{\brdT} {\widetilde{\mathbf{d}}{}}
\newcommand{\breT} {\widetilde{\mathbf{e}}{}}
\newcommand{\brfT} {\widetilde{\mathbf{f}}{}}
\newcommand{\brgT} {\widetilde{\mathbf{g}}{}}
\newcommand{\brhT} {\widetilde{\mathbf{h}}{}}
\newcommand{\briT} {\widetilde{\mathbf{\imath}}{}}
\newcommand{\brjT} {\widetilde{\mathbf{\jmath}}{}}
\newcommand{\brkT} {\widetilde{\mathbf{k}}{}}
\newcommand{\brlT} {\widetilde{\mathbf{\ell}}{}}
\newcommand{\brmT} {\widetilde{\mathbf{m}}{}}
\newcommand{\brnT} {\widetilde{\mathbf{n}}{}}
\newcommand{\broT} {\widetilde{\mathbf{o}}{}}
\newcommand{\brpT} {\widetilde{\mathbf{p}}{}}
\newcommand{\brqT} {\widetilde{\mathbf{q}}{}}
\newcommand{\brrT} {\widetilde{\mathbf{r}}{}}
\newcommand{\brsT} {\widetilde{\mathbf{s}}{}}
\newcommand{\brtT} {\widetilde{\mathbf{t}}{}}
\newcommand{\bruT} {\widetilde{\mathbf{u}}{}}
\newcommand{\brvT} {\widetilde{\mathbf{v}}{}}
\newcommand{\brwT} {\widetilde{\mathbf{w}}{}}
\newcommand{\brxT} {\widetilde{\mathbf{x}}{}}
\newcommand{\bryT} {\widetilde{\mathbf{y}}{}}
\newcommand{\brzT} {\widetilde{\mathbf{z}}{}}

\newcommand{\brAT} {\widetilde{\mathbf{A}}{}}
\newcommand{\brBT} {\widetilde{\mathbf{B}}{}}
\newcommand{\brCT} {\widetilde{\mathbf{C}}{}}
\newcommand{\brDT} {\widetilde{\mathbf{D}}{}}
\newcommand{\brET} {\widetilde{\mathbf{E}}{}}
\newcommand{\brFT} {\widetilde{\mathbf{F}}{}}
\newcommand{\brGT} {\widetilde{\mathbf{G}}{}}
\newcommand{\brHT} {\widetilde{\mathbf{H}}{}}
\newcommand{\brIT} {\widetilde{\mathbf{I}}{}}
\newcommand{\brJT} {\widetilde{\mathbf{J}}{}}
\newcommand{\brKT} {\widetilde{\mathbf{K}}{}}
\newcommand{\brLT} {\widetilde{\mathbf{L}}{}}
\newcommand{\brMT} {\widetilde{\mathbf{M}}{}}
\newcommand{\brNT} {\widetilde{\mathbf{N}}{}}
\newcommand{\brOT} {\widetilde{\mathbf{O}}{}}
\newcommand{\brPT} {\widetilde{\mathbf{P}}{}}
\newcommand{\brQT} {\widetilde{\mathbf{Q}}{}}
\newcommand{\brRT} {\widetilde{\mathbf{R}}{}}
\newcommand{\brST} {\widetilde{\mathbf{S}}{}}
\newcommand{\brTT} {\widetilde{\mathbf{T}}{}}
\newcommand{\brUT} {\widetilde{\mathbf{U}}{}}
\newcommand{\brVT} {\widetilde{\mathbf{V}}{}}
\newcommand{\brWT} {\widetilde{\mathbf{W}}{}}
\newcommand{\brXT} {\widetilde{\mathbf{X}}{}}
\newcommand{\brYT} {\widetilde{\mathbf{Y}}{}}
\newcommand{\brZT} {\widetilde{\mathbf{Z}}{}}
%  -------------------------------
%  Hat letters, sansserif boldface
%  -------------------------------

\newcommand{\bsfah} {\hat{\bsfa}}
\newcommand{\bsfbh} {\hat{\bsfb}}
\newcommand{\bsfch} {\hat{\bsfc}}
\newcommand{\bsfdh} {\hat{\bsfd}}
\newcommand{\bsfeh} {\hat{\bsfe}}
\newcommand{\bsffh} {\hat{\bsff}}
\newcommand{\bsfgh} {\hat{\bsfg}}
\newcommand{\bsfhh} {\hat{\bsfh}}
\newcommand{\bsfih} {\hat{\bsfi}}
\newcommand{\bsfjh} {\hat{\bsfj}}
\newcommand{\bsfkh} {\hat{\bsfk}}
\newcommand{\bsflh} {\hat{\bsfl}}
\newcommand{\bsfmh} {\hat{\bsfm}}
\newcommand{\bsfnh} {\hat{\bsfn}}
\newcommand{\bsfoh} {\hat{\bsfo}}
\newcommand{\bsfph} {\hat{\bsfp}}
\newcommand{\bsfqh} {\hat{\bsfq}}
\newcommand{\bsfrh} {\hat{\bsfr}}
\newcommand{\bsfsh} {\hat{\bsfs}}
\newcommand{\bsfth} {\hat{\bsft}}
\newcommand{\bsfuh} {\hat{\bsfu}}
\newcommand{\bsfvh} {\hat{\bsfv}}
\newcommand{\bsfwh} {\hat{\bsfw}}
\newcommand{\bsfxh} {\hat{\bsfx}}
\newcommand{\bsfyh} {\hat{\bsfy}}
\newcommand{\bsfzh} {\hat{\bsfz}}

\newcommand{\bsfaH} {\widehat{\bsfa}}
\newcommand{\bsfbH} {\widehat{\bsfb}}
\newcommand{\bsfcH} {\widehat{\bsfc}}
\newcommand{\bsfdH} {\widehat{\bsfd}}
\newcommand{\bsfeH} {\widehat{\bsfe}}
\newcommand{\bsffH} {\widehat{\bsff}}
\newcommand{\bsfgH} {\widehat{\bsfg}}
\newcommand{\bsfhH} {\widehat{\bsfh}}
\newcommand{\bsfiH} {\widehat{\bsfi}}
\newcommand{\bsfjH} {\widehat{\bsfj}}
\newcommand{\bsfkH} {\widehat{\bsfk}}
\newcommand{\bsflH} {\widehat{\bsfl}}
\newcommand{\bsfmH} {\widehat{\bsfm}}
\newcommand{\bsfnH} {\widehat{\bsfn}}
\newcommand{\bsfoH} {\widehat{\bsfo}}
\newcommand{\bsfpH} {\widehat{\bsfp}}
\newcommand{\bsfqH} {\widehat{\bsfq}}
\newcommand{\bsfrH} {\widehat{\bsfr}}
\newcommand{\bsfsH} {\widehat{\bsfs}}
\newcommand{\bsftH} {\widehat{\bsft}}
\newcommand{\bsfuH} {\widehat{\bsfu}}
\newcommand{\bsfvH} {\widehat{\bsfv}}
\newcommand{\bsfwH} {\widehat{\bsfw}}
\newcommand{\bsfxH} {\widehat{\bsfx}}
\newcommand{\bsfyH} {\widehat{\bsfy}}
\newcommand{\bsfzH} {\widehat{\bsfz}}

\newcommand{\bsfAh} {\hat{\bsfA}}
\newcommand{\bsfBh} {\hat{\bsfB}}
\newcommand{\bsfCh} {\hat{\bsfC}}
\newcommand{\bsfDh} {\hat{\bsfD}}
\newcommand{\bsfEh} {\hat{\bsfE}}
\newcommand{\bsfFh} {\hat{\bsfF}}
\newcommand{\bsfGh} {\hat{\bsfG}}
\newcommand{\bsfHh} {\hat{\bsfH}}
\newcommand{\bsfIh} {\hat{\bsfI}}
\newcommand{\bsfJh} {\hat{\bsfJ}}
\newcommand{\bsfKh} {\hat{\bsfK}}
\newcommand{\bsfLh} {\hat{\bsfL}}
\newcommand{\bsfMh} {\hat{\bsfM}}
\newcommand{\bsfNh} {\hat{\bsfN}}
\newcommand{\bsfOh} {\hat{\bsfO}}
\newcommand{\bsfPh} {\hat{\bsfP}}
\newcommand{\bsfQh} {\hat{\bsfQ}}
\newcommand{\bsfRh} {\hat{\bsfR}}
\newcommand{\bsfSh} {\hat{\bsfS}}
\newcommand{\bsfTh} {\hat{\bsfT}}
\newcommand{\bsfUh} {\hat{\bsfU}}
\newcommand{\bsfVh} {\hat{\bsfV}}
\newcommand{\bsfWh} {\hat{\bsfW}}
\newcommand{\bsfXh} {\hat{\bsfX}}
\newcommand{\bsfYh} {\hat{\bsfY}}
\newcommand{\bsfZh} {\hat{\bsfZ}}

\newcommand{\bsfAH} {\widehat{\bsfA}}
\newcommand{\bsfBH} {\widehat{\bsfB}}
\newcommand{\bsfCH} {\widehat{\bsfC}}
\newcommand{\bsfDH} {\widehat{\bsfD}}
\newcommand{\bsfEH} {\widehat{\bsfE}}
\newcommand{\bsfFH} {\widehat{\bsfF}}
\newcommand{\bsfGH} {\widehat{\bsfG}}
\newcommand{\bsfHH} {\widehat{\bsfH}}
\newcommand{\bsfIH} {\widehat{\bsfI}}
\newcommand{\bsfJH} {\widehat{\bsfJ}}
\newcommand{\bsfKH} {\widehat{\bsfK}}
\newcommand{\bsfLH} {\widehat{\bsfL}}
\newcommand{\bsfMH} {\widehat{\bsfM}}
\newcommand{\bsfNH} {\widehat{\bsfN}}
\newcommand{\bsfOH} {\widehat{\bsfO}}
\newcommand{\bsfPH} {\widehat{\bsfP}}
\newcommand{\bsfQH} {\widehat{\bsfQ}}
\newcommand{\bsfRH} {\widehat{\bsfR}}
\newcommand{\bsfSH} {\widehat{\bsfS}}
\newcommand{\bsfTH} {\widehat{\bsfT}}
\newcommand{\bsfUH} {\widehat{\bsfU}}
\newcommand{\bsfVH} {\widehat{\bsfV}}
\newcommand{\bsfWH} {\widehat{\bsfW}}
\newcommand{\bsfXH} {\widehat{\bsfX}}
\newcommand{\bsfYH} {\widehat{\bsfY}}
\newcommand{\bsfZH} {\widehat{\bsfZ}}
%  -------------------------------
%  Hat letters, sansserif boldface
%  -------------------------------

\newcommand{\bsfab} {\bar{\bsfa}}
\newcommand{\bsfbb} {\bar{\bsfb}}
\newcommand{\bsfcb} {\bar{\bsfc}}
\newcommand{\bsfdb} {\bar{\bsfd}}
\newcommand{\bsfeb} {\bar{\bsfe}}
\newcommand{\bsffb} {\bar{\bsff}}
\newcommand{\bsfgb} {\bar{\bsfg}}
\newcommand{\bsfhb} {\bar{\bsfh}}
\newcommand{\bsfib} {\bar{\bsfi}}
\newcommand{\bsfjb} {\bar{\bsfj}}
\newcommand{\bsfkb} {\bar{\bsfk}}
\newcommand{\bsflb} {\bar{\bsfl}}
\newcommand{\bsfmb} {\bar{\bsfm}}
\newcommand{\bsfnb} {\bar{\bsfn}}
\newcommand{\bsfob} {\bar{\bsfo}}
\newcommand{\bsfpb} {\bar{\bsfp}}
\newcommand{\bsfqb} {\bar{\bsfq}}
\newcommand{\bsfrb} {\bar{\bsfr}}
\newcommand{\bsfsb} {\bar{\bsfs}}
\newcommand{\bsftb} {\bar{\bsft}}
\newcommand{\bsfub} {\bar{\bsfu}}
\newcommand{\bsfvb} {\bar{\bsfv}}
\newcommand{\bsfwb} {\bar{\bsfw}}
\newcommand{\bsfxb} {\bar{\bsfx}}
\newcommand{\bsfyb} {\bar{\bsfy}}
\newcommand{\bsfzb} {\bar{\bsfz}}

\newcommand{\bsfaB} {\overline{\bsfa}}
\newcommand{\bsfbB} {\overline{\bsfb}}
\newcommand{\bsfcB} {\overline{\bsfc}}
\newcommand{\bsfdB} {\overline{\bsfd}}
\newcommand{\bsfeB} {\overline{\bsfe}}
\newcommand{\bsffB} {\overline{\bsff}}
\newcommand{\bsfgB} {\overline{\bsfg}}
\newcommand{\bsfhB} {\overline{\bsfh}}
\newcommand{\bsfiB} {\overline{\bsfi}}
\newcommand{\bsfjB} {\overline{\bsfj}}
\newcommand{\bsfkB} {\overline{\bsfk}}
\newcommand{\bsflB} {\overline{\bsfl}}
\newcommand{\bsfmB} {\overline{\bsfm}}
\newcommand{\bsfnB} {\overline{\bsfn}}
\newcommand{\bsfoB} {\overline{\bsfo}}
\newcommand{\bsfpB} {\overline{\bsfp}}
\newcommand{\bsfqB} {\overline{\bsfq}}
\newcommand{\bsfrB} {\overline{\bsfr}}
\newcommand{\bsfsB} {\overline{\bsfs}}
\newcommand{\bsftB} {\overline{\bsft}}
\newcommand{\bsfuB} {\overline{\bsfu}}
\newcommand{\bsfvB} {\overline{\bsfv}}
\newcommand{\bsfwB} {\overline{\bsfw}}
\newcommand{\bsfxB} {\overline{\bsfx}}
\newcommand{\bsfyB} {\overline{\bsfy}}
\newcommand{\bsfzB} {\overline{\bsfz}}

\newcommand{\bsfAb} {\bar{\bsfA}}
\newcommand{\bsfBb} {\bar{\bsfB}}
\newcommand{\bsfCb} {\bar{\bsfC}}
\newcommand{\bsfDb} {\bar{\bsfD}}
\newcommand{\bsfEb} {\bar{\bsfE}}
\newcommand{\bsfFb} {\bar{\bsfF}}
\newcommand{\bsfGb} {\bar{\bsfG}}
\newcommand{\bsfHb} {\bar{\bsfH}}
\newcommand{\bsfIb} {\bar{\bsfI}}
\newcommand{\bsfJb} {\bar{\bsfJ}}
\newcommand{\bsfKb} {\bar{\bsfK}}
\newcommand{\bsfLb} {\bar{\bsfL}}
\newcommand{\bsfMb} {\bar{\bsfM}}
\newcommand{\bsfNb} {\bar{\bsfN}}
\newcommand{\bsfOb} {\bar{\bsfO}}
\newcommand{\bsfPb} {\bar{\bsfP}}
\newcommand{\bsfQb} {\bar{\bsfQ}}
\newcommand{\bsfRb} {\bar{\bsfR}}
\newcommand{\bsfSb} {\bar{\bsfS}}
\newcommand{\bsfTb} {\bar{\bsfT}}
\newcommand{\bsfUb} {\bar{\bsfU}}
\newcommand{\bsfVb} {\bar{\bsfV}}
\newcommand{\bsfWb} {\bar{\bsfW}}
\newcommand{\bsfXb} {\bar{\bsfX}}
\newcommand{\bsfYb} {\bar{\bsfY}}
\newcommand{\bsfZb} {\bar{\bsfZ}}

\newcommand{\bsfAB} {\overline{\bsfA}}
\newcommand{\bsfBB} {\overline{\bsfB}}
\newcommand{\bsfCB} {\overline{\bsfC}}
\newcommand{\bsfDB} {\overline{\bsfD}}
\newcommand{\bsfEB} {\overline{\bsfE}}
\newcommand{\bsfFB} {\overline{\bsfF}}
\newcommand{\bsfGB} {\overline{\bsfG}}
\newcommand{\bsfHB} {\overline{\bsfH}}
\newcommand{\bsfIB} {\overline{\bsfI}}
\newcommand{\bsfJB} {\overline{\bsfJ}}
\newcommand{\bsfKB} {\overline{\bsfK}}
\newcommand{\bsfLB} {\overline{\bsfL}}
\newcommand{\bsfMB} {\overline{\bsfM}}
\newcommand{\bsfNB} {\overline{\bsfN}}
\newcommand{\bsfOB} {\overline{\bsfO}}
\newcommand{\bsfPB} {\overline{\bsfP}}
\newcommand{\bsfQB} {\overline{\bsfQ}}
\newcommand{\bsfRB} {\overline{\bsfR}}
\newcommand{\bsfSB} {\overline{\bsfS}}
\newcommand{\bsfTB} {\overline{\bsfT}}
\newcommand{\bsfUB} {\overline{\bsfU}}
\newcommand{\bsfVB} {\overline{\bsfV}}
\newcommand{\bsfWB} {\overline{\bsfW}}
\newcommand{\bsfXB} {\overline{\bsfX}}
\newcommand{\bsfYB} {\overline{\bsfY}}
\newcommand{\bsfZB} {\overline{\bsfZ}}
%  -------------------------------
%  Hat letters, sansserif boldface
%  -------------------------------

\newcommand{\bsfat} {\tilde{\bsfa}}
\newcommand{\bsfbt} {\tilde{\bsfb}}
\newcommand{\bsfct} {\tilde{\bsfc}}
\newcommand{\bsfdt} {\tilde{\bsfd}}
\newcommand{\bsfet} {\tilde{\bsfe}}
\newcommand{\bsfft} {\tilde{\bsff}}
\newcommand{\bsfgt} {\tilde{\bsfg}}
\newcommand{\bsfht} {\tilde{\bsfh}}
\newcommand{\bsfit} {\tilde{\bsfi}}
\newcommand{\bsfjt} {\tilde{\bsfj}}
\newcommand{\bsfkt} {\tilde{\bsfk}}
\newcommand{\bsflt} {\tilde{\bsfl}}
\newcommand{\bsfmt} {\tilde{\bsfm}}
\newcommand{\bsfnt} {\tilde{\bsfn}}
\newcommand{\bsfot} {\tilde{\bsfo}}
\newcommand{\bsfpt} {\tilde{\bsfp}}
\newcommand{\bsfqt} {\tilde{\bsfq}}
\newcommand{\bsfrt} {\tilde{\bsfr}}
\newcommand{\bsfst} {\tilde{\bsfs}}
\newcommand{\bsftt} {\tilde{\bsft}}
\newcommand{\bsfut} {\tilde{\bsfu}}
\newcommand{\bsfvt} {\tilde{\bsfv}}
\newcommand{\bsfwt} {\tilde{\bsfw}}
\newcommand{\bsfxt} {\tilde{\bsfx}}
\newcommand{\bsfyt} {\tilde{\bsfy}}
\newcommand{\bsfzt} {\tilde{\bsfz}}

\newcommand{\bsfaT} {\widetilde{\bsfa}}
\newcommand{\bsfbT} {\widetilde{\bsfb}}
\newcommand{\bsfcT} {\widetilde{\bsfc}}
\newcommand{\bsfdT} {\widetilde{\bsfd}}
\newcommand{\bsfeT} {\widetilde{\bsfe}}
\newcommand{\bsffT} {\widetilde{\bsff}}
\newcommand{\bsfgT} {\widetilde{\bsfg}}
\newcommand{\bsfhT} {\widetilde{\bsfh}}
\newcommand{\bsfiT} {\widetilde{\bsfi}}
\newcommand{\bsfjT} {\widetilde{\bsfj}}
\newcommand{\bsfkT} {\widetilde{\bsfk}}
\newcommand{\bsflT} {\widetilde{\bsfl}}
\newcommand{\bsfmT} {\widetilde{\bsfm}}
\newcommand{\bsfnT} {\widetilde{\bsfn}}
\newcommand{\bsfoT} {\widetilde{\bsfo}}
\newcommand{\bsfpT} {\widetilde{\bsfp}}
\newcommand{\bsfqT} {\widetilde{\bsfq}}
\newcommand{\bsfrT} {\widetilde{\bsfr}}
\newcommand{\bsfsT} {\widetilde{\bsfs}}
\newcommand{\bsftT} {\widetilde{\bsft}}
\newcommand{\bsfuT} {\widetilde{\bsfu}}
\newcommand{\bsfvT} {\widetilde{\bsfv}}
\newcommand{\bsfwT} {\widetilde{\bsfw}}
\newcommand{\bsfxT} {\widetilde{\bsfx}}
\newcommand{\bsfyT} {\widetilde{\bsfy}}
\newcommand{\bsfzT} {\widetilde{\bsfz}}

\newcommand{\bsfAt} {\tilde{\bsfA}}
\newcommand{\bsfBt} {\tilde{\bsfB}}
\newcommand{\bsfCt} {\tilde{\bsfC}}
\newcommand{\bsfDt} {\tilde{\bsfD}}
\newcommand{\bsfEt} {\tilde{\bsfE}}
\newcommand{\bsfFt} {\tilde{\bsfF}}
\newcommand{\bsfGt} {\tilde{\bsfG}}
\newcommand{\bsfHt} {\tilde{\bsfH}}
\newcommand{\bsfIt} {\tilde{\bsfI}}
\newcommand{\bsfJt} {\tilde{\bsfJ}}
\newcommand{\bsfKt} {\tilde{\bsfK}}
\newcommand{\bsfLt} {\tilde{\bsfL}}
\newcommand{\bsfMt} {\tilde{\bsfM}}
\newcommand{\bsfNt} {\tilde{\bsfN}}
\newcommand{\bsfOt} {\tilde{\bsfO}}
\newcommand{\bsfPt} {\tilde{\bsfP}}
\newcommand{\bsfQt} {\tilde{\bsfQ}}
\newcommand{\bsfRt} {\tilde{\bsfR}}
\newcommand{\bsfSt} {\tilde{\bsfS}}
\newcommand{\bsfTt} {\tilde{\bsfT}}
\newcommand{\bsfUt} {\tilde{\bsfU}}
\newcommand{\bsfVt} {\tilde{\bsfV}}
\newcommand{\bsfWt} {\tilde{\bsfW}}
\newcommand{\bsfXt} {\tilde{\bsfX}}
\newcommand{\bsfYt} {\tilde{\bsfY}}
\newcommand{\bsfZt} {\tilde{\bsfZ}}

\newcommand{\bsfAT} {\widetilde{\bsfA}}
\newcommand{\bsfBT} {\widetilde{\bsfB}}
\newcommand{\bsfCT} {\widetilde{\bsfC}}
\newcommand{\bsfDT} {\widetilde{\bsfD}}
\newcommand{\bsfET} {\widetilde{\bsfE}}
\newcommand{\bsfFT} {\widetilde{\bsfF}}
\newcommand{\bsfGT} {\widetilde{\bsfG}}
\newcommand{\bsfHT} {\widetilde{\bsfH}}
\newcommand{\bsfIT} {\widetilde{\bsfI}}
\newcommand{\bsfJT} {\widetilde{\bsfJ}}
\newcommand{\bsfKT} {\widetilde{\bsfK}}
\newcommand{\bsfLT} {\widetilde{\bsfL}}
\newcommand{\bsfMT} {\widetilde{\bsfM}}
\newcommand{\bsfNT} {\widetilde{\bsfN}}
\newcommand{\bsfOT} {\widetilde{\bsfO}}
\newcommand{\bsfPT} {\widetilde{\bsfP}}
\newcommand{\bsfQT} {\widetilde{\bsfQ}}
\newcommand{\bsfRT} {\widetilde{\bsfR}}
\newcommand{\bsfST} {\widetilde{\bsfS}}
\newcommand{\bsfTT} {\widetilde{\bsfT}}
\newcommand{\bsfUT} {\widetilde{\bsfU}}
\newcommand{\bsfVT} {\widetilde{\bsfV}}
\newcommand{\bsfWT} {\widetilde{\bsfW}}
\newcommand{\bsfXT} {\widetilde{\bsfX}}
\newcommand{\bsfYT} {\widetilde{\bsfY}}
\newcommand{\bsfZT} {\widetilde{\bsfZ}}
%  ------------------
%  Hat letters, other
%  ------------------

\newcommand{\ahat}{\hat{a}}
\newcommand{\bhat}{\hat{b}}
\newcommand{\chat}{\hat{c}}
\newcommand{\dhat}{\hat{d}}
\newcommand{\ehat}{\hat{e}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\ghat}{\hat{g}}
\newcommand{\hhat}{\hat{h}}
\newcommand{\ihat}{\hat{\imath}}
\newcommand{\jhat}{\hat{\jmath}}
\newcommand{\khat}{\hat{k}}
\newcommand{\lhat}{\hat{l}}
\newcommand{\mhat}{\hat{m}}
\newcommand{\nhat}{\hat{n}}
\newcommand{\ohat}{\hat{o}}
\newcommand{\phat}{\hat{p}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\rhat}{\hat{r}}
\newcommand{\shat}{\hat{s}}
\newcommand{\that}{\hat{t}}
\newcommand{\uhat}{\hat{u}}
\newcommand{\vhat}{\hat{v}}
\newcommand{\what}{\hat{w}}
\newcommand{\xhat}{\hat{x}}
\newcommand{\yhat}{\hat{y}}
\newcommand{\zhat}{\hat{z}}

\newcommand{\Ahat}{\hat{A}}
\newcommand{\Bhat}{\hat{B}}
\newcommand{\Chat}{\hat{C}}
\newcommand{\Dhat}{\hat{D}}
\newcommand{\Ehat}{\hat{E}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\Ghat}{\hat{G}}
\newcommand{\Hhat}{\hat{H}}
\newcommand{\Ihat}{\hat{I}}
\newcommand{\Jhat}{\hat{J}}
\newcommand{\Khat}{\hat{K}}
\newcommand{\Lhat}{\hat{L}}
\newcommand{\Mhat}{\hat{M}}
\newcommand{\Nhat}{\hat{N}}
\newcommand{\Ohat}{\hat{O}}
\newcommand{\Phat}{\hat{P}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\Rhat}{\hat{R}}
\newcommand{\Shat}{\hat{S}}
\newcommand{\That}{\hat{T}}
\newcommand{\Uhat}{\hat{U}}
\newcommand{\Vhat}{\hat{V}}
\newcommand{\What}{\hat{W}}
\newcommand{\Xhat}{\hat{X}}
\newcommand{\Yhat}{\hat{Y}}
\newcommand{\Zhat}{\hat{Z}}

\newcommand{\aHat}{\widehat{a}}
\newcommand{\bHat}{\widehat{b}}
\newcommand{\cHat}{\widehat{c}}
\newcommand{\dHat}{\widehat{d}}
\newcommand{\eHat}{\widehat{e}}
\newcommand{\fHat}{\widehat{f}}
\newcommand{\gHat}{\widehat{g}}
\newcommand{\hHat}{\widehat{h}}
\newcommand{\iHat}{\widehat{i}}
\newcommand{\jHat}{\widehat{j}}
\newcommand{\kHat}{\widehat{k}}
\newcommand{\lHat}{\widehat{l}}
\newcommand{\mHat}{\widehat{m}}
\newcommand{\nHat}{\widehat{n}}
\newcommand{\oHat}{\widehat{o}}
\newcommand{\pHat}{\widehat{p}}
\newcommand{\qHat}{\widehat{q}}
\newcommand{\rHat}{\widehat{r}}
\newcommand{\sHat}{\widehat{s}}
\newcommand{\tHat}{\widehat{t}}
\newcommand{\uHat}{\widehat{u}}
\newcommand{\vHat}{\widehat{v}}
\newcommand{\wHat}{\widehat{w}}
\newcommand{\xHat}{\widehat{x}}
\newcommand{\yHat}{\widehat{y}}
\newcommand{\zHat}{\widehat{z}}

\newcommand{\AHat}{\widehat{A}}
\newcommand{\BHat}{\widehat{B}}
\newcommand{\CHat}{\widehat{C}}
\newcommand{\DHat}{\widehat{D}}
\newcommand{\EHat}{\widehat{E}}
\newcommand{\FHat}{\widehat{F}}
\newcommand{\GHat}{\widehat{G}}
\newcommand{\HHat}{\widehat{H}}
\newcommand{\IHat}{\widehat{I}}
\newcommand{\JHat}{\widehat{J}}
\newcommand{\KHat}{\widehat{K}}
\newcommand{\LHat}{\widehat{L}}
\newcommand{\MHat}{\widehat{M}}
\newcommand{\NHat}{\widehat{N}}
\newcommand{\OHat}{\widehat{O}}
\newcommand{\PHat}{\widehat{P}}
\newcommand{\QHat}{\widehat{Q}}
\newcommand{\RHat}{\widehat{R}}
\newcommand{\SHat}{\widehat{S}}
\newcommand{\THat}{\widehat{T}}
\newcommand{\UHat}{\widehat{U}}
\newcommand{\VHat}{\widehat{V}}
\newcommand{\WHat}{\widehat{W}}
\newcommand{\XHat}{\widehat{X}}
\newcommand{\YHat}{\widehat{Y}}
\newcommand{\ZHat}{\widehat{Z}}
%  ------------------------------------------------------
%  Bar boldmath letters (short bar and wide bar versions)
%  ------------------------------------------------------

\newcommand{\bfab} {\bar{\boldsymbol{a}}{}}
\newcommand{\bfbb} {\bar{\boldsymbol{b}}{}}
\newcommand{\bfcb} {\bar{\boldsymbol{c}}{}}
\newcommand{\bfdb} {\bar{\boldsymbol{d}}{}}
\newcommand{\bfeb} {\bar{\boldsymbol{e}}{}}
\newcommand{\bffb} {\bar{\boldsymbol{f}}{}}
\newcommand{\bfgb} {\bar{\boldsymbol{g}}{}}
\newcommand{\bfhb} {\bar{\boldsymbol{b}}{}}
\newcommand{\bfjb} {\bar{\boldsymbol{j}}{}}
\newcommand{\bfkb} {\bar{\boldsymbol{k}}{}}
\newcommand{\bflb} {\bar{\boldsymbol{\ell}}{}}
\newcommand{\bfmb} {\bar{\boldsymbol{m}}{}}
\newcommand{\bfnb} {\bar{\boldsymbol{n}}{}}
\newcommand{\bfob} {\bar{\boldsymbol{o}}{}}
\newcommand{\bfpb} {\bar{\boldsymbol{p}}{}}
\newcommand{\bfqb} {\bar{\boldsymbol{q}}{}}
\newcommand{\bfrb} {\bar{\boldsymbol{r}}{}}
\newcommand{\bfsb} {\bar{\boldsymbol{s}}{}}
\newcommand{\bftb} {\bar{\boldsymbol{t}}{}}
\newcommand{\bfub} {\bar{\boldsymbol{u}}{}}
\newcommand{\bfvb} {\bar{\boldsymbol{v}}{}}
\newcommand{\bfwb} {\bar{\boldsymbol{w}}{}}
\newcommand{\bfxb} {\bar{\boldsymbol{x}}{}}
\newcommand{\bfyb} {\bar{\boldsymbol{y}}{}}
\newcommand{\bfzb} {\bar{\boldsymbol{z}}{}}

\newcommand{\bfAb} {\bar{\boldsymbol{A}}{}}
\newcommand{\bfBb} {\bar{\boldsymbol{B}}{}}
\newcommand{\bfCb} {\bar{\boldsymbol{C}}{}}
\newcommand{\bfDb} {\bar{\boldsymbol{D}}{}}
\newcommand{\bfEb} {\bar{\boldsymbol{E}}{}}
\newcommand{\bfFb} {\bar{\boldsymbol{F}}{}}
\newcommand{\bfGb} {\bar{\boldsymbol{G}}{}}
\newcommand{\bfHb} {\bar{\boldsymbol{B}}{}}
\newcommand{\bfIb} {\bar{\boldsymbol{I}}{}}
\newcommand{\bfJb} {\bar{\boldsymbol{J}}{}}
\newcommand{\bfKb} {\bar{\boldsymbol{K}}{}}
\newcommand{\bfLb} {\bar{\boldsymbol{L}}{}}
\newcommand{\bfMb} {\bar{\boldsymbol{M}}{}}
\newcommand{\bfNb} {\bar{\boldsymbol{N}}{}}
\newcommand{\bfOb} {\bar{\boldsymbol{O}}{}}
\newcommand{\bfPb} {\bar{\boldsymbol{P}}{}}
\newcommand{\bfQb} {\bar{\boldsymbol{Q}}{}}
\newcommand{\bfRb} {\bar{\boldsymbol{R}}{}}
\newcommand{\bfSb} {\bar{\boldsymbol{S}}{}}
\newcommand{\bfTb} {\bar{\boldsymbol{T}}{}}
\newcommand{\bfUb} {\bar{\boldsymbol{U}}{}}
\newcommand{\bfVb} {\bar{\boldsymbol{V}}{}}
\newcommand{\bfWb} {\bar{\boldsymbol{W}}{}}
\newcommand{\bfXb} {\bar{\boldsymbol{X}}{}}
\newcommand{\bfYb} {\bar{\boldsymbol{Y}}{}}
\newcommand{\bfZb} {\bar{\boldsymbol{Z}}{}}

\newcommand{\bfAB} {\overline{\boldsymbol{A}}{}}
\newcommand{\bfBB} {\overline{\boldsymbol{B}}{}}
\newcommand{\bfCB} {\overline{\boldsymbol{C}}{}}
\newcommand{\bfDB} {\overline{\boldsymbol{D}}{}}
\newcommand{\bfEB} {\overline{\boldsymbol{E}}{}}
\newcommand{\bfFB} {\overline{\boldsymbol{F}}{}}
\newcommand{\bfGB} {\overline{\boldsymbol{G}}{}}
\newcommand{\bfHB} {\overline{\boldsymbol{H}}{}}
\newcommand{\bfIB} {\overline{\boldsymbol{I}}{}}
\newcommand{\bfJB} {\overline{\boldsymbol{J}}{}}
\newcommand{\bfKB} {\overline{\boldsymbol{K}}{}}
\newcommand{\bfLB} {\overline{\boldsymbol{L}}{}}
\newcommand{\bfMB} {\overline{\boldsymbol{M}}{}}
\newcommand{\bfNB} {\overline{\boldsymbol{N}}{}}
\newcommand{\bfOB} {\overline{\boldsymbol{O}}{}}
\newcommand{\bfPB} {\overline{\boldsymbol{P}}{}}
\newcommand{\bfQB} {\overline{\boldsymbol{Q}}{}}
\newcommand{\bfRB} {\overline{\boldsymbol{R}}{}}
\newcommand{\bfSB} {\overline{\boldsymbol{S}}{}}
\newcommand{\bfTB} {\overline{\boldsymbol{T}}{}}
\newcommand{\bfUB} {\overline{\boldsymbol{U}}{}}
\newcommand{\bfVB} {\overline{\boldsymbol{V}}{}}
\newcommand{\bfWB} {\overline{\boldsymbol{W}}{}}
\newcommand{\bfXB} {\overline{\boldsymbol{X}}{}}
\newcommand{\bfYB} {\overline{\boldsymbol{Y}}{}}
\newcommand{\bfZB} {\overline{\boldsymbol{Z}}{}}

\newcommand{\bfaB} {\overline{\boldsymbol{a}}{}}
\newcommand{\bfbB} {\overline{\boldsymbol{b}}{}}
\newcommand{\bfcB} {\overline{\boldsymbol{c}}{}}
\newcommand{\bfdB} {\overline{\boldsymbol{d}}{}}
\newcommand{\bfeB} {\overline{\boldsymbol{e}}{}}
\newcommand{\bffB} {\overline{\boldsymbol{f}}{}}
\newcommand{\bfgB} {\overline{\boldsymbol{g}}{}}
\newcommand{\bfhB} {\overline{\boldsymbol{h}}{}}
\newcommand{\bfiB} {\overline{\boldsymbol{i}}{}}
\newcommand{\bfjB} {\overline{\boldsymbol{j}}{}}
\newcommand{\bfkB} {\overline{\boldsymbol{k}}{}}
\newcommand{\bflB} {\overline{\boldsymbol{l}}{}}
\newcommand{\bfmB} {\overline{\boldsymbol{m}}{}}
\newcommand{\bfnB} {\overline{\boldsymbol{n}}{}}
\newcommand{\bfoB} {\overline{\boldsymbol{o}}{}}
\newcommand{\bfpB} {\overline{\boldsymbol{p}}{}}
\newcommand{\bfqB} {\overline{\boldsymbol{q}}{}}
\newcommand{\bfrB} {\overline{\boldsymbol{r}}{}}
\newcommand{\bfsB} {\overline{\boldsymbol{s}}{}}
\newcommand{\bftB} {\overline{\boldsymbol{t}}{}}
\newcommand{\bfuB} {\overline{\boldsymbol{u}}{}}
\newcommand{\bfvB} {\overline{\boldsymbol{v}}{}}
\newcommand{\bfwB} {\overline{\boldsymbol{w}}{}}
\newcommand{\bfxB} {\overline{\boldsymbol{x}}{}}
\newcommand{\bfyB} {\overline{\boldsymbol{y}}{}}
\newcommand{\bfzB} {\overline{\boldsymbol{z}}{}}
%  ------------------------------------------------------
%  Bar boldface letters (short bar and wide bar versions)
%  ------------------------------------------------------

\newcommand{\brab} {\bar{\mathbf{a}}{}}
\newcommand{\brbb} {\bar{\mathbf{b}}{}}
\newcommand{\brcb} {\bar{\mathbf{c}}{}}
\newcommand{\brdb} {\bar{\mathbf{d}}{}}
\newcommand{\breb} {\bar{\mathbf{e}}{}}
\newcommand{\brfb} {\bar{\mathbf{f}}{}}
\newcommand{\brgb} {\bar{\mathbf{g}}{}}
\newcommand{\brhb} {\bar{\mathbf{h}}{}}
\newcommand{\brib} {\bar{\mathbf{i}}{}}
\newcommand{\brjb} {\bar{\mathbf{j}}{}}
\newcommand{\brkb} {\bar{\mathbf{k}}{}}
\newcommand{\brlb} {\bar{\mathbf{l}}{}}
\newcommand{\brmb} {\bar{\mathbf{m}}{}}
\newcommand{\brnb} {\bar{\mathbf{n}}{}}
\newcommand{\brob} {\bar{\mathbf{o}}{}}
\newcommand{\brpb} {\bar{\mathbf{p}}{}}
\newcommand{\brqb} {\bar{\mathbf{q}}{}}
\newcommand{\brrb} {\bar{\mathbf{r}}{}}
\newcommand{\brsb} {\bar{\mathbf{s}}{}}
\newcommand{\brtb} {\bar{\mathbf{t}}{}}
\newcommand{\brub} {\bar{\mathbf{u}}{}}
\newcommand{\brvb} {\bar{\mathbf{v}}{}}
\newcommand{\brwb} {\bar{\mathbf{w}}{}}
\newcommand{\brxb} {\bar{\mathbf{x}}{}}
\newcommand{\bryb} {\bar{\mathbf{y}}{}}
\newcommand{\brzb} {\bar{\mathbf{z}}{}}

\newcommand{\brAb} {\bar{\mathbf{A}}{}}
\newcommand{\brBb} {\bar{\mathbf{B}}{}}
\newcommand{\brCb} {\bar{\mathbf{C}}{}}
\newcommand{\brDb} {\bar{\mathbf{D}}{}}
\newcommand{\brEb} {\bar{\mathbf{E}}{}}
\newcommand{\brFb} {\bar{\mathbf{F}}{}}
\newcommand{\brGb} {\bar{\mathbf{G}}{}}
\newcommand{\brHb} {\bar{\mathbf{H}}{}}
\newcommand{\brIb} {\bar{\mathbf{I}}{}}
\newcommand{\brJb} {\bar{\mathbf{J}}{}}
\newcommand{\brKb} {\bar{\mathbf{K}}{}}
\newcommand{\brLb} {\bar{\mathbf{L}}{}}
\newcommand{\brMb} {\bar{\mathbf{M}}{}}
\newcommand{\brNb} {\bar{\mathbf{N}}{}}
\newcommand{\brOb} {\bar{\mathbf{O}}{}}
\newcommand{\brPb} {\bar{\mathbf{P}}{}}
\newcommand{\brQb} {\bar{\mathbf{Q}}{}}
\newcommand{\brRb} {\bar{\mathbf{R}}{}}
\newcommand{\brSb} {\bar{\mathbf{S}}{}}
\newcommand{\brTb} {\bar{\mathbf{T}}{}}
\newcommand{\brUb} {\bar{\mathbf{U}}{}}
\newcommand{\brVb} {\bar{\mathbf{V}}{}}
\newcommand{\brWb} {\bar{\mathbf{W}}{}}
\newcommand{\brXb} {\bar{\mathbf{X}}{}}
\newcommand{\brYb} {\bar{\mathbf{Y}}{}}
\newcommand{\brZb} {\bar{\mathbf{Z}}{}}

\newcommand{\braB} {\overline{\mathbf{a}}{}}
\newcommand{\brbB} {\overline{\mathbf{b}}{}}
\newcommand{\brcB} {\overline{\mathbf{c}}{}}
\newcommand{\brdB} {\overline{\mathbf{d}}{}}
\newcommand{\breB} {\overline{\mathbf{e}}{}}
\newcommand{\brfB} {\overline{\mathbf{f}}{}}
\newcommand{\brgB} {\overline{\mathbf{g}}{}}
\newcommand{\brhB} {\overline{\mathbf{h}}{}}
\newcommand{\briB} {\overline{\mathbf{i}}{}}
\newcommand{\brjB} {\overline{\mathbf{j}}{}}
\newcommand{\brkB} {\overline{\mathbf{k}}{}}
\newcommand{\brlB} {\overline{\mathbf{l}}{}}
\newcommand{\brmB} {\overline{\mathbf{m}}{}}
\newcommand{\brnB} {\overline{\mathbf{n}}{}}
\newcommand{\broB} {\overline{\mathbf{o}}{}}
\newcommand{\brpB} {\overline{\mathbf{p}}{}}
\newcommand{\brqB} {\overline{\mathbf{q}}{}}
\newcommand{\brrB} {\overline{\mathbf{r}}{}}
\newcommand{\brsB} {\overline{\mathbf{s}}{}}
\newcommand{\brtB} {\overline{\mathbf{t}}{}}
\newcommand{\bruB} {\overline{\mathbf{u}}{}}
\newcommand{\brvB} {\overline{\mathbf{v}}{}}
\newcommand{\brwB} {\overline{\mathbf{w}}{}}
\newcommand{\brxB} {\overline{\mathbf{x}}{}}
\newcommand{\bryB} {\overline{\mathbf{y}}{}}
\newcommand{\brzB} {\overline{\mathbf{z}}{}}

\newcommand{\brAB} {\overline{\mathbf{A}}{}}
\newcommand{\brBB} {\overline{\mathbf{B}}{}}
\newcommand{\brCB} {\overline{\mathbf{C}}{}}
\newcommand{\brDB} {\overline{\mathbf{D}}{}}
\newcommand{\brEB} {\overline{\mathbf{E}}{}}
\newcommand{\brFB} {\overline{\mathbf{F}}{}}
\newcommand{\brGB} {\overline{\mathbf{G}}{}}
\newcommand{\brHB} {\overline{\mathbf{H}}{}}
\newcommand{\brIB} {\overline{\mathbf{I}}{}}
\newcommand{\brJB} {\overline{\mathbf{J}}{}}
\newcommand{\brKB} {\overline{\mathbf{K}}{}}
\newcommand{\brLB} {\overline{\mathbf{L}}{}}
\newcommand{\brMB} {\overline{\mathbf{M}}{}}
\newcommand{\brNB} {\overline{\mathbf{N}}{}}
\newcommand{\brOB} {\overline{\mathbf{O}}{}}
\newcommand{\brPB} {\overline{\mathbf{P}}{}}
\newcommand{\brQB} {\overline{\mathbf{Q}}{}}
\newcommand{\brRB} {\overline{\mathbf{R}}{}}
\newcommand{\brSB} {\overline{\mathbf{S}}{}}
\newcommand{\brTB} {\overline{\mathbf{T}}{}}
\newcommand{\brUB} {\overline{\mathbf{U}}{}}
\newcommand{\brVB} {\overline{\mathbf{V}}{}}
\newcommand{\brWB} {\overline{\mathbf{W}}{}}
\newcommand{\brXB} {\overline{\mathbf{X}}{}}
\newcommand{\brYB} {\overline{\mathbf{Y}}{}}
\newcommand{\brZB} {\overline{\mathbf{Z}}{}}
%  ---------------------------------------------
%  Bar letters (short bar and wide bar versions)
%  ---------------------------------------------

\newcommand{\Abar}{\bar{A}{}}
\newcommand{\Bbar}{\bar{B}{}}
\newcommand{\Cbar}{\bar{C}{}}
\newcommand{\Dbar}{\bar{D}{}}
\newcommand{\Ebar}{\bar{E}{}}
\newcommand{\Fbar}{\bar{F}{}}
\newcommand{\Gbar}{\bar{G}{}}
\newcommand{\Hbar}{\bar{H}{}}
\newcommand{\Ibar}{\bar{I}{}}
\newcommand{\Jbar}{\bar{J}{}}
\newcommand{\Kbar}{\bar{K}{}}
\newcommand{\Lbar}{\Lbar{}{}}
\newcommand{\Mbar}{\bar{M}{}}
\newcommand{\Nbar}{\Nbar{}{}}
\newcommand{\Obar}{\Obar{}{}}
\newcommand{\Pbar}{\bar{P}{}}
\newcommand{\Qbar}{\bar{Q}{}}
\newcommand{\Rbar}{\Rbar{}{}}
\newcommand{\Sbar}{\bar{S}{}}
\newcommand{\Tbar}{\Tbar{}{}}
\newcommand{\Ubar}{\bar{U}{}}
\newcommand{\Vbar}{\bar{V}{}}
\newcommand{\Wbar}{\bar{W}{}}
\newcommand{\Xbar}{\bar{X}{}}
\newcommand{\Ybar}{\bar{Y}{}}
\newcommand{\Zbar}{\bar{Z}{}}

\newcommand{\abar}{\bar{a}{}}
\newcommand{\bbar}{\bar{b}{}}
\newcommand{\cbar}{\bar{c}{}}
\newcommand{\dbar}{\bar{d}{}}
\newcommand{\ebar}{\bar{e}{}}
\newcommand{\fbar}{\bar{f}{}}
\newcommand{\gbar}{\bar{g}{}}
\Newcommand{\hbar}{\bar{h}{}}
\newcommand{\ibar}{\bar{\imath}{}}
\newcommand{\jbar}{\bar{\jmath}{}}
\newcommand{\kbar}{\bar{k}{}}
\newcommand{\lbar}{\bar{\ell}{}}
\newcommand{\mbar}{\bar{m}{}}
\newcommand{\nbar}{\bar{n}{}}
\newcommand{\obar}{\bar{o}{}}
\newcommand{\pbar}{\bar{p}{}}
\newcommand{\qbar}{\bar{q}{}}
\newcommand{\rbar}{\bar{r}{}}
\newcommand{\sbar}{\bar{s}{}}
\newcommand{\tbar}{\bar{t}{}}
\newcommand{\ubar}{\bar{u}{}}
\newcommand{\vbar}{\bar{v}{}}
\newcommand{\wbar}{\bar{w}{}}
\newcommand{\xbar}{\bar{x}{}}
\newcommand{\ybar}{\bar{y}{}}
\newcommand{\zbar}{\bar{z}{}}

\newcommand{\ABar}{\overline{A}{}}
\newcommand{\BBar}{\overline{B}{}}
\newcommand{\CBar}{\overline{C}{}}
\newcommand{\DBar}{\overline{D}{}}
\newcommand{\EBar}{\overline{E}{}}
\newcommand{\FBar}{\overline{F}{}}
\newcommand{\GBar}{\overline{G}{}}
\newcommand{\HBar}{\overline{H}{}}
\newcommand{\IBar}{\overline{I}{}}
\newcommand{\JBar}{\overline{J}{}}
\newcommand{\KBar}{\overline{K}{}}
\newcommand{\LBar}{\overline{L}{}}
\newcommand{\MBar}{\overline{M}{}}
\newcommand{\NBar}{\overline{N}{}}
\newcommand{\OBar}{\overline{O}{}}
\newcommand{\PBar}{\overline{P}{}}
\newcommand{\QBar}{\overline{Q}{}}
\newcommand{\RBar}{\overline{R}{}}
\newcommand{\SBar}{\overline{S}{}}
\newcommand{\TBar}{\overline{T}{}}
\newcommand{\UBar}{\overline{U}{}}
\newcommand{\VBar}{\overline{V}{}}
\newcommand{\WBar}{\overline{W}{}}
\newcommand{\XBar}{\overline{X}{}}
\newcommand{\YBar}{\overline{Y}{}}
\newcommand{\ZBar}{\overline{Z}{}}

\newcommand{\aBar}{\overline{a}{}}
\newcommand{\bBar}{\overline{b}{}}
\newcommand{\cBar}{\overline{c}{}}
\newcommand{\dBar}{\overline{d}{}}
\newcommand{\eBar}{\overline{e}{}}
\newcommand{\fBar}{\overline{f}{}}
\newcommand{\gBar}{\overline{g}{}}
\newcommand{\hBar}{\overline{h}{}}
\newcommand{\iBar}{\overline{\imath}{}}
\newcommand{\jBar}{\overline{\jmath}{}}
\newcommand{\kBar}{\overline{k}{}}
\newcommand{\lBar}{\overline{\ell}{}}
\newcommand{\mBar}{\overline{m}{}}
\newcommand{\nBar}{\overline{n}{}}
\newcommand{\oBar}{\overline{o}{}}
\newcommand{\pBar}{\overline{p}{}}
\newcommand{\qBar}{\overline{q}{}}
\newcommand{\rBar}{\overline{r}{}}
\newcommand{\sBar}{\overline{s}{}}
\newcommand{\tBar}{\overline{t}{}}
\newcommand{\uBar}{\overline{u}{}}
\newcommand{\vBar}{\overline{v}{}}
\newcommand{\wBar}{\overline{w}{}}
\newcommand{\xBar}{\overline{x}{}}
\newcommand{\yBar}{\overline{y}{}}
\newcommand{\zBar}{\overline{z}{}}
%  -------------------------------------------
%  Blackboard-bold symbols (uppercase letters)
%  -------------------------------------------

\newcommand{\Abb} {\mathbb{A}}
\Newcommand{\Bbb} {\mathbb{B}}
\newcommand{\Cbb} {\mathbb{C}}
\newcommand{\Dbb} {\mathbb{D}}
\newcommand{\Ebb} {\mathbb{E}}
\newcommand{\Fbb} {\mathbb{F}}
\newcommand{\Gbb} {\mathbb{G}}
\newcommand{\Hbb} {\mathbb{H}}
\newcommand{\Ibb} {\mathbb{I}}
\newcommand{\Jbb} {\mathbb{J}}
\newcommand{\Kbb} {\mathbb{K}}
\newcommand{\Lbb} {\mathbb{L}}
\newcommand{\Mbb} {\mathbb{M}}
\newcommand{\Nbb} {\mathbb{N}}
\newcommand{\Obb} {\mathbb{O}}
\newcommand{\Pbb} {\mathbb{P}}
\newcommand{\Qbb} {\mathbb{Q}}
\newcommand{\Rbb} {\mathbb{R}}
\newcommand{\Sbb} {\mathbb{S}}
\newcommand{\Tbb} {\mathbb{T}}
\newcommand{\Ubb} {\mathbb{U}}
\newcommand{\Vbb} {\mathbb{V}}
\newcommand{\Wbb} {\mathbb{W}}
\newcommand{\Xbb} {\mathbb{X}}
\newcommand{\Ybb} {\mathbb{Y}}
\newcommand{\Zbb} {\mathbb{Z}}
%  ---------------------------
%  Boldface Greek letters, bar
%  ---------------------------

\newcommand{\bfDelb}{\bar{\bfDel}}
\newcommand{\bfGab}{\bar{\bfGa}}
\newcommand{\bfLab}{\bar{\bfLa}}
\newcommand{\bfmPib}{\bar{\bfmPi}}
\newcommand{\bfOmb}{\bar{\bfOm}}
\newcommand{\bfPhb}{\bar{\bfPh}}
\newcommand{\bfPib}{\bar{\bfPi}}
\newcommand{\bfPsb}{\bar{\bfPs}}
\newcommand{\bfSigb}{\bar{\bfSig}}
\newcommand{\bfThb}{\bar{\bfTh}}
\newcommand{\bfXib}{\bar{\bfXi}}

\newcommand{\bfpib}{\bar{\bfpi}}
\newcommand{\bfvpib}{\bar{\bfvpi}}
\newcommand{\bfalb}{\bar{\bfal}}
\newcommand{\bfbeb}{\bar{\bfbe}}
\newcommand{\bfchib}{\bar{\bfchi}}
\newcommand{\bfdelb}{\bar{\bfdel}}
\newcommand{\bfepsvb}{\bar{\bfepsv}}
\newcommand{\bfepsb}{\bar{\bfeps}}
\newcommand{\bfetab}{\bar{\bfeta}}
\newcommand{\bfgab}{\bar{\bfga}}
\newcommand{\bflab}{\bar{\bfla}}
\newcommand{\bfkab}{\bar{\bfka}}
\newcommand{\bfiob}{\bar{\bfio}}
\newcommand{\bfmpib}{\bar{\bfmpi}}
\newcommand{\bfmub}{\bar{\bfmu}}
\newcommand{\bfnub}{\bar{\bfnu}}
\newcommand{\bfupsb}{\bar{\bfups}}
\newcommand{\bfoob}{\bar{\bfoo}}
\newcommand{\bfphb}{\bar{\bfph}}
\newcommand{\bfphcb}{\bar{\bfphc}}
\newcommand{\bfpsb}{\bar{\bfps}}
\newcommand{\bfrhob}{\bar{\bfrho}}
\newcommand{\bfrhvb}{\bar{\bfrhv}}
\newcommand{\bfsigb}{\bar{\bfsig}}
\newcommand{\bftaub}{\bar{\bftau}}
\newcommand{\bfthb}{\bar{\bfth}}
\newcommand{\bfthvb}{\bar{\bfthv}}
\newcommand{\bfxib}{\bar{\bfxi}}
\newcommand{\bfzetb}{\bar{\bfzet}}
\newcommand{\btetab}{\bar{\bteta}}

\newcommand{\bfDelB}{\overline{\bfDel}}
\newcommand{\bfGaB}{\overline{\bfGa}}
\newcommand{\bfLaB}{\overline{\bfLa}}
\newcommand{\bfmPiB}{\overline{\bfmPi}}
\newcommand{\bfOmB}{\overline{\bfOm}}
\newcommand{\bfPhB}{\overline{\bfPh}}
\newcommand{\bfPiB}{\overline{\bfPi}}
\newcommand{\bfPsB}{\overline{\bfPs}}
\newcommand{\bfSigB}{\overline{\bfSig}}
\newcommand{\bfThB}{\overline{\bfTh}}
\newcommand{\bfXiB}{\overline{\bfXi}}

\newcommand{\bfpiB}{\overline{\bfpi}}
\newcommand{\bfvpiB}{\overline{\bfvpi}}
\newcommand{\bfalB}{\overline{\bfal}}
\newcommand{\bfbeB}{\overline{\bfbe}}
\newcommand{\bfchiB}{\overline{\bfchi}}
\newcommand{\bfdelB}{\overline{\bfdel}}
\newcommand{\bfepsvB}{\overline{\bfepsv}}
\newcommand{\bfepsB}{\overline{\bfeps}}
\newcommand{\bfetaB}{\overline{\bfeta}}
\newcommand{\bfgaB}{\overline{\bfga}}
\newcommand{\bflaB}{\overline{\bfla}}
\newcommand{\bfkaB}{\overline{\bfka}}
\newcommand{\bfioB}{\overline{\bfio}}
\newcommand{\bfmpiB}{\overline{\bfmpi}}
\newcommand{\bfmuB}{\overline{\bfmu}}
\newcommand{\bfnuB}{\overline{\bfnu}}
\newcommand{\bfupsB}{\overline{\bfups}}
\newcommand{\bfooB}{\overline{\bfoo}}
\newcommand{\bfphB}{\overline{\bfph}}
\newcommand{\bfphcB}{\overline{\bfphc}}
\newcommand{\bfpsB}{\overline{\bfps}}
\newcommand{\bfrhoB}{\overline{\bfrho}}
\newcommand{\bfrhvB}{\overline{\bfrhv}}
\newcommand{\bfsigB}{\overline{\bfsig}}
\newcommand{\bftauB}{\overline{\bftau}}
\newcommand{\bfthB}{\overline{\bfth}}
\newcommand{\bfthvB}{\overline{\bfthv}}
\newcommand{\bfxiB}{\overline{\bfxi}}
\newcommand{\bfzetB}{\overline{\bfzet}}
\newcommand{\btetaB}{\overline{\bteta}}
%  -----------------------------
%  Boldface Greek letters, tilde
%  -----------------------------

\newcommand{\bfDelt}{\tilde{\bfDel}}
\newcommand{\bfGat}{\tilde{\bfGa}}
\newcommand{\bfLat}{\tilde{\bfLa}}
\newcommand{\bfmPit}{\tilde{\bfmPi}}
\newcommand{\bfOmt}{\tilde{\bfOm}}
\newcommand{\bfPht}{\tilde{\bfPh}}
\newcommand{\bfPit}{\tilde{\bfPi}}
\newcommand{\bfPst}{\tilde{\bfPs}}
\newcommand{\bfSigt}{\tilde{\bfSig}}
\newcommand{\bfTht}{\tilde{\bfTh}}
\newcommand{\bfXit}{\tilde{\bfXi}}

\newcommand{\bfpit}{\tilde{\bfpi}}
\newcommand{\bfvpit}{\tilde{\bfvpi}}
\newcommand{\bfalt}{\tilde{\bfal}}
\newcommand{\bfbet}{\tilde{\bfbe}}
\newcommand{\bfchit}{\tilde{\bfchi}}
\newcommand{\bfdelt}{\tilde{\bfdel}}
\newcommand{\bfepsvt}{\tilde{\bfepsv}}
\newcommand{\bfepst}{\tilde{\bfeps}}
\newcommand{\bfetat}{\tilde{\bfeta}}
\newcommand{\bfgat}{\tilde{\bfga}}
\newcommand{\bflat}{\tilde{\bfla}}
\newcommand{\bfkat}{\tilde{\bfka}}
\newcommand{\bfiot}{\tilde{\bfio}}
\newcommand{\bfmpit}{\tilde{\bfmpi}}
\newcommand{\bfmut}{\tilde{\bfmu}}
\newcommand{\bfnut}{\tilde{\bfnu}}
\newcommand{\bfupst}{\tilde{\bfups}}
\newcommand{\bfoot}{\tilde{\bfoo}}
\newcommand{\bfpht}{\tilde{\bfph}}
\newcommand{\bfphct}{\tilde{\bfphc}}
\newcommand{\bfpst}{\tilde{\bfps}}
\newcommand{\bfrhot}{\tilde{\bfrho}}
\newcommand{\bfrhvt}{\tilde{\bfrhv}}
\newcommand{\bfsigt}{\tilde{\bfsig}}
\newcommand{\bftaut}{\tilde{\bftau}}
\newcommand{\bftht}{\tilde{\bfth}}
\newcommand{\bfthvt}{\tilde{\bfthv}}
\newcommand{\bfxit}{\tilde{\bfxi}}
\newcommand{\bfzett}{\tilde{\bfzet}}
\newcommand{\btetat}{\tilde{\bteta}}

\newcommand{\bfDelT}{\widetilde{\bfDel}}
\newcommand{\bfGaT}{\widetilde{\bfGa}}
\newcommand{\bfLaT}{\widetilde{\bfLa}}
\newcommand{\bfmPiT}{\widetilde{\bfmPi}}
\newcommand{\bfOmT}{\widetilde{\bfOm}}
\newcommand{\bfPhT}{\widetilde{\bfPh}}
\newcommand{\bfPiT}{\widetilde{\bfPi}}
\newcommand{\bfPsT}{\widetilde{\bfPs}}
\newcommand{\bfSigT}{\widetilde{\bfSig}}
\newcommand{\bfThT}{\widetilde{\bfTh}}
\newcommand{\bfXiT}{\widetilde{\bfXi}}

\newcommand{\bfpiT}{\widetilde{\bfpi}}
\newcommand{\bfvpiT}{\widetilde{\bfvpi}}
\newcommand{\bfalT}{\widetilde{\bfal}}
\newcommand{\bfbeT}{\widetilde{\bfbe}}
\newcommand{\bfchiT}{\widetilde{\bfchi}}
\newcommand{\bfdelT}{\widetilde{\bfdel}}
\newcommand{\bfepsvT}{\widetilde{\bfepsv}}
\newcommand{\bfepsT}{\widetilde{\bfeps}}
\newcommand{\bfetaT}{\widetilde{\bfeta}}
\newcommand{\bfgaT}{\widetilde{\bfga}}
\newcommand{\bflaT}{\widetilde{\bfla}}
\newcommand{\bfkaT}{\widetilde{\bfka}}
\newcommand{\bfioT}{\widetilde{\bfio}}
\newcommand{\bfmpiT}{\widetilde{\bfmpi}}
\newcommand{\bfmuT}{\widetilde{\bfmu}}
\newcommand{\bfnuT}{\widetilde{\bfnu}}
\newcommand{\bfupsT}{\widetilde{\bfups}}
\newcommand{\bfooT}{\widetilde{\bfoo}}
\newcommand{\bfphT}{\widetilde{\bfph}}
\newcommand{\bfphcT}{\widetilde{\bfphc}}
\newcommand{\bfpsT}{\widetilde{\bfps}}
\newcommand{\bfrhoT}{\widetilde{\bfrho}}
\newcommand{\bfrhvT}{\widetilde{\bfrhv}}
\newcommand{\bfsigT}{\widetilde{\bfsig}}
\newcommand{\bftauT}{\widetilde{\bftau}}
\newcommand{\bfthT}{\widetilde{\bfth}}
\newcommand{\bfthvT}{\widetilde{\bfthv}}
\newcommand{\bfxiT}{\widetilde{\bfxi}}
\newcommand{\bfzetT}{\widetilde{\bfzet}}
\newcommand{\btetaT}{\widetilde{\bteta}}

%  ---------------------------
%  Boldface Greek letters, hat
%  ---------------------------

\newcommand{\bfDelh}{\hat{\bfDel}}
\newcommand{\bfGah}{\hat{\bfGa}}
\newcommand{\bfLah}{\hat{\bfLa}}
\newcommand{\bfmPih}{\hat{\bfmPi}}
\newcommand{\bfOmh}{\hat{\bfOm}}
\newcommand{\bfPhh}{\hat{\bfPh}}
\newcommand{\bfPih}{\hat{\bfPi}}
\newcommand{\bfPsh}{\hat{\bfPs}}
\newcommand{\bfSigh}{\hat{\bfSig}}
\newcommand{\bfThh}{\hat{\bfTh}}
\newcommand{\bfXih}{\hat{\bfXi}}

\newcommand{\bfpih}{\hat{\bfpi}}
\newcommand{\bfvpih}{\hat{\bfvpi}}
\newcommand{\bfalh}{\hat{\bfal}}
\newcommand{\bfbeh}{\hat{\bfbe}}
\newcommand{\bfchih}{\hat{\bfchi}}
\newcommand{\bfdelh}{\hat{\bfdel}}
\newcommand{\bfepsvh}{\hat{\bfepsv}}
\newcommand{\bfepsh}{\hat{\bfeps}}
\newcommand{\bfetah}{\hat{\bfeta}}
\newcommand{\bfgah}{\hat{\bfga}}
\newcommand{\bflah}{\hat{\bfla}}
\newcommand{\bfkah}{\hat{\bfka}}
\newcommand{\bfioh}{\hat{\bfio}}
\newcommand{\bfmpih}{\hat{\bfmpi}}
\newcommand{\bfmuh}{\hat{\bfmu}}
\newcommand{\bfnuh}{\hat{\bfnu}}
\newcommand{\bfupsh}{\hat{\bfups}}
\newcommand{\bfooh}{\hat{\bfoo}}
\newcommand{\bfphh}{\hat{\bfph}}
\newcommand{\bfphch}{\hat{\bfphc}}
\newcommand{\bfpsh}{\hat{\bfps}}
\newcommand{\bfrhoh}{\hat{\bfrho}}
\newcommand{\bfrhvh}{\hat{\bfrhv}}
\newcommand{\bfsigh}{\hat{\bfsig}}
\newcommand{\bftauh}{\hat{\bftau}}
\newcommand{\bfthh}{\hat{\bfth}}
\newcommand{\bfthvh}{\hat{\bfthv}}
\newcommand{\bfxih}{\hat{\bfxi}}
\newcommand{\bfzeth}{\hat{\bfzet}}
\newcommand{\btetah}{\hat{\bteta}}

\newcommand{\bfDelH}{\widehat{\bfDel}}
\newcommand{\bfGaH}{\widehat{\bfGa}}
\newcommand{\bfLaH}{\widehat{\bfLa}}
\newcommand{\bfmPiH}{\widehat{\bfmPi}}
\newcommand{\bfOmH}{\widehat{\bfOm}}
\newcommand{\bfPhH}{\widehat{\bfPh}}
\newcommand{\bfPiH}{\widehat{\bfPi}}
\newcommand{\bfPsH}{\widehat{\bfPs}}
\newcommand{\bfSigH}{\widehat{\bfSig}}
\newcommand{\bfThH}{\widehat{\bfTh}}
\newcommand{\bfXiH}{\widehat{\bfXi}}

\newcommand{\bfpiH}{\widehat{\bfpi}}
\newcommand{\bfvpiH}{\widehat{\bfvpi}}
\newcommand{\bfalH}{\widehat{\bfal}}
\newcommand{\bfbeH}{\widehat{\bfbe}}
\newcommand{\bfchiH}{\widehat{\bfchi}}
\newcommand{\bfdelH}{\widehat{\bfdel}}
\newcommand{\bfepsvH}{\widehat{\bfepsv}}
\newcommand{\bfepsH}{\widehat{\bfeps}}
\newcommand{\bfetaH}{\widehat{\bfeta}}
\newcommand{\bfgaH}{\widehat{\bfga}}
\newcommand{\bflaH}{\widehat{\bfla}}
\newcommand{\bfkaH}{\widehat{\bfka}}
\newcommand{\bfioH}{\widehat{\bfio}}
\newcommand{\bfmpiH}{\widehat{\bfmpi}}
\newcommand{\bfmuH}{\widehat{\bfmu}}
\newcommand{\bfnuH}{\widehat{\bfnu}}
\newcommand{\bfupsH}{\widehat{\bfups}}
\newcommand{\bfooH}{\widehat{\bfoo}}
\newcommand{\bfphH}{\widehat{\bfph}}
\newcommand{\bfphcH}{\widehat{\bfphc}}
\newcommand{\bfpsH}{\widehat{\bfps}}
\newcommand{\bfrhoH}{\widehat{\bfrho}}
\newcommand{\bfrhvH}{\widehat{\bfrhv}}
\newcommand{\bfsigH}{\widehat{\bfsig}}
\newcommand{\bftauH}{\widehat{\bftau}}
\newcommand{\bfthH}{\widehat{\bfth}}
\newcommand{\bfthvH}{\widehat{\bfthv}}
\newcommand{\bfxiH}{\widehat{\bfxi}}
\newcommand{\bfzetH}{\widehat{\bfzet}}
\newcommand{\btetaH}{\widehat{\bteta}}

%  -----------------------------
%  Boldface Greek letters, red
%  -----------------------------

\newcommand{\bfDelR}{\RBmath{\Delta}}
\newcommand{\bfGaR}{\RBmath{\Gamma}}
\newcommand{\bfLaR}{\RBmath{\Lambda}}
\newcommand{\bfmPiR}{\RBmath{\Pi}}
\newcommand{\bfOmR}{\RBmath{\Omega}}
\newcommand{\bfPhR}{\RBmath{\Phi}}
\newcommand{\bfPiR}{\RBmath{\Pi}}
\newcommand{\bfPsR}{\RBmath{\Psi}}
\newcommand{\bfSigR}{\RBmath{\Sigma}}
\newcommand{\bfThR}{\RBmath{\Theta}}
\newcommand{\bfXiR}{\RBmath{\Xi}}

\newcommand{\bfpiR}{\RBmath{\pi}}
\newcommand{\bfvpiR}{\RBmath{\varpi}}
\newcommand{\bfalR}{\RBmath{\alpha}}
\newcommand{\bfbeR}{\RBmath{\beta}}
\newcommand{\bfchiR}{\RBmath{\chi}}
\newcommand{\bfdelR}{\RBmath{\delta}}
\newcommand{\bfepsvR}{\RBmath{\epsilon}}
\newcommand{\bfepsR}{\RBmath{\varepsilon}}
\newcommand{\bfetaR}{\RBmath{\eta}}
\newcommand{\bfgaR}{\RBmath{\gamma}}
\newcommand{\bflaR}{\RBmath{\lambda}}
\newcommand{\bfkaR}{\RBmath{\kappa}}
\newcommand{\bfioR}{\RBmath{\iota}}
\newcommand{\bfmpiR}{\RBmath{\varpi}}
\newcommand{\bfmuR}{\RBmath{\mu}}
\newcommand{\bfnuR}{\RBmath{\nu}}
\newcommand{\bfupsR}{\RBmath{\upsilon}}
\newcommand{\bfooR}{\RBmath{\omega}}
\newcommand{\bfphR}{\RBmath{\varphi}}
\newcommand{\bfphcR}{\RBmath{\phi}}
\newcommand{\bfpsR}{\RBmath{\psi}}
\newcommand{\bfrhoR}{\RBmath{\rho}}
\newcommand{\bfrhvR}{\RBmath{\varrho}}
\newcommand{\bfsigR}{\RBmath{\sigma}}
\newcommand{\bftauR}{\RBmath{\tau}}
\newcommand{\bfthR}{\RBmath{\theta}}
\newcommand{\bfthvR}{\RBmath{\vartheta}}
\newcommand{\bfxiR}{\RBmath{\xi}}
\newcommand{\bfzetR}{\RBmath{\zeta}}
\newcommand{\btetaR}{\RBmath{\theta}}

%  ----------------------------
%  Boldface Greek letters, blue
%  ----------------------------

\newcommand{\bfDelBB}{\BBmath{\Delta}}
\newcommand{\bfGaBB}{\BBmath{\Gamma}}
\newcommand{\bfLaBB}{\BBmath{\Lambda}}
\newcommand{\bfmPiBB}{\BBmath{\Pi}}
\newcommand{\bfOmBB}{\BBmath{\Omega}}
\newcommand{\bfPhBB}{\BBmath{\Phi}}
\newcommand{\bfPiBB}{\BBmath{\Pi}}
\newcommand{\bfPsBB}{\BBmath{\Psi}}
\newcommand{\bfSigBB}{\BBmath{\Sigma}}
\newcommand{\bfThBB}{\BBmath{\Theta}}
\newcommand{\bfXiBB}{\BBmath{\Xi}}

\newcommand{\bfpiBB}{\BBmath{\pi}}
\newcommand{\bfvpiBB}{\BBmath{\varpi}}
\newcommand{\bfalBB}{\BBmath{\alpha}}
\newcommand{\bfbeBB}{\BBmath{\beta}}
\newcommand{\bfchiBB}{\BBmath{\chi}}
\newcommand{\bfdelBB}{\BBmath{\delta}}
\newcommand{\bfepsvBB}{\BBmath{\epsilon}}
\newcommand{\bfepsBB}{\BBmath{\varepsilon}}
\newcommand{\bfetaBB}{\BBmath{\eta}}
\newcommand{\bfgaBB}{\BBmath{\gamma}}
\newcommand{\bflaBB}{\BBmath{\lambda}}
\newcommand{\bfkaBB}{\BBmath{\kappa}}
\newcommand{\bfioBB}{\BBmath{\iota}}
\newcommand{\bfmpiBB}{\BBmath{\varpi}}
\newcommand{\bfmuBB}{\BBmath{\mu}}
\newcommand{\bfnuBB}{\BBmath{\nu}}
\newcommand{\bfupsBB}{\BBmath{\upsilon}}
\newcommand{\bfooBB}{\BBmath{\omega}}
\newcommand{\bfphBB}{\BBmath{\varphi}}
\newcommand{\bfphcBB}{\BBmath{\phi}}
\newcommand{\bfpsBB}{\BBmath{\psi}}
\newcommand{\bfrhoBB}{\BBmath{\rho}}
\newcommand{\bfrhvBB}{\BBmath{\varrho}}
\newcommand{\bfsigBB}{\BBmath{\sigma}}
\newcommand{\bftauBB}{\BBmath{\tau}}
\newcommand{\bfthBB}{\BBmath{\theta}}
\newcommand{\bfthvBB}{\BBmath{\vartheta}}
\newcommand{\bfxiBB}{\BBmath{\xi}}
\newcommand{\bfzetBB}{\BBmath{\zeta}}
\newcommand{\btetaBB}{\BBmath{\theta}}

%  -----------------------------
%  Boldface Greek letters, green
%  -----------------------------

\newcommand{\bfDelG}{\GBmath{\Delta}}
\newcommand{\bfGaG}{\GBmath{\Gamma}}
\newcommand{\bfLaG}{\GBmath{\Lambda}}
\newcommand{\bfmPiG}{\GBmath{\Pi}}
\newcommand{\bfOmG}{\GBmath{\Omega}}
\newcommand{\bfPhG}{\GBmath{\Phi}}
\newcommand{\bfPiG}{\GBmath{\Pi}}
\newcommand{\bfPsG}{\GBmath{\Psi}}
\newcommand{\bfSigG}{\GBmath{\Sigma}}
\newcommand{\bfThG}{\GBmath{\Theta}}
\newcommand{\bfXiG}{\GBmath{\Xi}}

\newcommand{\bfpiG}{\GBmath{\pi}}
\newcommand{\bfvpiG}{\GBmath{\varpi}}
\newcommand{\bfalG}{\GBmath{\alpha}}
\newcommand{\bfbeG}{\GBmath{\beta}}
\newcommand{\bfchiG}{\GBmath{\chi}}
\newcommand{\bfdelG}{\GBmath{\delta}}
\newcommand{\bfepsvG}{\GBmath{\epsilon}}
\newcommand{\bfepsG}{\GBmath{\varepsilon}}
\newcommand{\bfetaG}{\GBmath{\eta}}
\newcommand{\bfgaG}{\GBmath{\gamma}}
\newcommand{\bflaG}{\GBmath{\lambda}}
\newcommand{\bfkaG}{\GBmath{\kappa}}
\newcommand{\bfioG}{\GBmath{\iota}}
\newcommand{\bfmpiG}{\GBmath{\varpi}}
\newcommand{\bfmuG}{\GBmath{\mu}}
\newcommand{\bfnuG}{\GBmath{\nu}}
\newcommand{\bfupsG}{\GBmath{\upsilon}}
\newcommand{\bfooG}{\GBmath{\omega}}
\newcommand{\bfphG}{\GBmath{\varphi}}
\newcommand{\bfphcG}{\GBmath{\phi}}
\newcommand{\bfpsG}{\GBmath{\psi}}
\newcommand{\bfrhoG}{\GBmath{\rho}}
\newcommand{\bfrhvG}{\GBmath{\varrho}}
\newcommand{\bfsigG}{\GBmath{\sigma}}
\newcommand{\bftauG}{\GBmath{\tau}}
\newcommand{\bfthG}{\GBmath{\theta}}
\newcommand{\bfthvG}{\GBmath{\vartheta}}
\newcommand{\bfxiG}{\GBmath{\xi}}
\newcommand{\bfzetG}{\GBmath{\zeta}}
\newcommand{\btetaG}{\GBmath{\theta}}

%  ------------------
%  Greek letters, bar
%  ------------------

\newcommand{\Deltab}{\bar{\Delta}}
\newcommand{\Gammab}{\bar{\Gamma}}
\newcommand{\Lambdab}{\bar{\Lambda}}
\newcommand{\Pib}{\bar{\Pi}}
\newcommand{\Omegab}{\bar{\Omega}}
\newcommand{\Phib}{\bar{\Phi}}
\newcommand{\Psib}{\bar{\Psi}}
\newcommand{\Sigmab}{\bar{\Sigma}}
\newcommand{\Thetab}{\bar{\Theta}}
\newcommand{\Xib}{\bar{\Xi}}

\newcommand{\pib}{\bar{\pi}}
\newcommand{\alphab}{\bar{\alpha}}
\newcommand{\betab}{\bar{\beta}}
\newcommand{\chib}{\bar{\chi}}
\newcommand{\deltab}{\bar{\delta}}
\newcommand{\epsilonb}{\bar{\epsilon}}
\newcommand{\epsb}{\bar{\varepsilon}}
\newcommand{\etab}{\bar{\eta}}
\newcommand{\gammab}{\bar{\gamma}}
\newcommand{\lambdab}{\bar{\lambda}}
\newcommand{\kappab}{\bar{\kappa}}
\newcommand{\iotab}{\bar{\iota}}
\newcommand{\varpib}{\bar{\varpi}}
\newcommand{\mub}{\bar{\mu}}
\newcommand{\nub}{\bar{\nu}}
\newcommand{\upsilonb}{\bar{\upsilon}}
\newcommand{\omegab}{\bar{\omega}}
\newcommand{\varphib}{\bar{\varphi}}
\newcommand{\phib}{\bar{\phi}}
\newcommand{\psib}{\bar{\psi}}
\newcommand{\rhob}{\bar{\rho}}
\newcommand{\varrhob}{\bar{\varrho}}
\newcommand{\sigmab}{\bar{\sigma}}
\newcommand{\taub}{\bar{\tau}}
\newcommand{\thetab}{\bar{\theta}}
\newcommand{\varthetab}{\bar{\vartheta}}
\newcommand{\xib}{\bar{\xi}}
\newcommand{\zetab}{\bar{\zeta}}

\newcommand{\DeltaB}{\overline{\Delta}}
\newcommand{\GammaB}{\overline{\Gamma}}
\newcommand{\LambdaB}{\overline{\Lambda}}
\newcommand{\PiB}{\overline{\Pi}}
\newcommand{\OmegaB}{\overline{\Omega}}
\newcommand{\PhiB}{\overline{\Phi}}
\newcommand{\PsiB}{\overline{\Psi}}
\newcommand{\SigmaB}{\overline{\Sigma}}
\newcommand{\ThetaB}{\overline{\Theta}}
\newcommand{\XiB}{\overline{\Xi}}

\newcommand{\piB}{\overline{\pi}}
\newcommand{\alphaB}{\overline{\alpha}}
\newcommand{\betaBB}{\overline{\beta}}
\newcommand{\chiB}{\overline{\chi}}
\newcommand{\deltaB}{\overline{\delta}}
\newcommand{\epsilonB}{\overline{\epsilon}}
\newcommand{\epsB}{\overline{\varepsilon}}
\newcommand{\etaBB}{\overline{\eta}}
\newcommand{\gammaB}{\overline{\gamma}}
\newcommand{\lambdaB}{\overline{\lambda}}
\newcommand{\kappaB}{\overline{\kappa}}
\newcommand{\iotaB}{\overline{\iota}}
\newcommand{\varpiB}{\overline{\varpi}}
\newcommand{\muB}{\overline{\mu}}
\newcommand{\nuB}{\overline{\nu}}
\newcommand{\upsilonB}{\overline{\upsilon}}
\newcommand{\omegaB}{\overline{\omega}}
\newcommand{\varphiB}{\overline{\varphi}}
\newcommand{\phiB}{\overline{\phi}}
\newcommand{\psiB}{\overline{\psi}}
\newcommand{\rhoB}{\overline{\rho}}
\newcommand{\varrhoB}{\overline{\varrho}}
\newcommand{\sigmaB}{\overline{\sigma}}
\newcommand{\tauB}{\overline{\tau}}
\newcommand{\thetaB}{\overline{\theta}}
\newcommand{\varthetaB}{\overline{\vartheta}}
\newcommand{\xiB}{\overline{\xi}}
\newcommand{\zetaB}{\overline{\zeta}}

%  ------------------
%  Greek letters, hat
%  ------------------

\newcommand{\Deltat}{\tilde{\Delta}}
\newcommand{\Gammat}{\tilde{\Gamma}}
\newcommand{\Lambdat}{\tilde{\Lambda}}
\newcommand{\Omegat}{\tilde{\Omega}}
\newcommand{\Phit}{\tilde{\Phi}}
\newcommand{\Pit}{\tilde{\Pi}}
\newcommand{\Psit}{\tilde{\Psi}}
\newcommand{\Sigmat}{\tilde{\Sigma}}
\newcommand{\Thetat}{\tilde{\Theta}}
\newcommand{\Xit}{\tilde{\Xi}}

\newcommand{\pit}{\tilde{\pi}}
\newcommand{\alphat}{\tilde{\alpha}}
\newcommand{\betat}{\tilde{\beta}}
\newcommand{\chit}{\tilde{\chi}}
\newcommand{\deltat}{\tilde{\delta}}
\newcommand{\epsilont}{\tilde{\epsilon}}
\newcommand{\epst}{\tilde{\varepsilon}}
\newcommand{\etat}{\tilde{\eta}}
\newcommand{\gammat}{\tilde{\gamma}}
\newcommand{\lambdat}{\tilde{\lambda}}
\newcommand{\kappat}{\tilde{\kappa}}
\newcommand{\iotat}{\tilde{\iota}}
\newcommand{\varpit}{\tilde{\varpi}}
\newcommand{\mut}{\tilde{\mu}}
\newcommand{\nut}{\tilde{\nu}}
\newcommand{\upsilont}{\tilde{\upsilon}}
\newcommand{\omegat}{\tilde{\omega}}
\newcommand{\varphit}{\tilde{\varphi}}
\newcommand{\phit}{\tilde{\phi}}
\newcommand{\psit}{\tilde{\psi}}
\newcommand{\rhot}{\tilde{\rho}}
\newcommand{\varrhot}{\tilde{\varrho}}
\newcommand{\sigmat}{\tilde{\sigma}}
\newcommand{\taut}{\tilde{\tau}}
\newcommand{\thetat}{\tilde{\theta}}
\newcommand{\varthetat}{\tilde{\vartheta}}
\newcommand{\xit}{\tilde{\xi}}
\newcommand{\zetat}{\tilde{\zeta}}

\newcommand{\DeltaT}{\widetilde{\Delta}}
\newcommand{\GammaT}{\widetilde{\Gamma}}
\newcommand{\LambdaT}{\widetilde{\Lambda}}
\newcommand{\OmegaT}{\widetilde{\Omega}}
\newcommand{\PhiT}{\widetilde{\Phi}}
\newcommand{\PiT}{\widetilde{\Pi}}
\newcommand{\PsiT}{\widetilde{\Psi}}
\newcommand{\SigmaT}{\widetilde{\Sigma}}
\newcommand{\ThetaT}{\widetilde{\Theta}}
\newcommand{\XiT}{\widetilde{\Xi}}

\newcommand{\piT}{\widetilde{\pi}}
\newcommand{\alphaT}{\widetilde{\alpha}}
\newcommand{\betaT}{\widetilde{\beta}}
\newcommand{\chiT}{\widetilde{\chi}}
\newcommand{\deltaT}{\widetilde{\delta}}
\newcommand{\epsilonT}{\widetilde{\epsilon}}
\newcommand{\epsT}{\widetilde{\varepsilon}}
\newcommand{\etaT}{\widetilde{\eta}}
\newcommand{\gammaT}{\widetilde{\gamma}}
\newcommand{\lambdaT}{\widetilde{\lambda}}
\newcommand{\kappaT}{\widetilde{\kappa}}
\newcommand{\iotaT}{\widetilde{\iota}}
\newcommand{\varpiT}{\widetilde{\varpi}}
\newcommand{\muT}{\widetilde{\mu}}
\newcommand{\nuT}{\widetilde{\nu}}
\newcommand{\upsilonT}{\widetilde{\upsilon}}
\newcommand{\omegaT}{\widetilde{\omega}}
\newcommand{\varphiT}{\widetilde{\varphi}}
\newcommand{\phiT}{\widetilde{\phi}}
\newcommand{\psiT}{\widetilde{\psi}}
\newcommand{\rhoT}{\widetilde{\rho}}
\newcommand{\varrhoT}{\widetilde{\varrho}}
\newcommand{\sigmaT}{\widetilde{\sigma}}
\newcommand{\tauT}{\widetilde{\tau}}
\newcommand{\thetaT}{\widetilde{\theta}}
\newcommand{\varthetaT}{\widetilde{\vartheta}}
\newcommand{\xiT}{\widetilde{\xi}}
\newcommand{\zetaT}{\widetilde{\zeta}}
%  ------------------
%  Greek letters, tilde
%  ------------------

\newcommand{\Deltah}{\hat{\Delta}}
\newcommand{\Gammah}{\hat{\Gamma}}
\newcommand{\Lambdah}{\hat{\Lambda}}
\newcommand{\Omegah}{\hat{\Omega}}
\newcommand{\Phih}{\hat{\Phi}}
\newcommand{\Pih}{\hat{\Pi}}
\newcommand{\Psih}{\hat{\Psi}}
\newcommand{\Sigmah}{\hat{\Sigma}}
\newcommand{\Thetah}{\hat{\Theta}}
\newcommand{\Xih}{\hat{\Xi}}

\newcommand{\pih}{\hat{\pi}}
\newcommand{\alphah}{\hat{\alpha}}
\newcommand{\betah}{\hat{\beta}}
\newcommand{\chih}{\hat{\chi}}
\newcommand{\deltah}{\hat{\delta}}
\newcommand{\epsilonh}{\hat{\epsilon}}
\newcommand{\epsh}{\hat{\varepsilon}}
\newcommand{\etah}{\hat{\eta}}
\newcommand{\gammah}{\hat{\gamma}}
\newcommand{\lambdah}{\hat{\lambda}}
\newcommand{\kappah}{\hat{\kappa}}
\newcommand{\iotah}{\hat{\iota}}
\newcommand{\varpih}{\hat{\varpi}}
\newcommand{\muh}{\hat{\mu}}
\newcommand{\nuh}{\hat{\nu}}
\newcommand{\upsilonh}{\hat{\upsilon}}
\newcommand{\omegah}{\hat{\omega}}
\newcommand{\varphih}{\hat{\varphi}}
\newcommand{\phih}{\hat{\phi}}
\newcommand{\psih}{\hat{\psi}}
\newcommand{\rhoh}{\hat{\rho}}
\newcommand{\varrhoh}{\hat{\varrho}}
\newcommand{\sigmah}{\hat{\sigma}}
\newcommand{\tauh}{\hat{\tau}}
\newcommand{\thetah}{\hat{\theta}}
\newcommand{\varthetah}{\hat{\vartheta}}
\newcommand{\xih}{\hat{\xi}}
\newcommand{\zetah}{\hat{\zeta}}

\newcommand{\DeltaH}{\widehat{\Delta}}
\newcommand{\GammaH}{\widehat{\Gamma}}
\newcommand{\LambdaH}{\widehat{\Lambda}}
\newcommand{\PiH}{\widehat{\Pi}}
\newcommand{\OmegaH}{\widehat{\Omega}}
\newcommand{\PhiH}{\widehat{\Phi}}
\newcommand{\PsiH}{\widehat{\Psi}}
\newcommand{\SigmaH}{\widehat{\Sigma}}
\newcommand{\ThetaH}{\widehat{\Theta}}
\newcommand{\XiH}{\widehat{\Xi}}

\newcommand{\piH}{\widehat{\pi}}
\newcommand{\alphaH}{\widehat{\alpha}}
\newcommand{\betaH}{\widehat{\beta}}
\newcommand{\chiH}{\widehat{\chi}}
\newcommand{\deltaH}{\widehat{\delta}}
\newcommand{\epsilonH}{\widehat{\epsilon}}
\newcommand{\epsH}{\widehat{\varepsilon}}
\newcommand{\etaH}{\widehat{\eta}}
\newcommand{\gammaH}{\widehat{\gamma}}
\newcommand{\lambdaH}{\widehat{\lambda}}
\newcommand{\kappaH}{\widehat{\kappa}}
\newcommand{\iotaH}{\widehat{\iota}}
\newcommand{\varpiH}{\widehat{\varpi}}
\newcommand{\muH}{\widehat{\mu}}
\newcommand{\nuH}{\widehat{\nu}}
\newcommand{\upsilonH}{\widehat{\upsilon}}
\newcommand{\omegaH}{\widehat{\omega}}
\newcommand{\varphiH}{\widehat{\varphi}}
\newcommand{\phiH}{\widehat{\phi}}
\newcommand{\psiH}{\widehat{\psi}}
\newcommand{\rhoH}{\widehat{\rho}}
\newcommand{\varrhoH}{\widehat{\varrho}}
\newcommand{\sigmaH}{\widehat{\sigma}}
\newcommand{\tauH}{\widehat{\tau}}
\newcommand{\thetaH}{\widehat{\theta}}
\newcommand{\varthetaH}{\widehat{\vartheta}}
\newcommand{\xiH}{\widehat{\xi}}
\newcommand{\zetaH}{\widehat{\zeta}}



%  ----------------------
%  Boldface Greek letters
%  ----------------------

\newcommand{\bfDel}{\boldsymbol{\Delta}}
\newcommand{\bfGa}{\boldsymbol{\Gamma}}
\newcommand{\bfLa}{\boldsymbol{\Lambda}}
\newcommand{\bfmPi}{\boldsymbol{\Pi}}
\newcommand{\bfOm}{\boldsymbol{\Omega}}
\newcommand{\bfPh}{\boldsymbol{\Phi}}
\newcommand{\bfPi}{\boldsymbol{\Pi}}
\newcommand{\bfPs}{\boldsymbol{\Psi}}
\newcommand{\bfSig}{\boldsymbol{\Sigma}}
\newcommand{\bfTh}{\boldsymbol{\Theta}}
\newcommand{\bfXi}{\boldsymbol{\Xi}}

\newcommand{\bfpi}{\boldsymbol{\pi}}
\newcommand{\bfvpi}{\boldsymbol{\varpi}}
\newcommand{\bfal}{\boldsymbol{\alpha}}
\newcommand{\bfbe}{\boldsymbol{\beta}}
\newcommand{\bfchi}{\boldsymbol{\chi}}
\newcommand{\bfdel}{\boldsymbol{\delta}}
\newcommand{\bfepsv}{\boldsymbol{\epsilon}}
\newcommand{\bfeps}{\boldsymbol{\eps}}
\Newcommand{\bfeta}{\boldsymbol{\eta}}
\newcommand{\bfga}{\boldsymbol{\gamma}}
\newcommand{\bfla}{\boldsymbol{\lambda}}
\newcommand{\bfka}{\boldsymbol{\kappa}}
\newcommand{\bfio}{\boldsymbol{\iota}}
\newcommand{\bfmpi}{\boldsymbol{\varpi}}
\newcommand{\bfmu}{\boldsymbol{\mu}}
\newcommand{\bfnu}{\boldsymbol{\nu}}
\newcommand{\bfups}{\boldsymbol{\upsilon}}
\newcommand{\bfoo}{\boldsymbol{\omega}}
\newcommand{\bfph}{\boldsymbol{\varphi}}
\newcommand{\bfphc}{\boldsymbol{\phi}}
\newcommand{\bfps}{\boldsymbol{\psi}}
\newcommand{\bfrho}{\boldsymbol{\rho}}
\newcommand{\bfrhv}{\boldsymbol{\varrho}}
\newcommand{\bfsig}{\boldsymbol{\sigma}}
\newcommand{\bftau}{\boldsymbol{\tau}}
\newcommand{\bfth}{\boldsymbol{\theta}}
\newcommand{\bfthv}{\boldsymbol{\vartheta}}
\newcommand{\bfxi}{\boldsymbol{\xi}}
\newcommand{\bfzet}{\boldsymbol{\zeta}}
\newcommand{\bteta}{\boldsymbol{\theta}}



==> files/others.tex <==
%  Environnements
\newenvironment{cmatrix}{\left\{\begin{matrix}}{\end{matrix}\right\}}

\newcommand{\Newcommand}[2]{\providecommand{#1}{}\renewcommand{#1}{#2}}


\newcommand{\retainlabel}[1]{\label{#1}\sbox0{\ref{#1}}}
%--------------------------------------------------------------------------------------
%  Title-inserting command, used in proofs cut into steps
%-------------------------------------------------------------------------------------
\makeatletter
\newcommand{\proofstep}[1]{%
  \par% ensure starting on a new paragraph
  \addvspace{\smallskipamount}% some vertical space
  \textit{#1\@addpunct{.}}\enspace\ignorespaces
}
\makeatother
%--------------------------------------------------------------------------------------
%  Blank box placeholder for figures (to avoid requiring any
%  particular graphics capabilities for printing this document). From amsart.
%-------------------------------------------------------------------------------------
\newcommand{\blankbox}[2]{%
  \parbox{\columnwidth}{\centering
%    Set fboxsep to 0 so that the actual size of the box will match the
%    given measurements more closely.
    \setlength{\fboxsep}{0pt}%
    \fbox{\raisebox{0pt}[#2]{\hspace{#1}}}%
  }%
}

